Complexity of Discrete Energy Minimization Problems

Discrete energy minimization is widely-used in computer vision and machine learning for problems such as MAP inference in graphical models. The problem, in general, is notoriously intractable, and finding the global optimal solution is known to be NP-hard. However, is it possible to approximate this problem with a reasonable ratio bound on the solution quality in polynomial time? We show in this paper that the answer is no. Specifically, we show that general energy minimization, even in the 2-label pairwise case, and planar energy minimization with three or more labels are exp-APX-complete. This finding rules out the existence of any approximation algorithm with a sub-exponential approximation ratio in the input size for these two problems, including constant factor approximations. Moreover, we collect and review the computational complexity of several subclass problems and arrange them on a complexity scale consisting of three major complexity classes -- PO, APX, and exp-APX, corresponding to problems that are solvable, approximable, and inapproximable in polynomial time. Problems in the first two complexity classes can serve as alternative tractable formulations to the inapproximable ones. This paper can help vision researchers to select an appropriate model for an application or guide them in designing new algorithms.

==> content/ideas.tex <==
\section{Alternative Ideas}



%:::\revisit[Do we still need the paragraph below? It is a detailed example on how this paper might provide guidance on selection an appropriate model for an application] ::Daniel to check it later
% also the importance of constant factor approximation
% In applications, it is preferable to formulate a real-world problem as a computational problem solvable in polynomial time. However, when the application requires a more complex model whose a global optimum is intractable, it is often satisfactory to solve the problem to a desired relative accuracy in the objective, \ie, reaching the optimum within a given ratio. Indeed, such algorithms exist such as the well-known Potts model can be approximated by alpha-expansion \cite{boykov2001approximate} within a constant factor of 2. In structural learning \cite{finley2008training} for example, it is acceptable to have a constant factor approximation algorithm for the inference oracle, also an instance of energy minimization, when efficient exact algorithms are not available. This is because the constant factor approximation for the inference oracle can yield a multiplicative bound on the learning objective, providing a relative guarantee for the quality of the learned parameters. In sum, the solution quality of structural learning depends on the approximation guarantees of the energy minimization subroutine. It is shown in cite{another eccv submission} that when such an efficient subroutine is impossible even in terms of constant ratio approximation, we should reformulate the learning objective to make the learning problem tractable.

%::: move to later... Therefore, algorithm designers should not expect to prove a reasonable approximation ratio guarantee for their algorithms on general energy minimization algorithms.

% When terms depending on three or more variables are present in~\eqref{eq:1}, the problem is known as {\em higher-order}\footnote{There is a discrepancy in the literature on whether to refer to~\eqref{eq:1} as first or second order. It has first order interactions when viewed as a Markov model. On the other hand, in QPBO it is a second order polynomial in $x$.}. We focus primarily on the pairwise case but notate results that hold for higher order as well. In the higher order pseudo-Boolean case, the problem is known as general pseudo-Boolean optimization or as $0$-$1$ polynomial programming.


% \paragraph{Complexity Classes} For decision problems, class NP (nondeterministic polynomial time) includes problems whose solution can be verified in polynomial time. Analogously for optimization problems, class NPO (NP-optimization) is introduced for problems whose solution feasibility can be verified in polynomial time. Its formal definition is given in \Section{sec:complexitytheory}. 
% %::: section does not exist
% The NP-hardness of an optimization problem means it is at least as hard as the hardest decision problem in the class NP. These concepts are illustrated in \Figure{fig:Classes-P-NP}.

% \begin{figure}[t]
% \begin{center}
% \resizebox{0.9\linewidth}{!}{
% \begin{tabular}{cc}
% \begin{tabular}{c}\includegraphics[width=0.43\linewidth]{figure/Classes-P-NP-crop.pdf}\end{tabular}%
% \ \ 
% 	 \begin{tabular}{c}\includegraphics[width=0.5\linewidth]{figure/Classes-NP-hard-crop.pdf}\\[5pt]
% 	\end{tabular}%
% 	\end{tabular}
% 	}
% \end{center}
%   \caption{Left: relation of complexity classes between decision and optimization problems. Optimization problems ``contain'' decision problems since any decision problem can be cast as an optimization over the set $\{$yes, no$\}$. If not clear from the picture, P $\subseteq$ NP, P $\subseteq$ PO and NP $\subseteq$ NPO. Right: arrows indicate that a problem can be reduced to other problem in polynomial time. %All NP problems can be reduced to NP-complete problems. If a problem is such that an NP-complete problem reduces to it, 
% % I am not sure you need to include the right part of the figure.  Anyone reading the paper should understand the basic concept of a reduction.
% NP-hard class contains NP-complete problems and all problems (not necessarily decision) that are at least as hard (to which an NP-complete problem, and thus all problems in NP, may be reduced).
% }
% \label{fig:Classes-P-NP}
% \end{figure}

Suggestions for the right part figure 2 (update: already merged with figure 1 now):

Three ways to improve it:

1. Keep the idea of using dots as problems and edges as reductions, but makes solid arrows larger and replace hollow arrows with a dotted boundary for NP-complete problems.

2. Actually, wikipedia has a nice figure explaining this problem:
\par
\url{https://en.wikipedia.org/wiki/P_versus_NP_problem#/media/File:P_np_np-complete_np-hard.svg}
\par
We don't need to introduce reduction here for a) simplicity, b) avoid technical issues:
Karp reduction is used for reductions among decision problems while Turing reduction is used from decision problems to optimization problems. In other words, the typical reduction used for decision problems does not work for optimizaiton problems.

3. Just remove the right half of figure 2 as it is already something well explained on Wikipedia. We can resort to just text explanation.

---------------------------------------





   %Discrete energy minimization is an established work engine for performing inference in graphical models 
%   Discrete energy minimization is a recognized optimization problem, used to solve MAP inference in graphical models and closely related to several well-known combinatorial optimization problems.
%<<<<<<< Updated upstream
   %In this paper we give a comprehensive overview of subclasses solvable in polynomial time as well as subclasses admitting a constant factor approximation. We further contribute to the study of complexity by showing that general energy minimization is exp-APX-complete, meaning it is as hard as any optimization problem with a polynomial-time computable objective function and whose arbitrary feasible solution can be found in polynomial time, and the general problem cannot be approximated with a better then exponential factor. The result holds already in case of two labels, \ie, for quadratic pseudo-Boolean optimization. Further, we show that planar problem with 3 labels is exp-APX-complete as well.
%% \par
% \revisit[I think it might be better to keep the exponential factor as in previous version. "as hard as bla bla" is still vague to people without a sense of what is an optimization problem.]
%=======
%   In this paper we give a comprehensive overview of subclasses solvable in polynomial time as well as subclasses admitting a constant factor approximation. We further contribute to the study of complexity by showing that general energy minimization is exp-APX-complete, meaning that 
% 	it is NP-hard to approximate it with a subexponential ratio. %find a solution with energy within a subexponential (in the problem size) factor of the minimum.
%  %and cannot be approximated with a better then exponential factor. 
% The result holds already in case of two labels, \ie, for quadratic pseudo-Boolean optimization. Further, we show that planar problem with 3 labels is exp-APX-complete as well.
% \par
% %\revisit[I think it might be better to keep the exponential factor as in previous version. "as hard as bla bla" is still vague to people without a sense of what is an optimization problem.]
% %>>>>>>> Stashed changes
     
% \revisit[See ideas.tex for an alternative abstract that is tied closer to computer vision]


% Discrete energy minimization problem, which can be used to solve MAP inference for graphical models, is widely adopted in computer vision and machine learning. Despite many subclass problems are identified as NP-hard, they are still used to model real world applications. In this paper, we present a comprehensive overview of the computational complexity of subclass problems by arranging them on a finer complexity scale consisting of three major complexity classes --- PO, APX, exp-APX, corresponding to problems that are solvable, approximable, inapproximable in polynomially time. The connections of these subclass problems will also be analyzed. We hope this overview will aid researchers in designing new optimization algorithms
% and in selecting appropriate models for their applications. Moreover, we contribute two important additions to this overview by showing that general energy minimization and planar 3-label energy minimization are exp-APX-complete. This essentially mean that there cannot be any approximation algorithm with an approximation ratio better than an exponential function in the input size for these two problems. Therefore algorithm designers should not expect to prove a reasonable approximation ratio guarantee for their algorithms on these problems.


---------------------------

Previous version of the related works:


% NP-hardness has been shown for the MAP assignment of belief networks by~\citet{Cooper-90} and \citet{Shimony-94}. \citet{Abdelbar-98} has shown that approximating the MAP assignment is also NP-hard. However, there are substantial differences from our result.
% Belief networks have a probability density function $p(x)$ that factors according to a directed acyclic graph, \eg, as $p(x_1,x_2,x_3) = p(x_1 | x_2,x_3)p(x_2)p(x_3)$. %Using the relation $p(x) = \exp(-f(x))$, 
% %The negative logarithm of the pdf is then representable as a partially separable function of the form~\eqref{eq:1}. Maximization of the probability 
% For belief networks, finding the MAP assignment\footnote{Same as the most probable estimate (MPE).} in a Bayesian network is related to energy minimization~\eqref{eq:1} by letting $f(x) = -\log(p(x))$. The product is transformed into the sum and so, \eg, factor $p(x_1 | x_2,x_3)$ corresponds to term $f_{1,2,3}(x_1,x_2,x_3)$.
% %
% Note, factors of at most two variables, \eg, $p(x_1 | x_2)$, can form only a tree-structured model. % and therefore a Bayesian Network corresponding to a given energy may require higher order factors.
% %In the other direction, 
% Therefore, a Bayesian network corresponding to the pairwise energy~\eqref{eq:1} may require to use factors of order up to $|V|$. \revisit[this sentence is confusing] % in the Bayesian Network representation. 
% It is seen that while the general problems are convertible, fixed-parameter classes (such as order and graph restrictions) differ. In addition, approximation ratio for probabilities translates to an absolute approximation (an additive bound) for energies.


% \citet{Abdelbar-98} has shown that approximating the MAP assignment is also NP-hard. However, there are substantial differences from our result.

% are two neccessary conditions for the problem to be in PO. 
% more general means not only undirected graphical models,
% not only MAP inference, also marginal, partition function

% how to properly cite this?
% http://www.cs.huji.ac.il/project/PASCAL/index.php

% It is well-known that QPBO is NP-hard, since it generalizes such problems as maximum cut and maximum 2-satisfiability~\cite{Karp-72}. 
% These problems are also known to be APX-complete~\cite{Papadimitriou-91} (implies NP-hardness). Therefore, QPBO is APX-hard.
% %::: this does not flow very well.  This next text is not really related work.  It is more about our work.  Maybe better to just say "In this paper, we prove the stronger claim that QPBO is complete in exp-APX."
% Completeness in exp-APX is stronger. 
%::: suggest moving the following text to the section on the proof.
% In particular, it shows that such problems as general traveling salesman problem (TSP) can be reduced to QPBO while preserving approximation ratio in a linear fashion.

%:::\revisit[Consider finding a place to explicitly stating that BNs capture different families of distributions than energy minimization and thus they are used to model different problems]

% NP-hardness has been shown for the MAP assignment of belief networks by~\citet{Cooper-90} and \citet{Shimony-94}. \citet{Abdelbar-98} has shown that approximating the MAP assignment is also NP-hard. However, there are substantial differences from our result.
% Belief networks have a probability density function $p(x)$ that factors according to a directed acyclic graph, \eg, as $p(x_1,x_2,x_3) = p(x_1 | x_2,x_3)p(x_2)p(x_3)$. %Using the relation $p(x) = \exp(-f(x))$, 
% %The negative logarithm of the pdf is then representable as a partially separable function of the form~\eqref{eq:1}. Maximization of the probability 
% For belief networks, finding the MAP assignment\footnote{Same as the most probable estimate (MPE).} in a Bayesian network is related to energy minimization~\eqref{eq:1} by letting $f(x) = -\log(p(x))$. The product is transformed into the sum and so, \eg, factor $p(x_1 | x_2,x_3)$ corresponds to term $f_{1,2,3}(x_1,x_2,x_3)$.
% %
% Note, factors of at most two variables, \eg, $p(x_1 | x_2)$, can form only a tree-structured model. % and therefore a Bayesian Network corresponding to a given energy may require higher order factors.
% %In the other direction, 
% Therefore, a Bayesian network corresponding to the pairwise energy~\eqref{eq:1} may require to use factors of order up to $|V|$. \revisit[this sentence is confusing] % in the Bayesian Network representation. 
% It is seen that while the general problems are convertible, fixed-parameter classes (such as order and graph restrictions) differ. In addition, approximation ratio for probabilities translates to an absolute approximation (an additive bound) for energies.
% %Matching the pairwise model~\eqref{eq:1} is not possible unless the Bayesian network is a chain. 
% %It is not possible to end up with a pairwise model~\eqref{eq:1} unless the Bayesian network is a chain. 
% %The factorization can be regarded as a Gibbs distribution, with the same factors.
% %When written as a Gibbs distribution, the order of the factors (the number of variables involved)
% \par
% \citet{Abdelbar-98} has shown that approximating the MAP assignment in the value of probability, \ie, finding $x$ such that
% \begin{align}\label{p-approx-ratio}
% \frac{p(x^*)}{p(x)} \leq r(n)
% \end{align}
% with a constant or polynomial ratio $r(n) \geq 1$ is NP-hard, showing that this problem is poly-APX-hard. 
% This result holds even after restricting to binary variables and factors of order 3.\footnote{\citet[\parSym 6.1]{Abdelbar-98} count incoming edges of the network: for a factor $p(x_1 | x_2,x_3)$ there are two, but the total number of variables it couples is 3.} In addition they showed that the following problems are also APX-hard:
% \begin{itemize}
% \item knowing the optimal solution, approximate the next optimal solution;
% \item knowing the optimal solution, approximate the optimal solution conditioned on a changed assignment of one variable. 
% \end{itemize}
% %The difference to our result is that approximation ration for MPE translates to additive approximation of energies (in order to translate a multiplicative factorization of a Belief Network to an additive one of the form~\eqref{eq:1}, the connection should be given by $p(x) = \exp(-E(x))$). 
% %Additionally, their proof was given for a model involving four-tuple interactions (three-tuple in case of~\cite[\parSym 6.1]{Abdelbar-98}), and in this respect ours is a refinement. 
% %We also imply a stronger hardness: while \cite{Abdelbar-98} shows it is NP-hard to approximate with a polynomial factor, we show it is NP-hard to approximate with a subexponential factor.
% However, \eqref{p-approx-ratio} translates to an absolute energy approximation with a bound of $\log (r(n))$, \ie, logarithmic in $n$. We will show as a corollary from our result that it provides a stronger inapproximability for probabilities. % than poly-APX-hard.
% %We will show as a corollary from our result that approximating in the value of probability is exp-APX-complete as well, which in particular implies the problem is poly-APX-hard.
% \par
% \citet{Kwisthout-11} showed NP-hardness of absolute approximation in the value of probability for MAP in Bayesian networks, and also studied different approximation measures: structure- rank- and expectation approximations and has established similar inapproximability results for them~\cite{Kwisthout-13}.
% %that is it NP-hard to find a solution $x$ such that 
% %$p(x) \geq p(x^*) - \rho$
% %that additive $\pro$-approximation of MAP is NP-hard for $\rho \geq > $.
% % \par
% % \revisit How additive approximation relates to multiplicative. Does our result implies \citet{Abdelbar-98} or other way around?

% %also that finding an approximate solution with the value of posteriori probability by at most  solution is NP-hard as well.
% %\citet{Abdelbar-98} has shown 

% %Work on stating the inference is NP-hard

% % Work on investigating the hardness of the problem from approximation perspective

% % Work on establishing complexity scales, i.e. by reductions other than AP-reduction.



==> content/postsubmissionTODO.tex <==
> [done] Planar 2-label problems are APX-hard,
as planar vertex cover is in APX:
http://dl.acm.org/citation.cfm?id=802205

> [done] Caption for figure 1. This scale defines a partial order on the hardness. The relationships of the complexity classes is given in eq ().

> [done] In the proof, '3-label problem' should be replaced with '3rd order 2-label problem'.

> [done] Expanding motivation and practical implication in the introduction

> [done] Typo fix, approximiable/inapproximiable -> approximable/inapproximable.

> [not fixed, since no good answer to this question] Better explanation on the sign problem (as in practice the sign can be negative). Note we cannot constrain all the potentials to be non-negative as negative potentials are used in the proof.

> [done] Add more text of the usefulness of our result

Comments from the first reviewer:
"
My complaints are mostly minor -- there are a few ways the paper could be improved to be more helpful to future researchers.

Figure 1 could use some work -- if I were to guess, this is likely to be the most frequently excerpted part of this paper, as it puts the current state of knowledge on these problems in one picture.

In particular, having the complexity classes as being points on the vertical line is somewhat confusing to me, as really they are subintervals or nested subsets, etc. Some different notation for classes vs. problems would be helpful. It might also make it more compact to have a set of nested ovals or similar? 

Also, I would encourage adding a few more of the most used problem classes with known complexity, in particular tree-structured graphs.

Line 33: You mention the pairwise case -- it may be worth pointing out that your results also cover the higher-order case as well, since as part of your proof of Theorem 3.1, you reduce w-3sat-triv to the higher order case first, and then from there to QPBO.

Definition 2.8: This is definitely the least intuitive definition of the paper -- I understand you're following previous notation, but since your proofs don't actually use the rational "r", maybe consider dropping it? Also, just giving some intuition that pi maps from instance1 to instance2, and sigma maps back from feasible solution2 to feasible solution1 would be helpful.

Proof of 3.1: Line 314, you say "3-label energy minimization" but I'm pretty sure you mean "2-label but higher order with cliques of size 3" (which is what the proof in the appendix does). 
Additionally, I don't think steps 4-6 are a good use of space in your proof sketch: they are basically just the standard recipe for proofs of AP reduction, and you've already said what they need to be in the preceding section. Instead, a simple line of "this construction gives an AP-reduction from w3sat-triv to QPBO, and therefore QPBO is exp-APX-complete" would suffice. This gives more space for including some details from the construction, such as the definition of the polynomial used (which is straightforward, and would help give more intuition to readers).

Similarly for 4.1, I would omit steps 2-4 and replace with a single line.
"


==> tcbbreakable.code.tex <==
%% The LaTeX package tcolorbox - version 3.80 (2015/11/27)
%% tcbbreakable.code.tex: Code for breakable colorboxes
%%
%% -------------------------------------------------------------------------------------------
%% Copyright (c) 2006-2015 by Prof. Dr. Dr. Thomas F. Sturm <thomas dot sturm at unibw dot de>
%% -------------------------------------------------------------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2005/12/01 or later.
%%
%% This work has the LPPL maintenance status `author-maintained'.
%%
%% This work consists of all files listed in README
%%
\tcb@set@library@version{3.80}

\let\tcb@parboxrestore@true=\tcb@parboxrestore
\let\tcb@parboxrestore@false\tcb@parbox@false@settings

% total height for boxes smaller than 0.4375\maxdimen and 0.4375\maxdimen else (ca 2.5m)
\def\tcb@defToTotalHeightBreakable#1#2{%
  \ifnum\ht#2<0 %
    \edef#1{7168pt}%
  \else\ifnum\ht#2<469762048 %
    \tcbdimto#1{\ht#2+\dp#2}%
  \else%
    \edef#1{7168pt}%
  \fi\fi%
}

\newbox\tcb@testbox

% for oversized boxes height is detected as \textheight or larger
\def\tcb@defToTotalHeightUnlimited#1#2{%
  \tcb@defToTotalHeightBreakable#1#2%
  \ifdim\dimexpr#1<\textheight\relax%
    \edef\tcb@thevfuzz{\the\vfuzz}%
    \edef\tcb@thevbadness{\the\vbadness}%
    \vfuzz=\maxdimen\vbadness=10000%
    \splittopskip=0pt%
    \splitmaxdepth=0pt%
    \savingvdiscards=1%
    \setbox\tcb@testbox=\vsplit#2 to \textheight%
    \vbadness=\tcb@thevbadness\vfuzz=\tcb@thevfuzz%
    \ifdim\wd#2=0pt\relax%
      \tcb@swap{#2}{\tcb@testbox}%
      \tcbdimto#1{\ht#2+\dp#2}%
    \else%
      \setbox#2=\vbox{%
        \unvbox\tcb@testbox%
        \splitdiscards%
        \unvbox#2}%
      \edef#1{7168pt}%
    \fi%
    \savingvdiscards=0%
  \fi%
}


\def\tcb@vbox#1#2{%
  \edef\reserved@a{%
    \endgroup%
    \setbox#1\vbox{\hsize=#2%
      \begingroup\aftergroup}%
      \def\noexpand\@currenvir{\@currenvir}%
      \def\noexpand\@currenvline{\on@line}}%
  \reserved@a%
  \@endpefalse%
  \color@begingroup%
  \textwidth\hsize%
  \columnwidth\hsize%
  \csname tcb@parboxrestore@\kvtcb@parbox\endcsname%
  \def\@mpfn{mpfootnote}%
  \def\thempfn{\thempfootnote}%
  \c@mpfootnote\z@%
  \let\@footnotetext\@mpfootnotetext%
  \let\@listdepth\@mplistdepth \@mplistdepth\z@%
  \@setminipage\tcb@hyph@fix%
  \let\tcb@drawcolorbox\tcb@drawcolorbox@standalone%
  \let\FN@pp@footnote\@empty% disable perpage mode of 'footmisc' package
  \ignorespaces%
}

\def\endtcb@vbox{%
  \par%
  \unskip%
  \ifvoid\@mpfootins\else%
    \vskip\skip\@mpfootins%
    \normalcolor%
    \footnoterule%
    \unvbox\@mpfootins%
  \fi%
  \@minipagefalse%
  \color@endgroup}

% remaining height
\def\tcb@comp@h@page{%
  \tcb@breakat@next%
  \ifdim\tcb@breakat@dim>0pt\relax%
    \tcbdimto\tcb@h@page{\tcb@breakat@dim-\kvtcb@shrinkbreakgoal}%
  \else%
    \ifx\kvtcb@float\@empty%
      \iftcb@multicol%
        \tcbdimto\tcb@h@page{\textheight-\kvtcb@shrinkbreakgoal}%
      \else%
        \ifdim\pagegoal=16383.99998pt
          \tcbdimto\tcb@h@page{\vsize-\kvtcb@shrinkbreakgoal}% detects floating objects
        \else%
          \tcb@comp@compress%
          \tcbdimto\tcb@h@page{\pagegoal-\pagetotal+\tcb@compress@height-\kvtcb@shrinkbreakgoal}%
        \fi%
      \fi%
    \else%
      \tcbdimto\tcb@h@page{\textheight-\kvtcb@shrinkbreakgoal}%
    \fi%
  \fi%
}

\def\tcb@comp@h@total@standalone{%
  \tcbdimto\tcb@h@padding{\kvtcb@bbtop@stand+\kvtcb@bbbottom@stand+\kvtcb@top@rule@stand+\kvtcb@bottom@rule@stand+\kvtcb@boxsep*2+\kvtcb@top+\kvtcb@bottom}%
  \tcbdimto\tcb@h@total{\tcb@h@padding+\tcb@h@padtitle+\tcb@h@upper+\tcb@h@segment+\tcb@h@lower}%
}


\newif\iftcb@final@box

\def\tcb@check@for@final@box{%
  \ifdim\tcb@h@total>\tcb@h@page\relax%
    \iftcb@multicol%
      \tcb@final@boxfalse%
    \else%
      \ifdim\tcb@h@total>\dimexpr\tcb@h@page+\kvtcb@enlargepage@flex\relax%
        \tcb@final@boxfalse%
      \else%
        \tcbdimto\tcb@temp{\tcb@h@total-\tcb@h@page}%
        \enlargethispage*{\tcb@temp}%
        \tcbdimto\tcb@h@page{\tcb@h@page+\tcb@temp}%
        \tcb@final@boxtrue%
      \fi%
    \fi%
  \else%
    \tcb@final@boxtrue%
  \fi%
}

\def\tcb@following@title{%
  \ifx\kvtcb@followingtitle\@empty%
    \tcb@hasTitlefalse%
    \let\tcb@h@title=\tcb@zpt%
    \let\tcb@h@padtitle=\tcb@zpt%
  \else%
    \tcb@hasTitletrue%
    \tcbdimto\tcb@w@title{\tcb@innerwidth-\kvtcb@boxsep*2-\kvtcb@lefttitle-\kvtcb@righttitle}%
    \begin{tcb@savebox}{\tcb@titlebox}{\tcb@w@title}\color{tcbcol@title}\kvtcb@fonttitle\kvtcb@followingtitle\end{tcb@savebox}%
    \tcbdimto\tcb@h@title{\ht\tcb@titlebox+\dp\tcb@titlebox}%
    \tcbdimto\tcb@h@padtitle{\kvtcb@title@rule+\kvtcb@boxsep*2+\kvtcb@toptitle+\kvtcb@bottomtitle+\tcb@h@title}%
  \fi%
}

\newbox\tcb@totalupperbox
\newbox\tcb@totallowerbox
\newif\iftcb@break@allowed

\def\tcb@enlbreak@next@final{%
  \ifdim\dimexpr\tcb@enlbreak@dim=0pt\relax
  \else%
    \iftcb@multicol\else\enlargethispage{\tcb@enlbreak@dim}\fi%
  \fi%
}

\def\tcb@enlbreak@next@scan#1/#2@{%
  \def\temp@a{#2}%
  \tcbdimto\tcb@enlbreak@dim{#1}%
  \ifx\temp@a\@empty%
    \let\tcb@enlbreak@next=\tcb@enlbreak@next@final%
  \else%
     \edef\tcb@enlbreak@seq{\temp@a @}%
  \fi%
  \tcb@enlbreak@next@final%
}

\def\tcb@enlbreak@next@step{%
  \edef\tcb@temp{\noexpand\tcb@enlbreak@next@scan\tcb@enlbreak@seq}%
  \tcb@temp%
}

\def\tcb@enlbreak@init{%
  \edef\tcb@enlbreak@seq{\kvtcb@enlargepage/@}%
  \let\tcb@enlbreak@next=\tcb@enlbreak@next@step%
  \tcb@enlbreak@next%
}


\def\tcb@breakat@next@scan#1/#2@{%
  \def\temp@a{#2}%
  \tcbdimto\tcb@breakat@dim{#1}%
  \ifx\temp@a\@empty%
    \let\tcb@breakat@next=\@empty%
  \else%
     \edef\tcb@breakat@seq{\temp@a @}%
  \fi%
}

\def\tcb@breakat@next@step{%
  \edef\tcb@temp{\noexpand\tcb@breakat@next@scan\tcb@breakat@seq}%
  \tcb@temp%
}

\def\tcb@breakat@init{%
  \edef\tcb@breakat@seq{\kvtcb@breakatdim/@}%
  \let\tcb@breakat@next=\tcb@breakat@next@step%
}


\newif\iftcb@multicol
\newif\iftcb@vfillbeforefirst

\def\tcb@do@nobreak@warning{%
  \iftcb@ignorenobreak%
    \tcb@warning{Using nobreak failed. You should set `ignore nobreak=false' to avoid this}%
  \else%
    \tcb@warning{Using nobreak failed. Try to enlarge `lines before break' or set page breaks manually}%
  \fi%
}

\def\tcb@handle@nobreak{%
  \tcb@enlbreak@init%
  \tcb@breakat@init%
  \tcb@comp@h@page%
  \tcbdimto\tcb@h@page{\tcb@h@page-1.5\baselineskip-\parskip-\lineskip}% security surcharge
  \tcb@comp@h@total@standalone%
  \tcb@check@for@final@box%
  \iftcb@final@box%
  \else%
    \ifdim\dimexpr\tcb@h@page-\tcb@h@padding-\tcb@h@padtitle<\kvtcb@breakminlines\baselineskip\relax%
      \tcbdimto\tcb@h@page{\tcb@h@page+3.5\baselineskip+\parskip+\lineskip}%
      \vspace{\tcb@h@page}%
      {\parskip\z@\nointerlineskip\noindent}%
      \vspace{-\tcb@h@page}%
      \par%
    \fi%
  \fi%
}

\def\tcb@prepare@break@operation{%
  \setcounter{tcbbreakpart}{0}%
  \let\tcb@nobreak@warning\@empty%
  \@ifundefined{columnbreak}{\tcb@multicolfalse}{%
    \ifnum\doublecol@number>\z@ %
      \tcb@multicoltrue%
    \else%
      \tcb@multicolfalse%
    \fi}%
  \ifx\kvtcb@float\@empty%
    \iftcb@nobreak{%
      \let\tcb@nobreak@warning\tcb@do@nobreak@warning%
      \iftcb@ignorenobreak%
        \kvtcb@beforebox%
      \else%
        \tcb@handle@nobreak%
      \fi%
    }{\kvtcb@beforebox}%
    \def\kvtcb@beforebox{\parskip\z@\nointerlineskip\noindent}%
    \noindent% applies parskip
    \vskip\lineskip{\parskip\z@\par\vskip\z@}\bgroup\@nobreakfalse\addpenalty\z@\egroup% force update vertical list
    \tcb@break@allowedtrue%
    \tcb@enlbreak@init%
  \else%
    \tcb@break@allowedfalse%
  \fi%
}

\def\tcb@height@fill@unbroken#1{%
  \tcb@prepare@break@operation%
  \tcb@breakat@init%
  \tcbset{compress page=#1}%
  \tcb@comp@h@page%
  \tcbset{height=\tcb@h@page-\kvtcb@bbtop@stand-\kvtcb@bbbottom@stand,after=\eject}%
}

\def\tcb@height@fill@unbroken@normal{\tcb@height@fill@unbroken{none}}
\def\tcb@height@fill@unbroken@compressed{\tcb@height@fill@unbroken{all}}

\def\tcb@use@after@lastbox{\bgroup\tcb@after@lastbox\egroup}

\def\tcb@drawcolorbox@breakable{%
  \tcb@prepare@break@operation%
  \global\let\tcb@after@lastbox=\kvtcb@afterbox%
  \let\kvtcb@afterbox=\@empty%
  \begingroup%
    \parskip\z@%
    \parindent\z@%
    \lineskip\z@%
    \topskip\z@%
    \tcb@split@start%
  \endgroup%
  \color{.}% hack for some special cases
  \ifx\kvtcb@float\@empty%
    \aftergroup\tcb@use@after@lastbox%
  \fi%
}

\def\tcb@split@start{%
  \tcb@breakat@init%
  \tcb@comp@h@page%
  % height calculation
  \tcb@comp@h@total@standalone%
  %
  \let\tcb@split@next=\relax%
  \tcb@check@for@final@box%
  \iftcb@final@box%
    \tcb@drawcolorbox@standalone%
  \else%
    \iftcb@break@allowed%
      \ifdim\dimexpr\tcb@h@page-\tcb@h@padding-\tcb@h@padtitle<\kvtcb@breakminlines\baselineskip\relax%
        \iftcb@multicol\columnbreak\else\pagebreak\fi%
        \tcb@nobreak@warning%
        \tcb@enlbreak@init\tcb@break@allowedfalse%
        \tcb@comp@h@page%
        \tcb@check@for@final@box%
        \iftcb@final@box%
          \tcb@drawcolorbox@standalone%
        \else%
          \let\tcb@split@next=\tcb@split@first%
        \fi%
      \else%
        \let\tcb@split@next=\tcb@split@first%
      \fi%
    \else%
      \let\tcb@split@next=\tcb@split@first%
    \fi%
  \fi%
  \tcb@split@next%
}


\def\tcb@setbox#1#2#3{%
  \setbox#1=\vbox{\unvbox#3}%
  \ifdim\dimexpr\ht#1+\dp#1>#2\relax%
    %\tcb@warning{Splitted box part too large by \the\dimexpr\ht#1+\dp#1-#2\relax}% switched off (99% useless/annoying)
    \setbox#1=\vbox to\the\dimexpr#2-\dp#1\relax{\unvbox#1}%
  \fi%
}


\def\tcb@setbox@upper#1#2{%
  \tcb@setbox\tcb@upperbox{#1}{#2}%
  \tcbdimto\tcb@h@upper{\ht\tcb@upperbox+\dp\tcb@upperbox}%
}


\def\tcb@split@upper@box@and@assemble{%
  \vfuzz=\maxdimen\vbadness=10000\savingvdiscards=1%
  \setbox\tcb@upperbox=\vsplit\tcb@totalupperbox to\tcb@split@dim%
  \edef\tcb@upper@box@badness{\the\badness}%
  \ifnum\tcb@upper@box@badness=1000000\relax%
    \setbox\tcb@totalupperbox=\vbox{%
      \unvbox\tcb@upperbox%
      \splitdiscards%
      \unvbox\tcb@totalupperbox}%
  \else%
    \tcb@setbox@upper{\tcb@split@dim}{\tcb@upperbox}%
  \fi%
  \vbadness=\tcb@thevbadness\vfuzz=\tcb@thevfuzz\savingvdiscards=0%
}


\def\tcb@split@upper@box{%
  \vfuzz=\maxdimen\vbadness=10000%
  \setbox\tcb@upperbox=\vsplit\tcb@totalupperbox to\tcb@split@dim%
  \edef\tcb@upper@box@badness{\the\badness}%
  \ifnum\tcb@upper@box@badness=1000000\relax%
    \tcb@warning{The upper box part has become overfull}%
  \fi%
  \tcb@setbox@upper{\tcb@split@dim}{\tcb@upperbox}%
  \vbadness=\tcb@thevbadness\vfuzz=\tcb@thevfuzz%
}


\def\tcb@setbox@lower#1#2{%
  \tcb@setbox\tcb@lowerbox{#1}{#2}%
  \tcbdimto\tcb@h@lower{\ht\tcb@lowerbox+\dp\tcb@lowerbox}%
}

\def\tcb@split@lower@box@and@assemble{%
  \vfuzz=\maxdimen\vbadness=10000\savingvdiscards=1%
  \setbox\tcb@lowerbox=\vsplit\tcb@totallowerbox to\tcb@split@dim%
  \edef\tcb@lower@box@badness{\the\badness}%
  \ifnum\tcb@lower@box@badness=1000000\relax%
    \setbox\tcb@totallowerbox=\vbox{%
      \unvbox\tcb@lowerbox%
      \splitdiscards%
      \unvbox\tcb@totallowerbox}%
  \else%
    \tcb@setbox@lower{\tcb@split@dim}{\tcb@lowerbox}%
  \fi%
  \vbadness=\tcb@thevbadness\vfuzz=\tcb@thevfuzz\savingvdiscards=0%
}


\def\tcb@split@lower@box{%
  \vfuzz=\maxdimen\vbadness=10000%
  \setbox\tcb@lowerbox=\vsplit\tcb@totallowerbox to\tcb@split@dim%
  \edef\tcb@lower@box@badness{\the\badness}%
  \ifnum\tcb@lower@box@badness=1000000\relax%
    \tcb@warning{The lower box part has become overfull}%
  \fi%
  \tcb@setbox@lower{\tcb@split@dim}{\tcb@lowerbox}%
  \vbadness=\tcb@thevbadness\vfuzz=\tcb@thevfuzz%
}


\def\tcb@split@setstate@first{%
  \edef\tcb@split@state{first}%
  \let\kvtcb@top@rule=\kvtcb@top@rule@stand%
  \let\kvtcb@bottom@rule=\kvtcb@bottom@rule@break%
  \let\kvtcb@bbtop=\kvtcb@bbtop@stand%
  \let\kvtcb@bbbottom=\kvtcb@bbbottom@break%
  \let\tcb@break@topsep=\tcb@zpt%
  \let\tcb@break@bottomsep=\kvtcb@bottomsep%
}

\def\tcb@split@setstate@middle{%
  \edef\tcb@split@state{middle}%
  \let\kvtcb@top@rule=\kvtcb@top@rule@break%
  \let\kvtcb@bottom@rule=\kvtcb@bottom@rule@break%
  \let\kvtcb@bbtop=\kvtcb@bbtop@break%
  \let\kvtcb@bbbottom=\kvtcb@bbbottom@break%
  \let\tcb@break@topsep=\kvtcb@topsep%
  \let\tcb@break@bottomsep=\kvtcb@bottomsep%
}

\def\tcb@split@setstate@last{%
  \edef\tcb@split@state{last}%
  \let\kvtcb@top@rule=\kvtcb@top@rule@break%
  \let\kvtcb@bottom@rule=\kvtcb@bottom@rule@stand%
  \let\kvtcb@bbtop=\kvtcb@bbtop@break%
  \let\kvtcb@bbbottom=\kvtcb@bbbottom@stand%
  \let\tcb@break@topsep=\kvtcb@topsep%
  \let\tcb@break@bottomsep=\tcb@zpt%
}


\def\tcb@split@force@standalone{%
  \tcb@comp@h@total@standalone%
  \ifdim\tcb@h@total>\tcb@h@page\relax%
    \tcbdimto\kvtcb@bbbottom@stand{\kvtcb@bbbottom@stand+\tcb@h@page-\tcb@h@total}%
  \fi%
}


\def\tcb@split@break@to@start{%
  \tcb@swap{\tcb@totalupperbox}{\tcb@upperbox}%
  \tcb@swap{\tcb@totallowerbox}{\tcb@lowerbox}%
  \tcbdimto\tcb@h@upper{\ht\tcb@upperbox+\dp\tcb@upperbox}%
  \tcbdimto\tcb@h@lower{\ht\tcb@lowerbox+\dp\tcb@lowerbox}%
  \iftcb@multicol\columnbreak\else\pagebreak\fi%
  \tcb@nobreak@warning%
  \tcb@enlbreak@init\tcb@break@allowedfalse%
  \let\tcb@split@next=\tcb@split@start%
}

\def\tcb@split@first{%
  \setcounter{tcbbreakpart}{1}%
  \ifx\kvtcb@float\@empty%
    \iftcb@vfillbeforefirst%
      \let\tcb@before@first=\vfill%
    \else%
    \let\tcb@before@first=\@empty%
    \fi%
    \let\tcb@before@middle=\@empty%
    \let\tcb@before@last=\@empty%
    \iftcb@multicol%
      \long\def\tcb@after@first{\par}% using \columnbreak here kills multicols' algortihm sometimes
      \long\def\tcb@after@middle{\par\vfill}%
    \else%
      \long\def\tcb@after@first{\par\pagebreak\tcb@enlbreak@next}%
      \long\def\tcb@after@middle{\par\vfill\eject\tcb@enlbreak@next}%
    \fi%
    \let\tcb@after@last=\par%
  \else%
    \edef\tcb@before@first{\noexpand\tcb@float@env@begin{tcbfloat}[\kvtcb@float]\noexpand\kvtcb@everyfloat}%
    \let\tcb@before@middle=\tcb@before@first%
    \let\tcb@before@last=\tcb@before@first%
    \let\tcb@after@first=\tcb@float@env@end%
    \let\tcb@after@middle=\tcb@float@env@end%
    \let\tcb@after@last=\tcb@float@env@end%
  \fi%
  %
  \edef\kvtcb@skin@@first{\kvtcb@skin@first}%
  \edef\kvtcb@skin@@middle{\kvtcb@skin@middle}%
  \edef\kvtcb@skin@@last{\kvtcb@skin@last}%
  %
  \let\tcb@h@breaksep@first=\kvtcb@bottomsep%
  \tcbdimto\tcb@h@breaksep@middle{\kvtcb@bottomsep+\kvtcb@topsep}%
  \let\tcb@h@breaksep@last=\kvtcb@topsep%
  \tcbdimto\tcb@h@padding@first{\kvtcb@bbtop@stand+\kvtcb@bbbottom@break+\kvtcb@top@rule@stand+\kvtcb@bottom@rule@break+\tcb@h@breaksep@first+\kvtcb@boxsep*2+\kvtcb@top+\kvtcb@bottom}%
  \tcbdimto\tcb@h@padding@middle{\kvtcb@bbtop@break+\kvtcb@bbbottom@break+\kvtcb@top@rule@break+\kvtcb@bottom@rule@break+\tcb@h@breaksep@middle+\kvtcb@boxsep*2+\kvtcb@top+\kvtcb@bottom}%
  \tcbdimto\tcb@h@padding@last{\kvtcb@bbtop@break+\kvtcb@bbbottom@stand+\kvtcb@top@rule@break+\kvtcb@bottom@rule@stand+\tcb@h@breaksep@last+\kvtcb@boxsep*2+\kvtcb@top+\kvtcb@bottom}%
  %
  \tcb@split@setstate@first%
  %
  \splittopskip=0pt%
  \splitmaxdepth=0pt%
  \edef\tcb@thevfuzz{\the\vfuzz}%
  \edef\tcb@thevbadness{\the\vbadness}%
  %
  \tcb@swap{\tcb@totalupperbox}{\tcb@upperbox}%
  \tcb@swap{\tcb@totallowerbox}{\tcb@lowerbox}%
  %
  \let\tcb@split@next=\relax%
  \tcbdimto\tcb@split@dim{\tcb@h@page-\tcb@h@padding@first-\tcb@h@padtitle}%
  \ifdim\tcb@split@dim<\tcb@h@upper\relax%
    %
    %
    \iftcb@break@allowed%
      \tcb@split@upper@box@and@assemble%
      \ifnum\tcb@upper@box@badness=1000000\relax%
        \tcb@split@break@to@start%
      \else%
        \ifdim\wd\tcb@totalupperbox=0pt\relax%
          \iftcb@lowerspace%
            \tcb@sdraw@U%
            \let\tcb@split@next=\tcb@split@SL%
          \else%
            \tcb@split@force@standalone%
            \tcb@drawcolorbox@standalone%
          \fi%
        \else%
          \ifdim\dimexpr\tcb@h@upper=0pt\relax%
            \tcb@split@break@to@start%
          \else%
            \tcb@sdraw@U%
            \let\tcb@split@next=\tcb@split@USL%
          \fi%
        \fi%
      \fi%
    \else%
      \tcb@split@upper@box%
      \ifdim\wd\tcb@totalupperbox=0pt\relax%
        \iftcb@lowerspace%
          \tcb@sdraw@U%
          \let\tcb@split@next=\tcb@split@SL%
        \else%
          \tcb@split@force@standalone%
          \tcb@drawcolorbox@standalone%
        \fi%
      \else%
        \tcb@sdraw@U%
        \let\tcb@split@next=\tcb@split@USL%
      \fi%
    \fi%
  \else%
    \tcb@swap{\tcb@totalupperbox}{\tcb@upperbox}%
    \iftcb@lowerspace%
      \tcbdimto\tcb@split@dim{\tcb@split@dim-\tcb@h@upper-\tcb@h@segment}%
      \ifdim\tcb@split@dim<\kvtcb@breakminlines\baselineskip\relax%
        \tcb@sdraw@U%
        \let\tcb@split@next=\tcb@split@SL%
      \else
        \tcb@split@lower@box@and@assemble%
        \ifnum\tcb@lower@box@badness=1000000\relax%
          \tcb@sdraw@U%
          \let\tcb@split@next=\tcb@split@SL%
        \else%
          \ifdim\wd\tcb@totallowerbox=0pt\relax%
            \tcb@split@force@standalone%
            \tcb@drawcolorbox@standalone%
          \else%
            \tcb@sdraw@USL%
            \let\tcb@split@next=\tcb@split@L%
          \fi%
        \fi%
      \fi%
    \else%
      \tcb@split@force@standalone%
      \tcb@drawcolorbox@standalone%
    \fi%
  \fi%
  \tcb@split@next%
}


\def\tcb@split@force@last{%
  \tcb@split@setstate@last%
  \ifdim\tcb@h@total>\tcb@h@page%
    \tcbdimto\kvtcb@bbbottom{\kvtcb@bbbottom+\tcb@h@page-\tcb@h@total}%
  \fi%
}

\def\tcb@nextbreakpart{%
  \stepcounter{tcbbreakpart}%
  \tcb@count@boxes%
  \iftcb@checkpage%
    \tcb@phantom@savepage%
    \tcb@hasPhantomtrue%
    \sbox\tcb@phantombox{\kvtcb@phantom}%
    \let\kvtcb@phantom\@empty%
  \fi%
  \tcb@following@title%
}


\def\tcb@split@USL{%
  \tcb@nextbreakpart%
  \tcb@comp@h@page%
  \tcb@defToTotalHeight\tcb@h@upper{\tcb@totalupperbox}%
  \tcbdimto\tcb@h@total{\tcb@h@padding@last+\tcb@h@padtitle+\tcb@h@upper+\tcb@h@segment+\tcb@h@lower}%
  %
  \let\tcb@split@next=\relax%
  \tcb@check@for@final@box%
  \iftcb@final@box%
    \tcb@split@setstate@last%
    \tcb@setbox@upper{\tcb@h@upper}{\tcb@totalupperbox}%
    \iftcb@lowerspace%
      \tcb@setbox@lower{\tcb@h@lower}{\tcb@totallowerbox}%
      \tcb@sdraw@USL%
    \else
      \tcb@sdraw@U%
    \fi%
  \else
    \tcb@split@setstate@middle%
    \tcbdimto\tcb@split@dim{\tcb@h@page-\tcb@h@padding@middle-\tcb@h@padtitle}%
    \ifdim\tcb@split@dim<\tcb@h@upper\relax%
      \tcb@split@upper@box%
      \ifdim\wd\tcb@totalupperbox=0pt\relax%
        \iftcb@lowerspace%
          \tcb@sdraw@U%
          \let\tcb@split@next=\tcb@split@SL%
        \else%
          \tcb@split@force@last%
          \tcb@sdraw@U%
        \fi%
      \else%
        \tcb@sdraw@U%
        \let\tcb@split@next=\tcb@split@USL%
      \fi%
    \else%
      \tcb@setbox@upper{\tcb@h@upper}{\tcb@totalupperbox}%
      \iftcb@lowerspace%
        \tcbdimto\tcb@split@dim{\tcb@split@dim-\tcb@h@upper-\tcb@h@segment}
        \ifdim\tcb@split@dim<\kvtcb@breakminlines\baselineskip\relax%
          \tcb@sdraw@U%
          \let\tcb@split@next=\tcb@split@SL%
        \else
          \tcb@split@lower@box@and@assemble%
          \ifnum\tcb@lower@box@badness=1000000\relax%
            \tcb@sdraw@U%
            \let\tcb@split@next=\tcb@split@SL%
          \else%
            \ifdim\wd\tcb@totallowerbox=0pt\relax%
              \tcb@split@force@last%
              \tcb@sdraw@USL%
            \else%
              \tcb@sdraw@USL%
              \let\tcb@split@next=\tcb@split@L%
            \fi%
          \fi%
        \fi%
      \else%
        \tcb@split@force@last%
        \tcb@sdraw@U%
      \fi%
    \fi%
  \fi%
  \tcb@split@next%
}


\def\tcb@split@SL{%
  \tcb@nextbreakpart%
  \tcb@comp@h@page%
  \let\tcb@h@upper=\tcb@zpt%
  \tcb@defToTotalHeight\tcb@h@lower{\tcb@totallowerbox}%
  \tcbdimto\tcb@h@total{\tcb@h@padding@last-\kvtcb@top-\kvtcb@boxsep+\tcb@h@padtitle+\tcb@h@segment+\tcb@h@lower}%
  %
  \let\tcb@split@next=\relax%
  \tcb@check@for@final@box%
  \iftcb@final@box%
    \tcb@split@setstate@last%
    \tcb@setbox@lower{\tcb@h@lower}{\tcb@totallowerbox}%
    \tcb@sdraw@SL%
  \else
    \tcb@split@setstate@middle%
    \tcbdimto\tcb@split@dim{\tcb@h@page-\tcb@h@padding@middle+\kvtcb@top+\kvtcb@boxsep-\tcb@h@padtitle-\tcb@h@segment}%
    \tcb@split@lower@box%
    \ifdim\wd\tcb@totallowerbox=0pt\relax%
      \tcb@split@force@last%
      \tcb@sdraw@SL%
    \else
      \tcb@sdraw@SL%
      \let\tcb@split@next=\tcb@split@L%
    \fi%
  \fi%
  \tcb@split@next%
}


\def\tcb@split@L{%
  \tcb@nextbreakpart%
  \tcb@comp@h@page%
  \let\tcb@h@upper=\tcb@zpt%
  \tcb@defToTotalHeight\tcb@h@lower{\tcb@totallowerbox}%
  \tcbdimto\tcb@h@total{\tcb@h@padding@last+\tcb@h@padtitle+\tcb@h@lower}%
  %
  \let\tcb@split@next=\relax%
  \tcb@check@for@final@box%
  \iftcb@final@box%
    \tcb@split@setstate@last%
    \tcb@setbox@lower{\tcb@h@lower}{\tcb@totallowerbox}%
    \tcb@sdraw@L%
  \else
    \tcb@split@setstate@middle%
    \tcbdimto\tcb@split@dim{\tcb@h@page-\tcb@h@padding@middle-\tcb@h@padtitle}%
    \tcb@split@lower@box%
    \ifdim\wd\tcb@totallowerbox=0pt\relax%
      \tcb@split@force@last%
      \tcb@sdraw@L%
    \else
      \tcb@sdraw@L%
      \let\tcb@split@next=\tcb@split@L%
    \fi%
  \fi%
  \tcb@split@next%
}


\def\tcb@break@ch@fixed{%
  \ifdim\tcb@natheight<\tcb@h@page\relax%
    \tcbdimto\kvtcb@height@fixed{\tcb@h@page-\kvtcb@bbtop-\kvtcb@bbbottom}%
    \tcb@ch@fixed%
  \else%
    \tcb@ch@natural%
  \fi%
}


\def\tcb@sdraw@USL{%
  \begingroup%
  \tcbset{skin=\csname kvtcb@skin@@\tcb@split@state\endcsname}%
  \csuse{tcb@extras@\tcb@split@state}%
  \tcb@afteroptions@hook%
  \def\tcb@segment@state{1}%
  \tcbdimto\tcb@natheight{\tcb@h@padtitle+\kvtcb@top@rule+\kvtcb@bottom@rule+\kvtcb@boxsep*2+\kvtcb@top+\kvtcb@bottom+\tcb@h@upper+\tcb@h@segment+\tcb@h@lower+\csname tcb@h@breaksep@\tcb@split@state\endcsname}%
  \csname tcb@break@ch@\tcb@split@state\endcsname%
  \tcbdimto\tcb@innerheight{\tcb@height-\kvtcb@top@rule-\kvtcb@bottom@rule-\tcb@h@padtitle}%
  \tcb@drawing@env@begin%
    \tcb@extensions@preframe%
     % draw frame and interior
    \tcb@adraw@frame%
    \tcb@adraw@interior%
    \iftcb@lowerseparated%
      \tcb@segmentation@code%
    \fi%
    \tcb@adraw@title%
    \tcb@extensions@postframe%
    % draw text boxes
    \tcb@tdraw@title%
    \tcb@tdraw@upper%
    \tcb@tdraw@lower%
    \tcb@extensions@final%
  \tcb@drawing@env@end%
  \endgroup%
}


\def\tcb@sdraw@U{%
  \begingroup%
  \tcbset{skin=\csname kvtcb@skin@@\tcb@split@state\endcsname}%
  \csuse{tcb@extras@\tcb@split@state}%
  \tcb@afteroptions@hook%
  \def\tcb@segment@state{0}%
  \tcbdimto\tcb@natheight{\tcb@h@padtitle+\kvtcb@top@rule+\kvtcb@bottom@rule+\kvtcb@boxsep*2+\kvtcb@top+\kvtcb@bottom+\tcb@h@upper+\csname tcb@h@breaksep@\tcb@split@state\endcsname}%
  \csname tcb@break@ch@\tcb@split@state\endcsname%
  \tcbdimto\tcb@innerheight{\tcb@height-\kvtcb@top@rule-\kvtcb@bottom@rule-\tcb@h@padtitle}%
  \tcb@drawing@env@begin%
    \tcb@extensions@preframe%
    % draw frame and interior
    \tcb@adraw@frame%
    \tcb@adraw@interior%
    \tcb@adraw@title%
    \tcb@extensions@postframe%
    % draw text boxes
    \tcb@tdraw@title%
    \tcb@tdraw@upper%
    \tcb@extensions@final%
  \tcb@drawing@env@end%
  \endgroup%
}


\def\tcb@sdraw@SL{%
  \begingroup%
  \tcbset{skin=\csname kvtcb@skin@@\tcb@split@state\endcsname}%
  \csuse{tcb@extras@\tcb@split@state}%
  \tcb@afteroptions@hook%
  \def\tcb@segment@state{1}%
  \tcbdimto\tcb@natheight{\tcb@h@padtitle+\kvtcb@top@rule+\kvtcb@bottom@rule+\kvtcb@bottom+\kvtcb@boxsep+\tcb@h@segment+\tcb@h@lower+\csname tcb@h@breaksep@\tcb@split@state\endcsname}%
  \csname tcb@break@ch@\tcb@split@state\endcsname%
  \tcbdimto\tcb@innerheight{\tcb@height-\kvtcb@top@rule-\kvtcb@bottom@rule-\tcb@h@padtitle}%
  \tcb@drawing@env@begin%
    \tcb@extensions@preframe%
    % draw frame and interior
    \tcb@adraw@frame%
    \tcb@adraw@interior%
    \iftcb@lowerseparated%
      \tcb@segmentation@code%
    \fi%
    \tcb@adraw@title%
    \tcb@extensions@postframe%
    % draw text boxes
    \tcb@tdraw@title%
    \tcb@tdraw@lower%
    \tcb@extensions@final%
  \tcb@drawing@env@end%
  \endgroup%
}


\def\tcb@sdraw@L{%
  \begingroup%
  \tcbset{skin=\csname kvtcb@skin@@\tcb@split@state\endcsname}%
  \csuse{tcb@extras@\tcb@split@state}%
  \tcb@afteroptions@hook%
  \def\tcb@segment@state{2}%
  \tcbdimto\tcb@natheight{\tcb@h@padtitle+\kvtcb@top@rule+\kvtcb@bottom@rule+\kvtcb@boxsep*2+\kvtcb@top+\kvtcb@bottom+\ht\tcb@lowerbox+\dp\tcb@lowerbox+\csname tcb@h@breaksep@\tcb@split@state\endcsname}%
  \csname tcb@break@ch@\tcb@split@state\endcsname%
  \tcbdimto\tcb@innerheight{\tcb@height-\kvtcb@top@rule-\kvtcb@bottom@rule-\tcb@h@padtitle}%
  \tcb@drawing@env@begin%
    \tcb@extensions@preframe%
    % draw frame and interior
    \tcb@adraw@frame%
    \tcb@adraw@interior%
    \tcb@adraw@title%
    \tcb@extensions@postframe%
    % draw text boxes
    \tcb@tdraw@title%
    \tcb@tdraw@lower%
    \tcb@extensions@final%
  \tcb@drawing@env@end%
  \endgroup%
}



\tcbset{%
  breakable@true/.code={%
    \let\tcb@savebox=\tcb@vbox%
    \let\endtcb@savebox=\endtcb@vbox%
    \let\tcb@defToTotalHeight=\tcb@defToTotalHeightBreakable%
    \let\tcb@drawcolorbox=\tcb@drawcolorbox@breakable},
  breakable@unlimited/.code={%
    \let\tcb@savebox=\tcb@vbox%
    \let\endtcb@savebox=\endtcb@vbox%
    \let\tcb@defToTotalHeight=\tcb@defToTotalHeightUnlimited%
    \let\tcb@drawcolorbox=\tcb@drawcolorbox@breakable},
  breakable/.style={breakable@#1},
  breakable/.default=true,%
  unbreakable/.style={breakable=false},%
  enforce breakable/.code={%
    \let\tcb@savebox=\tcb@vbox%
    \let\endtcb@savebox=\endtcb@vbox%
    \let\tcb@defToTotalHeight=\tcb@defToTotalHeightBreakable%
    \let\tcb@drawcolorbox=\tcb@drawcolorbox@breakable},
  title after break/.store in=\kvtcb@followingtitle,%
  notitle after break/.style={title after break=},%
  adjusted title after break/.style={title after break={#1\vphantom{\kvtcb@adjusttext}}},%
  lines before break/.store in=\kvtcb@breakminlines,%
  shrink break goal/.store in=\kvtcb@shrinkbreakgoal,%
  toprule at break/.store in=\kvtcb@top@rule@break,
  bottomrule at break/.store in=\kvtcb@bottom@rule@break,
  topsep at break/.store in=\kvtcb@topsep,%
  bottomsep at break/.store in=\kvtcb@bottomsep,%
  pad before break/.code={\let\kvtcb@bottom@rule@break=\tcb@zpt%
    \tcbdimto\kvtcb@bottomsep{#1-\kvtcb@bottom-\kvtcb@boxsep}},%
  pad before break*/.style={pad before break={#1},%
    code={\tcbdimto\tcb@temp{\kvtcb@bottom@rule@stand-\kvtcb@bottomsep}%
      \ifdim\tcb@temp>0pt\relax%
        \tcbdimto\kvtcb@enlargepage@flex{\kvtcb@enlargepage@flex+\tcb@temp}\fi}},%
  pad after break/.code={\let\kvtcb@top@rule@break=\tcb@zpt%
    \tcbdimto\kvtcb@topsep{#1-\kvtcb@top-\kvtcb@boxsep}},%
  pad at break/.style={pad before break={#1},pad after break={#1}},%
  pad at break*/.style={pad before break*={#1},pad after break={#1}},%
  enlargepage/.store in=\kvtcb@enlargepage,%
  enlargepage flexible/.store in=\kvtcb@enlargepage@flex,%
  break at/.store in=\kvtcb@breakatdim,%
  height fixed for/.is choice,%
  height fixed for/none/.code={%
    \let\tcb@break@ch@first=\tcb@ch@natural%
    \let\tcb@break@ch@middle=\tcb@ch@natural%
    \let\tcb@break@ch@last=\tcb@ch@natural},%
  height fixed for/first/.code={%
    \let\tcb@break@ch@first=\tcb@break@ch@fixed%
    \let\tcb@break@ch@middle=\tcb@ch@natural%
    \let\tcb@break@ch@last=\tcb@ch@natural},%
  height fixed for/middle/.code={%
    \let\tcb@break@ch@first=\tcb@ch@natural%
    \let\tcb@break@ch@middle=\tcb@break@ch@fixed%
    \let\tcb@break@ch@last=\tcb@ch@natural},%
  height fixed for/last/.code={%
    \let\tcb@break@ch@first=\tcb@ch@natural%
    \let\tcb@break@ch@middle=\tcb@ch@natural%
    \let\tcb@break@ch@last=\tcb@break@ch@fixed},%
  height fixed for/first and middle/.code={%
    \let\tcb@break@ch@first=\tcb@break@ch@fixed%
    \let\tcb@break@ch@middle=\tcb@break@ch@fixed%
    \let\tcb@break@ch@last=\tcb@ch@natural},%
  height fixed for/middle and last/.code={%
    \let\tcb@break@ch@first=\tcb@ch@natural%
    \let\tcb@break@ch@middle=\tcb@break@ch@fixed%
    \let\tcb@break@ch@last=\tcb@break@ch@fixed},%
  height fixed for/all/.code={%
    \let\tcb@break@ch@first=\tcb@break@ch@fixed%
    \let\tcb@break@ch@middle=\tcb@break@ch@fixed%
    \let\tcb@break@ch@last=\tcb@break@ch@fixed},%
  vfill before first/.is if=tcb@vfillbeforefirst,%
  height fill/true/.code={\let\tcb@height@adjust\tcb@height@fill@unbroken@normal},%
  height fill/maximum/.code={\let\tcb@height@adjust\tcb@height@fill@unbroken@compressed},%
  height fill/.default=true,%
  compress page/.is choice,%
  compress page/all/.code={\def\tcb@comp@compress{\def\tcb@compress@height{\pageshrink-1sp}}},%
  compress page/none/.code={\def\tcb@comp@compress{\let\tcb@compress@height\tcb@zpt}},%
  compress page/baselineskip/.code={\def\tcb@comp@compress{%
    \ifdim\pageshrink>\baselineskip%
      \let\tcb@compress@height\baselineskip%
    \else%
      \def\tcb@compress@height{\pageshrink-1sp}%
    \fi}},%
  compress page/.default=all,%
  compress page=baselineskip,% global setting
  extras unbroken/.code={\appto\tcb@extras@unbroken{\tcbset{#1}}},%
  extras first/.code={\appto\tcb@extras@first{\tcbset{#1}}},%
  extras middle/.code={\appto\tcb@extras@middle{\tcbset{#1}}},%
  extras last/.code={\appto\tcb@extras@last{\tcbset{#1}}},%
  extras/.style={extras unbroken={#1},extras first={#1},extras middle={#1},extras last={#1}},%
  extras broken/.style={extras first={#1},extras middle={#1},extras last={#1}},%
  extras unbroken and first/.style={extras unbroken={#1},extras first={#1}},%
  extras unbroken and last/.style={extras unbroken={#1},extras last={#1}},%
  extras middle and last/.style={extras middle={#1},extras last={#1}},%
  extras first and middle/.style={extras first={#1},extras middle={#1}},%
  no extras unbroken/.code={\let\tcb@extras@unbroken\@empty},%
  no extras first/.code={\let\tcb@extras@first\@empty},%
  no extras middle/.code={\let\tcb@extras@middle\@empty},%
  no extras last/.code={\let\tcb@extras@last\@empty},%
  no extras/.code={\let\tcb@extras@unbroken\@empty\let\tcb@extras@first\@empty\let\tcb@extras@middle\@empty\let\tcb@extras@last\@empty},%
  if odd page*/.style 2 args={check odd page,extras={if odd page={#1}{#2}}},%
}


\tcbset{%
  reset@breakable/.style={%
    unbreakable,notitle after break,
    shrink break goal=0pt,
    lines before break=2,
    topsep at break=0pt,
    bottomsep at break=0pt,
    enlargepage=0pt,enlargepage flexible=0pt,
    break at=0pt,
    height fixed for=none,
    vfill before first=false,
    no extras,
  },
  initialize@reset=reset@breakable,
}


==> tcbdocumentation.code.tex <==
%% The LaTeX package tcolorbox - version 3.80 (2015/11/27)
%% tcbdocumentation.code.tex: Code for LaTeX documentations
%%
%% -------------------------------------------------------------------------------------------
%% Copyright (c) 2006-2015 by Prof. Dr. Dr. Thomas F. Sturm <thomas dot sturm at unibw dot de>
%% -------------------------------------------------------------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2005/12/01 or later.
%%
%% This work has the LPPL maintenance status `author-maintained'.
%%
%% This work consists of all files listed in README
%%
\tcb@set@library@version{3.80}

\tcbuselibrary{listings,skins,xparse,external}

\RequirePackage{pifont}[2005/04/12]
\RequirePackage{marvosym}[2011/07/20]
\ifdefined\printindex\else\RequirePackage{makeidx}[2000/03/29]\fi
\RequirePackage{refcount}[2011/10/16]
\RequirePackage{hyperref}[2012/02/06]
\ifdefined\marginnote\else\RequirePackage{marginnote}[2012/03/29]\fi

\definecolor{Option}{rgb}{0.118,0.546,0.222}
\definecolor{Definition}{rgb}{0.784,0.06,0.176}
\definecolor{ExampleFrame}{rgb}{0.628,0.705,0.942}
\definecolor{ExampleBack}{rgb}{0.963,0.971,0.994}
\definecolor{Hyperlink}{rgb}{0.281,0.275,0.485}

\def\colDef#1{\textcolor{\kvtcb@col@command}{#1}}
\def\colOpt#1{\textcolor{\kvtcb@col@opt}{#1}}

\lstdefinestyle{tcbdocumentation}{language={[LaTeX]TeX},
    aboveskip={0\p@ \@plus 6\p@},
    belowskip={0\p@ \@plus 6\p@},
    columns=fullflexible,
    keepspaces=true,
    breaklines=true,
    prebreak={\Righttorque},
    postbreak={\space\Lefttorque},
    breakatwhitespace=true,
    basicstyle=\ttfamily\footnotesize,
    extendedchars=true,
    moredelim={[is][\itshape\rmfamily]{^^a7}{^^a7}},
    nolol,inputencoding=\kvtcb@listingencoding}

% The following macros are taken from ltxdoc
\DeclareRobustCommand\cs[1]{\texttt{\char`\\#1}}
\def\meta@font@select{\rmfamily\itshape}

\AtEndPreamble{%
  \@ifpackageloaded{doc}{%
  }{% code taken from doc.sty
    \ifx\l@nohyphenation\undefined
      \newlanguage\l@nohyphenation
    \fi
    \DeclareRobustCommand\meta[1]{%
         \ensuremath\langle
         \ifmmode \expandafter \nfss@text \fi
         {%
          \meta@font@select
          \edef\meta@hyphen@restore
            {\hyphenchar\the\font\the\hyphenchar\font}%
          \hyphenchar\font\m@ne
          \language\l@nohyphenation
          #1\/%
          \meta@hyphen@restore
         }\ensuremath\rangle
    }%
  }%
}%

\def\marg#1{%
  {\ttfamily\char`\{}\meta{#1}{\ttfamily\char`\}}}
\def\oarg#1{%
  \colOpt{{\ttfamily[}\meta{#1}{\ttfamily]}}}

\newrobustcmd\tcb@cs[1]{{\catcode`\_=12\relax\catcode`\@11\relax\ttfamily\char`\\\scantokens{#1}\unskip}}
\newrobustcmd\tcb@scantokens[1]{{\catcode`\_=12\relax\catcode`\@11\relax\ttfamily\scantokens{#1}\unskip}}

\newif\iftcb@doc@toindex
\newif\iftcb@doc@colorize
\newif\iftcb@doc@annotate

% language specific texts
\tcbset{
  doclang/.cd,
  color/.store in=\kvtcb@text@color,
  colors/.store in=\kvtcb@text@colors,
  counter/.store in=\kvtcb@text@counter,
  counters/.store in=\kvtcb@text@counters,
  environment content/.store in=\kvtcb@text@envcontent,
  environment/.store in=\kvtcb@text@env,
  environments/.store in=\kvtcb@text@envs,
  index/.store in=\kvtcb@text@index,
  key/.store in=\kvtcb@text@key,
  keys/.store in=\kvtcb@text@keys,
  length/.store in=\kvtcb@text@length,
  lengths/.store in=\kvtcb@text@lengths,
  new/.store in=\kvtcb@text@new,
  pageshort/.store in=\kvtcb@text@pageshort,
  updated/.store in=\kvtcb@text@updated,
  value/.store in=\kvtcb@text@value,
  values/.store in=\kvtcb@text@values,
}

% documentation options
\tcbset{
  documentation listing options/.store in=\kvtcb@doclistingoptions,%
  documentation listing style/.style={documentation listing options={style=#1}},%
  documentation minted style/.store in=\kvtcb@docmintstyle,
  documentation minted options/.store in=\kvtcb@docmintoptions,
  color command/.store in=\kvtcb@col@command,
  color environment/.store in=\kvtcb@col@environment,
  color key/.store in=\kvtcb@col@key,
  color value/.store in=\kvtcb@col@value,
  color counter/.store in=\kvtcb@col@counter,
  color length/.store in=\kvtcb@col@length,
  color color/.store in=\kvtcb@col@color,
  color definition/.style={color command={#1},color environment={#1},color key={#1},
    color value={#1},color color={#1},color counter={#1},color length={#1}},
  color option/.store in=\kvtcb@col@opt,
  color hyperlink/.store in=\kvtcb@colhyper,
  color frame/.store in=\kvtcb@colhyper,
  index actual/.store in=\idx@actual,
  index quote/.store in=\idx@quote,
  index level/.store in=\idx@level,
  index format/.store in=\idx@format,
  index colorize/.is if=tcb@doc@colorize,%
  index annotate/.is if=tcb@doc@annotate,%
  index command/.code={\def\kvtcb@index@command##1{#1{##1}}},%
  index command name/.code={\def\kvtcb@index@command##1{\index[#1]{##1}}},%
  doc left/.dimstore in=\kvtcb@doc@left,
  doc right/.dimstore in=\kvtcb@doc@right,
  doc left indent/.dimstore in=\kvtcb@doc@indentleft,
  doc right indent/.dimstore in=\kvtcb@doc@indentright,
  doc head command/.style={doc@head@command/.style={#1}},
  doc head environment/.style={doc@head@environment/.style={#1}},
  doc head key/.style={doc@head@key/.style={#1}},
  doc head/.style={doc head command={#1},doc head environment={#1},doc head key={#1}},
  before doc body command/.store in=\kvtcb@doc@body@command@before,
  after doc body command/.store in=\kvtcb@doc@body@command@after,
  before doc body environment/.store in=\kvtcb@doc@body@environment@before,
  after doc body environment/.store in=\kvtcb@doc@body@environment@after,
  before doc body key/.store in=\kvtcb@doc@body@key@before,
  after doc body key/.store in=\kvtcb@doc@body@key@after,
  before doc body/.style={before doc body command={#1},before doc body environment={#1},before doc body key={#1}},
  after doc body/.style={after doc body command={#1},after doc body environment={#1},after doc body key={#1}},
  doc description/.store in=\kvtcb@doc@description,%
  doc into index/.is if=tcb@doc@toindex,%
  doc updated/.style={before upper={\tcbdocmarginnote{\tcbdocupdated{#1}}}},
  doc new/.style={before upper={\tcbdocmarginnote{\tcbdocnew{#1}}}},
  doc new and updated/.style 2 args={before upper={\tcbdocmarginnote{\tcbdocnew{#1}\\\tcbdocupdated{#2}}}},
  doc marginnote/.style={doc@marginnote/.style={#1}},
}


% styles
\tcbset{
  docexample/.style={colframe=ExampleFrame,colback=ExampleBack,
    before skip=\medskipamount,after skip=\medskipamount,
    fontlower=\footnotesize},
  documentation minted style=,
  documentation minted options={tabsize=2,fontsize=\small},
  index default settings/.style={index actual={@},index quote={"},index level={!}},
  index german settings/.style={index actual={=},index quote={!},index level={>}},
  english language/.code={\tcbset{doclang/.cd,
    color=color,colors=Colors,
    counter=counter,counters=Counters,
    environment content=environment content,
    environment=environment,environments=Environments,
    index=Index,
    key=key,keys=Keys,
    length=length,lengths=Lengths,
    new=New,
    pageshort={P.},
    updated=Updated,
    value=value,values=Values}},
}

\AtBeginDocument{%
  \csname tcb@doc@index@\idx@format\endcsname%
  \hypersetup{
  citecolor=\kvtcb@colhyper,
  linkcolor=\kvtcb@colhyper,
  urlcolor=\kvtcb@colhyper,
  filecolor=\kvtcb@colhyper,
  menucolor=\kvtcb@colhyper
}}

\def\dispExample{\tcb@layer@pushup\tcbset{docexample}\begingroup\tcbwritetemp}

\def\enddispExample{%
  \endtcbwritetemp\endgroup%
  \begin{tcolorbox}%
  \tcb@doc@usetemplisting%
  \tcblower%
  \tcbusetemp%
  \end{tcolorbox}%
}

\newenvironment{dispExample*}[1]{%
  \tcb@layer@pushup\tcbset{docexample,#1}\begingroup\tcbwritetemp%
  }{\enddispExample}

\def\dispListing{\tcb@layer@pushup\tcbset{docexample}\begingroup\tcbwritetemp}

\def\enddispListing{%
  \endtcbwritetemp\endgroup%
  \begin{tcolorbox}%
  \tcb@doc@usetemplisting%
  \end{tcolorbox}%
}

\newenvironment{dispListing*}[1]{%
  \tcb@layer@pushup\tcbset{docexample,#1}\begingroup\tcbwritetemp%
  }{\enddispListing}

% index auxiliary macros
\def\tcb@Index@Print@CA#1#2#3{%
  \iftcb@doc@colorize\textcolor{#2}{\tcb@scantokens{#1}}\else\tcb@scantokens{#1}\fi%
  \iftcb@doc@annotate\ #3\fi%
}

\def\tcb@Index@Print@C#1#2{%
  \iftcb@doc@colorize\textcolor{#2}{\tcb@scantokens{#1}}\else\tcb@scantokens{#1}\fi%
}

\def\tcb@Index@Print@ComCA#1#2#3{%
  \iftcb@doc@colorize\textcolor{#2}{\tcb@cs{#1}}\else\tcb@cs{#1}\fi%
  \iftcb@doc@annotate\ #3\fi%
}

\def\tcb@Index@Print@ComC#1#2{%
  \iftcb@doc@colorize\textcolor{#2}{\tcb@cs{#1}}\else\tcb@cs{#1}\fi%
}

\newrobustcmd{\tcbIndexPrintComC}[1]{\tcb@Index@Print@ComC{#1}{\kvtcb@col@command}}
\def\tcb@Print@Com#1{\textcolor{\kvtcb@col@command}{\bfseries\tcb@cs{#1}}}

\newrobustcmd{\tcbIndexPrintEnvCA}[1]{\tcb@Index@Print@CA{#1}{\kvtcb@col@environment}{\kvtcb@text@env}}
\newrobustcmd{\tcbIndexPrintEnvC}[1]{\tcb@Index@Print@C{#1}{\kvtcb@col@environment}}
\def\tcb@Print@Env#1{\textcolor{\kvtcb@col@environment}{\bfseries\tcb@scantokens{#1}}}

\newrobustcmd{\tcbIndexPrintKeyCA}[1]{\tcb@Index@Print@CA{#1}{\kvtcb@col@key}{\kvtcb@text@key}}
\newrobustcmd{\tcbIndexPrintKeyC}[1]{\tcb@Index@Print@C{#1}{\kvtcb@col@key}}
\def\tcb@Print@Key#1{\textcolor{\kvtcb@col@key}{\bfseries\tcb@scantokens{#1}}}

\newrobustcmd{\tcbIndexPrintValCA}[1]{\tcb@Index@Print@CA{#1}{\kvtcb@col@value}{\kvtcb@text@value}}
\newrobustcmd{\tcbIndexPrintValC}[1]{\tcb@Index@Print@C{#1}{\kvtcb@col@value}}
\def\tcb@Print@Val#1{\textcolor{\kvtcb@col@value}{\bfseries\tcb@scantokens{#1}}}

\newrobustcmd{\tcbIndexPrintColCA}[1]{\tcb@Index@Print@CA{#1}{\kvtcb@col@color}{\kvtcb@text@color}}
\newrobustcmd{\tcbIndexPrintColC}[1]{\tcb@Index@Print@C{#1}{\kvtcb@col@color}}
\def\tcb@Print@Col#1{\textcolor{\kvtcb@col@color}{\bfseries\tcb@scantokens{#1}}}

\newrobustcmd{\tcbIndexPrintCountCA}[1]{\tcb@Index@Print@CA{#1}{\kvtcb@col@counter}{\kvtcb@text@counter}}
\newrobustcmd{\tcbIndexPrintCountC}[1]{\tcb@Index@Print@C{#1}{\kvtcb@col@counter}}
\def\tcb@Print@Count#1{\textcolor{\kvtcb@col@counter}{\bfseries\tcb@scantokens{#1}}}

\newrobustcmd{\tcbIndexPrintLenCA}[1]{\tcb@Index@Print@ComCA{#1}{\kvtcb@col@length}{\kvtcb@text@length}}
\newrobustcmd{\tcbIndexPrintLenC}[1]{\tcb@Index@Print@ComC{#1}{\kvtcb@col@length}}
\def\tcb@Print@Len#1{\textcolor{\kvtcb@col@length}{\bfseries\tcb@cs{#1}}}

\def\tcb@index@Com#1{\iftcb@doc@toindex\kvtcb@index@command{#1\idx@actual\tcbIndexPrintComC{#1}}\fi}
\def\tcb@index@Env#1{\iftcb@doc@toindex\kvtcb@index@command{#1\idx@actual\tcbIndexPrintEnvCA{#1}}\kvtcb@index@command{\kvtcb@text@envs\idx@level#1\idx@actual\tcbIndexPrintEnvC{#1}}\fi}
\def\tcb@index@Key#1{\iftcb@doc@toindex\kvtcb@index@command{#1\idx@actual\tcbIndexPrintKeyCA{#1}}\kvtcb@index@command{\kvtcb@text@keys\idx@level#1\idx@actual\tcbIndexPrintKeyC{#1}}\fi}%
\def\tcb@index@KeyPath#1#2{\iftcb@doc@toindex\kvtcb@index@command{#2\idx@actual\tcbIndexPrintKeyCA{#2}}\kvtcb@index@command{\kvtcb@text@keys\idx@level#1\idx@actual\tcbIndexPrintKeyC{/#1/}\idx@level#2\idx@actual\tcbIndexPrintKeyC{#2}}\fi}%
\def\tcb@index@Val#1{\iftcb@doc@toindex\kvtcb@index@command{#1\idx@actual\tcbIndexPrintValCA{#1}}\kvtcb@index@command{\kvtcb@text@values\idx@level#1\idx@actual\tcbIndexPrintValC{#1}}\fi}
\def\tcb@index@Col#1{\iftcb@doc@toindex\kvtcb@index@command{#1\idx@actual\tcbIndexPrintColCA{#1}}\kvtcb@index@command{\kvtcb@text@colors\idx@level#1\idx@actual\tcbIndexPrintColC{#1}}\fi}
\def\tcb@index@Count#1{\iftcb@doc@toindex\kvtcb@index@command{#1\idx@actual\tcbIndexPrintCountCA{#1}}\kvtcb@index@command{\kvtcb@text@counters\idx@level#1\idx@actual\tcbIndexPrintCountC{#1}}\fi}
\def\tcb@index@Len#1{\iftcb@doc@toindex\kvtcb@index@command{#1\idx@actual\tcbIndexPrintLenCA{#1}}\kvtcb@index@command{\kvtcb@text@lengths\idx@level#1\idx@actual\tcbIndexPrintLenC{#1}}\fi}

\def\brackets#1{{\ttfamily\char`\{}#1{\ttfamily\char`\}}}

\newenvironment{tcb@manual@entry}{\begin{list}{}{%
  \setlength{\leftmargin}{\kvtcb@doc@left}%
  \setlength{\itemindent}{0pt}%
  \setlength{\itemsep}{0pt}%
  \setlength{\parsep}{0pt}%
  \setlength{\rightmargin}{\kvtcb@doc@right}%
  }\item}{\end{list}}

\def\tcb@manual@top#1{\itemsep=0pt\parskip=0pt\item\strut{#1}\par\topsep=0pt}

\def\tcb@doc@do@description{%
  \ifx\kvtcb@doc@description\@empty\else\tcblower\raggedleft(\kvtcb@doc@description)\fi%
}

\newtcolorbox{tcb@doc@head}[1]{blank,colback=white,colframe=white,
  code={\tcbdimto\tcb@temp@grow@left{-\kvtcb@doc@indentleft}%
        \tcbdimto\tcb@temp@grow@right{-\kvtcb@doc@indentright}},
  grow to left by=\tcb@temp@grow@left,%
  grow to right by=\tcb@temp@grow@right,
  sidebyside,sidebyside align=top,
  sidebyside gap=-\tcb@w@upper@real,
  phantom=\phantomsection,%
  enlarge bottom by=-0.2\baselineskip,#1}

% main documentation environments
\newenvironment{docCommand}[3][]{\tcbset{#1}%
  \begin{tcb@manual@entry}%
  \begin{tcb@doc@head}{doc@head@command}%
  \tcb@Print@Com{#2}\tcb@index@Com{#2}\protected@edef\@currentlabel{\noexpand\tcb@cs{#2}}\label{com:#2}{\ttfamily #3}%
  \tcb@doc@do@description%
  \end{tcb@doc@head}\tcbset{before upper=}\kvtcb@doc@body@command@before}%
  {\kvtcb@doc@body@command@after\end{tcb@manual@entry}}

\newenvironment{docCommand*}{\bgroup\tcb@doc@toindexfalse\begin{docCommand}}{\end{docCommand}\egroup}

\newenvironment{docEnvironment}[3][]{\tcbset{#1}%
  \begin{tcb@manual@entry}%
  \begin{tcb@doc@head}{doc@head@environment}%
  \strut\cs{begin}\brackets{\tcb@Print@Env{#2}}\tcb@index@Env{#2}\protected@edef\@currentlabel{#2}\label{env:#2}{\ttfamily #3}\par%
  \strut~~\meta{\kvtcb@text@envcontent}\par%
  \strut\cs{end}\brackets{\tcb@Print@Env{#2}}%
  \tcb@doc@do@description%
  \end{tcb@doc@head}\tcbset{before upper=}\kvtcb@doc@body@environment@before}%
  {\kvtcb@doc@body@environment@after\end{tcb@manual@entry}}

\newenvironment{docEnvironment*}{\bgroup\tcb@doc@toindexfalse\begin{docEnvironment}}{\end{docEnvironment}\egroup}

\NewDocumentEnvironment{docKey}{ O{} +O{} m m +m }{\tcbset{#2,doc description={#5}}%
  \begin{tcb@manual@entry}%
  \begin{tcb@doc@head}{doc@head@key}%
  \ifblank{#1}{%
    \tcb@Print@Key{#3}\tcb@index@Key{#3}\protected@edef\@currentlabel{#3}\label{key:#3}{\ttfamily #4}%
  }{%
    \tcb@Print@Key{/#1/#3}%
    \tcb@index@KeyPath{#1}{#3}\protected@edef\@currentlabel{/#1/#3}\label{key:/#1/#3}{\ttfamily #4}%
  }%
  \tcb@doc@do@description%
  \end{tcb@doc@head}\tcbset{before upper=}\kvtcb@doc@body@key@before}%
  {\kvtcb@doc@body@key@after\end{tcb@manual@entry}}

\newenvironment{docKey*}{\bgroup\tcb@doc@toindexfalse\begin{docKey}}{\end{docKey}\egroup}

\def\tcbmakedocSubKey#1#2{%
  \NewDocumentEnvironment{#1}{ O{} +O{} m m +m }{%
    \ifblank{##1}{\def\tcb@key@path{#2}}{\def\tcb@key@path{#2/##1}}%
    \begin{docKey}[\tcb@key@path][##2]{##3}{##4}{##5}}%
      {\end{docKey}}%
  \newenvironment{#1*}{\bgroup\tcb@doc@toindexfalse\begin{#1}}{\end{#1}\egroup}%
}

\DeclareDocumentCommand\docAuxCommand{sm}{%
  \tcb@Print@Com{#2}%
  \IfBooleanTF{#1}{}{\tcb@index@Com{#2}}%
}

\DeclareDocumentCommand\docAuxEnvironment{sm}{%
  \tcb@Print@Env{#2}%
  \IfBooleanTF{#1}{}{\tcb@index@Env{#2}}%
}

\DeclareDocumentCommand\docAuxKey{sO{}m}{%
  \ifblank{#2}{%
    \tcb@Print@Key{#3}%
    \IfBooleanTF{#1}{}{\tcb@index@Key{#3}}%
  }{%
    \tcb@Print@Key{/#2/#3}%
    \IfBooleanTF{#1}{}{\tcb@index@KeyPath{#2}{#3}}%
}}

\DeclareDocumentCommand\docColor{sm}{%
  \tcb@Print@Col{#2}%
  \IfBooleanTF{#1}{}{\tcb@index@Col{#2}}%
}

\DeclareDocumentCommand\docCounter{sm}{%
  \tcb@Print@Count{#2}%
  \IfBooleanTF{#1}{}{\tcb@index@Count{#2}}%
}

\DeclareDocumentCommand\docLength{sm}{%
  \tcb@Print@Len{#2}%
  \IfBooleanTF{#1}{}{\tcb@index@Len{#2}}%
}

\DeclareDocumentCommand\docValue{sm}{%
  \tcb@Print@Val{#2}%
  \IfBooleanTF{#1}{}{\tcb@index@Val{#2}}%
}

\setrefcountdefault{-1}
\DeclareDocumentCommand\tcb@ref@doc{msm}{%
  \hyperref[#1:#3]{\texttt{\ref*{#1:#3}}%
  \IfBooleanTF{#2}{}{%
    \ifnum\getpagerefnumber{#1:#3}=\thepage%
    \else%
      \textsuperscript{\ding{213}\,\kvtcb@text@pageshort\,\pageref*{#1:#3}}%
    \fi}}%
}

\def\refCom{\tcb@ref@doc{com}}
\def\refEnv{\tcb@ref@doc{env}}
\def\refKey{\tcb@ref@doc{key}}

\def\refAux#1{\textcolor{\kvtcb@colhyper}{\tcb@scantokens{#1}}}
\def\refAuxcs#1{\textcolor{\kvtcb@colhyper}{\tcb@cs{#1}}}

\newenvironment{absquote}
               {\list{}{\leftmargin2cm\rightmargin\leftmargin}%
                \item\relax\footnotesize}
               {\endlist}

\newcommand{\tcbdocmarginnote}[2][]{%
  \marginnote{%
  \begin{tcolorbox}[enhanced jigsaw,size=fbox,boxrule=1pt,leftrule=0pt,rightrule=0pt,
    arc=0pt,outer arc=1pt,boxsep=1pt,top=1pt,bottom=1pt,
    nobeforeafter,width=\marginparwidth,
    colframe=red!50!white,colback=red!25!yellow!5!white,fontupper=\scriptsize,before upper=\flushright,
    doc@marginnote,#1]#2\end{tcolorbox}}}

\newcommand*{\tcbdocnew}[1]{\kvtcb@text@new: #1}
\newcommand*{\tcbdocupdated}[1]{\kvtcb@text@updated: #1}

%--- index macros taken from pgfmanual-en-macros
\def\tcb@doc@index@pgf@{%
  \ifdefined\c@IndexColumns%
    \c@IndexColumns=2%
  \fi%
  \def\theindex{\@restonecoltrue
    \columnseprule \z@  \columnsep 29\p@
    \twocolumn[\index@prologue]%
    \parindent -30pt%
    \columnsep 15pt%
    \parskip 0pt plus 1pt%
    \leftskip 30pt%
    \rightskip 0pt plus 2cm%
    \small%
    \def\@idxitem{\par}%
    \let\item\@idxitem\ignorespaces}
  \def\endtheindex{\onecolumn}%
  \def\noindexing{\let\index=\@gobble}%
}

\def\tcb@doc@index@pgfsection{%
  \def\index@prologue{\section*{\kvtcb@text@index}\addcontentsline{toc}{section}{\kvtcb@text@index}%
    \par\noindent%
  }%
  \tcb@doc@index@pgf@%
}

\def\tcb@doc@index@pgfchapter{%
  \def\index@prologue{\ifdefined\phantomsection\phantomsection\fi\@makeschapterhead{\kvtcb@text@index}\addcontentsline{toc}{chapter}{\kvtcb@text@index}}%
  \tcb@doc@index@pgf@%
}

\let\tcb@doc@index@pgf=\tcb@doc@index@pgfsection%

\def\tcb@doc@index@doc{%
  \let\tcb@index@Com=\SpecialMainIndex%%
  \let\tcb@index@Env=\SpecialMainEnvIndex%
  \tcbset{index german settings}%
  \EnableCrossrefs%
  \PageIndex%
}

\def\tcb@doc@index@off{}%

\tcbset{%
  reset@documentation/.style={%
    index command=\index,%
    index format=pgf,
    english language,
    documentation listing style=tcbdocumentation,
    index default settings,
    color option=Option,
    color definition=Definition,
    color hyperlink=Hyperlink,
    doc left=2em,
    doc right=0pt,
    doc left indent=-2em,
    doc right indent=0pt,
    doc head=,
    before doc body=,
    after doc body=,
    doc description=,
    doc into index=true,
    index colorize=false,
    index annotate=true,
    doc marginnote=,
    },
  initialize@reset=reset@documentation,
}

% deprecated
\tcbset{
  before example/.store in=\kvtcb@beforeexample,
  after example/.store in=\kvtcb@afterexample,
    before example=\par\smallskip,
    after example=,
}


==> tcbexternal.code.tex <==
%% The LaTeX package tcolorbox - version 3.80 (2015/11/27)
%% tcbexternal.code.tex: Code for externalization
%%
%% -------------------------------------------------------------------------------------------
%% Copyright (c) 2006-2015 by Prof. Dr. Dr. Thomas F. Sturm <thomas dot sturm at unibw dot de>
%% -------------------------------------------------------------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2005/12/01 or later.
%%
%% This work has the LPPL maintenance status `author-maintained'.
%%
%% This work consists of all files listed in README
%%
\tcb@set@library@version{3.80}

{
\catcode`\"=12
\xdef\tcbexternal@normal@dq{"}
\catcode`\"=13
\gdef\tcbexternal@activate@normal@dq{\let"=\tcbexternal@normal@dq}
}

\long\def\tcbifexternal#1#2{%
  \ifdefined\TCBEXTERNALINPUT%
    #1%
  \else%
    #2%
  \fi%
}

\tcbifexternal{%
  \def\tcbEXTERNALIZE{%
    \RequirePackage{incgraph}%
    \TCBEXTERNALPREAMBLE%
    \begin{document}%
    \begin{inctext}[border=\TCBEXTERNALSAFETY]%
    \input{\TCBEXTERNALINPUT}%
    \end{inctext}%
    \end{document}%
  }%
}{%
  \def\tcbEXTERNALIZE{%
    \tcbset{
      external/.cd,
      externalize/.is if=tcb@externalize,
      externalize=true,
    }%
  }%
}

\@onlypreamble\tcbEXTERNALIZE

\def\tcbexternal@setbasename#1{%
  \edef\tcbexternal@job@name{\expandonce{\tcbexternal@prefix}\expandonce{#1}}%
  \edef\tcbexternal@job@mdfive{\expandonce{\tcbexternal@job@name.md5}}%
  \edef\tcbexternal@job@source{\expandonce{\tcbexternal@job@name.tex}}%
  \edef\tcbexternal@job@pdf{\expandonce{\tcbexternal@job@name.pdf}}%
}

\def\tcbexternal@corecompile{%
  \begingroup%
  \ifnum\the\catcode`\"=13 \tcbexternal@activate@normal@dq\fi%
  \message{=== Compile external '\tcbexternal@job@name': }%
  \immediate\openout\tcb@out="\tcbexternal@run@tex"
  \immediate\write\tcb@out{\string\gdef\string\TCBEXTERNALINPUT{"\tcbexternal@job@source"}}%
  \immediate\write\tcb@out{\string\gdef\string\TCBEXTERNALSAFETY{\tcbexternal@safety}}%
  \immediate\write\tcb@out{\string\gdef\string\TCBEXTERNALPREAMBLE{\expandonce{\tcbexternal@preamble}}}%
  \ifdefempty{\tcbexternal@preclass}{}{\immediate\write\tcb@out{\expandonce{\tcbexternal@preclass}}}%
  \immediate\write\tcb@out{\string\input{"\jobname.tex"}}%
  \immediate\closeout\tcb@out%
  \foreach \n in {1,...,\tcbexternal@runs}
  {%
    \immediate\write18{%
      \tcbexternal@compiler\space
      -shell-escape
      -halt-on-error
      -interaction=batchmode
      -jobname="\tcbexternal@job@name"
      "\tcbexternal@run@tex"
    }%
  }%
  \endgroup%
}

\def\tcbexternal@inputsource{%
  \IfFileExists{\tcbexternal@job@source}%
    {\input{\tcbexternal@job@source}}%
    {\tcb@error{File '\tcbexternal@job@source' missing.}{}}%
}

\def\tcbexternal@pdfmissing@warning{%
  \tcb@warning{File '\tcbexternal@job@pdf' missing.
    Compilation error or shell-escape wasn't enabled or a subdirectory could'nt be generated}%
  \message{Load '\tcbexternal@job@source' instead}%
  \tcbexternal@inputsource%
}

\def\tcbexternal@pdfmissing@error{%
  \tcb@error{File '\tcbexternal@job@pdf' missing.
    Compilation error or shell-escape wasn't enabled or a subdirectory could'nt be generated}{}%
}

\def\tcbexternal@inputpdf{%
  \IfFileExists{\tcbexternal@job@pdf}%
    {%
      \begingroup\edef\x{\endgroup%
        \noexpand\includegraphics[trim=\tcbexternal@safety\space\tcbexternal@safety%
        \space\tcbexternal@safety\space\tcbexternal@safety]{\expandonce{\tcbexternal@job@pdf}}}%
      \x%
    }%
    {\tcbexternal@pdfmissing}%
}

\newif\iftcb@externalize
\tcb@externalizefalse

\def\tcbexternal@generatemdivesum{%
  \iftcb@externalize%
    \def\tcbexternallastmdfivesum{}%
    \IfFileExists{\tcbexternal@job@mdfive}{\input{\tcbexternal@job@mdfive}}{}%
    \edef\tcbexternalmdfivesum{\pdfmdfivesum file {\tcbexternal@job@source}}%
  \else%
    \def\tcbexternallastmdfivesum{x}%
    \edef\tcbexternalmdfivesum{}%
  \fi%
  \immediate\openout\tcb@out=\tcbexternal@job@mdfive%
  \immediate\write\tcb@out{\string\def\string\tcbexternallastmdfivesum{\tcbexternalmdfivesum}\@percentchar}%
  \immediate\closeout\tcb@out%
}

\def\tcbexternal@conditionalcompile{%
  \IfFileExists{\tcbexternal@job@pdf}{%
    \ifdefstrequal{\tcbexternallastmdfivesum}{\tcbexternalmdfivesum}{%
    }{%
      \tcbexternal@corecompile%
    }%
  }{%
    \tcbexternal@corecompile%
  }%
}

\def\tcb@useexternal{%
  \tcbexternal@generatemdivesum%
  \iftcb@externalize%
    \tcbexternal@compile%
    \tcbexternal@inputpdf%
  \else%
    \tcbexternal@inputsource%
  \fi%
}

\newenvironment{tcbexternal}[2][]{%
  \tcbset{external/.cd,#1,name=#2}%
  \@ifundefined{@tcbexternal@JN@\tcbexternal@job@name}{%
      \global\@namedef{@tcbexternal@JN@\tcbexternal@job@name}{}%
    }{%
      \tcb@error{External job name '\tcbexternal@job@name' already used}%
        {Give a new unique name to the current external job.}%
    }%
  \begingroup%
  \let\tcb@verbatim@begin@hook=\tcbexternal@out@begin%
  \let\tcb@verbatim@end@hook=\tcbexternal@out@end%
  \tcbverbatimwrite{\tcbexternal@job@source}}%
{%
  \endtcbverbatimwrite\endgroup%
  \tcb@useexternal%
}

\long\def\new@tcb@externalizeenvironment#1#2#3#4#5{%
  \tcb@newenvironment{#1}[2][]{%
    #4%
    \begingroup%
    \tcbexternal[#3,##1,environment=#2]{##2}%
  }{%
    \endtcbexternal%
    \endgroup%
    #5%
  }%
}

\def\newtcbexternalizeenvironment{%
  \let\tcb@newenvironment\newenvironment%
  \new@tcb@externalizeenvironment%
}

\def\renewtcbexternalizeenvironment{%
  \let\tcb@newenvironment\renewenvironment%
  \new@tcb@externalizeenvironment%
}

\long\def\new@tcb@externalizetcolorbox#1#2#3#4{%
  \new@tcb@externalizeenvironment{#1}{#2}%
    {preamble tcbset={force nobeforeafter},#3}%
    {\tcb@layer@pushup\tcb@apply@box@options{#4}\tcb@set@normal@unbroken@beforeafter\tcb@before@unbroken}%
    {\tcb@after@unbroken}%
}

\def\newtcbexternalizetcolorbox{%
  \let\tcb@newenvironment\newenvironment%
  \new@tcb@externalizetcolorbox%
}

\def\renewtcbexternalizetcolorbox{%
  \let\tcb@newenvironment\renewenvironment%
  \new@tcb@externalizetcolorbox%
}


\newtcbexternalizeenvironment{extikzpicture}{tikzpicture}{}{}{}

\newtcbexternalizetcolorbox{extcolorbox}{tcolorbox}{}{}


\tcbset{
  external/.cd,
  %
  runner/.code={%
    \edef\tcbexternal@run@tex{\expandonce{#1}}%
  },
  %
  prefix/.store in=\tcbexternal@prefix,
  compiler/.store in=\tcbexternal@compiler,
  runs/.code={\numdef\tcbexternal@runs{#1}},
  name/.code={\tcbexternal@setbasename{#1}},
  safety/.store in=\tcbexternal@safety,
  preamble/.code={\appto\tcbexternal@preamble{#1}},
  preamble tcbset/.code={\appto\tcbexternal@preamble{\tcbset{#1}}},
  clear preamble/.code={\def\tcbexternal@preamble{}},
  preclass/.code={\appto\tcbexternal@preclass{#1}},
  clear preclass/.code={\def\tcbexternal@preclass{}},
  PassOptionsToPackage/.code 2 args={\appto\tcbexternal@preclass{\PassOptionsToPackage{#1}{#2}}},
  PassOptionsToClass/.code 2 args={\appto\tcbexternal@preclass{\PassOptionsToClass{#1}{#2}}},
  externalize/.code={},
  -/.style={externalize=false},
  %
  force remake/.is choice,
  force remake/true/.code={\let\tcbexternal@compile=\tcbexternal@corecompile},
  force remake/false/.code={\let\tcbexternal@compile=\tcbexternal@conditionalcompile},
  force remake/.default=true,
  !/.style=force remake,
  %
  input source on error/.is choice,
  input source on error/true/.code={\let\tcbexternal@pdfmissing=\tcbexternal@pdfmissing@warning},
  input source on error/false/.code={\let\tcbexternal@pdfmissing=\tcbexternal@pdfmissing@error},
  input source on error/.default=true,
  %
  plain/.code={%
    \let\tcbexternal@out@begin=\@empty%
    \let\tcbexternal@out@end=\@empty%
  },
  minipage/.code={%
    \appto\tcbexternal@out@begin{\immediate\write\tcb@out{\string\begin{minipage}{\the\dimexpr#1\relax}\string\ignorespaces\@percentchar}}%
    \preto\tcbexternal@out@end{\immediate\write\tcb@out{\string\end{minipage}\@percentchar}}%
  },
  minipage/.default=\linewidth,
  %
  environment with percent/.is choice,
  environment with percent/true/.style={%
    /tcb/external/environment/.code={%
      \appto\tcbexternal@out@begin{\immediate\write\tcb@out{\string\begin{##1}\@percentchar}}%
      \preto\tcbexternal@out@end{\immediate\write\tcb@out{\string\end{##1}\@percentchar}}%
    }
  },
  environment with percent/false/.style={%
    /tcb/external/environment/.code={%
      \appto\tcbexternal@out@begin{\immediate\write\tcb@out{\string\begin{##1}}}%
      \preto\tcbexternal@out@end{\immediate\write\tcb@out{\string\end{##1}}}%
    }
  },
  environment with percent/.default=true,
  %
  runner=\jobname_run.tex,
  prefix={external/},
  compiler=pdflatex,
  runs=1,
  name=unnamed,
  safety=2mm,
  clear preamble,
  clear preclass,
  force remake=false,
  input source on error,
  environment with percent,
  plain
}

\tcbset{%
  externalize example/.style={%
    external/name=#1,tempfile=\tcbexternal@job@source,
    code={\let\tcbusetemp=\tcb@useexternal}%
  },
  externalize example!/.style={externalize example=#1,external/force remake},
  externalize listing/.style={%
    external/name=#1,listing file=\tcbexternal@job@source,
    code={\let\tcbuselistingtext@input=\tcb@useexternal}%
  },
  externalize listing!/.style={externalize listing=#1,external/force remake},
}


==> tcbfitting.code.tex <==
%% The LaTeX package tcolorbox - version 3.80 (2015/11/27)
%% tcbfitting.code.tex: Code for fit boxes
%%
%% -------------------------------------------------------------------------------------------
%% Copyright (c) 2006-2015 by Prof. Dr. Dr. Thomas F. Sturm <thomas dot sturm at unibw dot de>
%% -------------------------------------------------------------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2005/12/01 or later.
%%
%% This work has the LPPL maintenance status `author-maintained'.
%%
%% This work consists of all files listed in README
%%
%\makeatletter
\tcb@set@library@version{3.80}

\newdimen\tcbfitdim
\newdimen\tcb@lowerfitdim
\newdimen\tcb@upperfitdim
\newif\iftcb@continue

\tcbset{%
  fit/.style={capture=fitbox},%
  fit to/.style args={#1 and #2}{capture=fitbox,width=#1,height=#2},%
  fit to height/.style={capture=fitbox,height=#1},%
  fit basedim/.code={\def\kvtcb@fit@basedim{#1}\tcbfitdim\kvtcb@fit@basedim},%
  fit skip/.store in=\kvtcb@fit@skip,%
  fit fontsize macros/.code={%
    \renewcommand\tiny{\tcb@setfontsize\tiny{0.5}}%
    \renewcommand\scriptsize{\tcb@setfontsize\scriptsize{0.7}}%
    \renewcommand\footnotesize{\tcb@setfontsize\footnotesize{0.8}}%
    \renewcommand\small{\tcb@setfontsize\small{0.9}}%
    \renewcommand\normalsize{\tcb@setfontsize\normalsize{1}}%
    \renewcommand\large{\tcb@setfontsize\large{1.2}}%
    \renewcommand\Large{\tcb@setfontsize\Large{1.44}}%
    \renewcommand\LARGE{\tcb@setfontsize\LARGE{1.728}}%
    \renewcommand\huge{\tcb@setfontsize\huge{2.0736}}%
    \renewcommand\Huge{\tcb@setfontsize\Huge{2.48832}}},%
  fit height plus/.style={fit,height plus=#1},%
  fit width plus/.dimstore in=\kvtcb@fit@plus@width,%
  fit height from/.style args={#1 to #2}{fit,height from={#1} to {#2}},
  fit width from/.style args={#1 to #2}{fit,width={#1},fit width plus={#2-#1}},
  fit maxstep/.store in=\kvtcb@fit@maxstep,%
  fit maxfontdiff/.store in=\kvtcb@fit@maxfontdiff,%
  fit maxfontdiffgap/.store in=\kvtcb@fit@maxfontdiffgap,%
  fit maxwidthdiff/.store in=\kvtcb@fit@maxwidthdiff,%
  fit maxwidthdiffgap/.store in=\kvtcb@fit@maxwidthdiffgap,%
  fit warning/.is choice,
  fit warning/on/.code={\let\tcb@fit@warn@begin=\@empty%
    \let\tcb@fit@warn@end=\@empty},
  fit warning/off/.code={\def\tcb@fit@warn@begin{\hbadness=10000\relax}%
    \let\tcb@fit@warn@end=\@empty},
  fit warning/final/.code={\tcb@cur@hbadness=\hbadness\def\tcb@fit@warn@begin{\hbadness=10000\relax}%
    \def\tcb@fit@warn@end{\hbadness=\tcb@cur@hbadness\relax\tcb@fit@@box}},
  fit algorithm/.is choice,
  fit algorithm/fontsize/.code={\let\tcbox@fitalgorithm=\tcbox@fitalgorithm@fontsize},
  fit algorithm/fontsize*/.code={\let\tcbox@fitalgorithm=\tcbox@fitalgorithm@fontsize@star},
  fit algorithm/areasize/.code={\let\tcbox@fitalgorithm=\tcbox@fitalgorithm@areasize},
  fit algorithm/areasize*/.code={\let\tcbox@fitalgorithm=\tcbox@fitalgorithm@areasize@star},
  fit algorithm/hybrid/.code={\let\tcbox@fitalgorithm=\tcbox@fitalgorithm@hybrid},
  fit algorithm/hybrid*/.code={\let\tcbox@fitalgorithm=\tcbox@fitalgorithm@hybrid@star},
  fit algorithm/squeeze/.code={\let\tcbox@fitalgorithm=\tcbox@fitalgorithm@squeeze},
  spartan@fit/.style={fit algorithm=squeeze},
}

\def\tcb@@capture@fitbox{%
  \let\endtcolorbox=\relax%
  \Collect@Body\tcbox@inner@fitbox@collected%
}

\def\tcbfontsize#1{\fontsize{#1\tcbfitdim}{#1\dimexpr\kvtcb@fit@skip\tcbfitdim}\selectfont}

\def\tcb@setfontsize#1#2{\@setfontsize#1{#2\tcbfitdim}{#2\dimexpr\kvtcb@fit@skip\tcbfitdim}}

\long\def\tcbox@inner@fitbox@collected#1{%
  \tcbox@inner@fitbox{#1}%
  \tcb@finalize@environment%
}

\newcount\tcb@cur@hbadness

\def\tcbox@fitalgorithm@fontsize{%
  \tcb@continuetrue%
  \loop%
    \tcbfitdim.5\tcbfitdim%
    \tcb@fit@@box%
    \ifnum\count@=\kvtcb@fit@maxstep\relax%
      \tcb@continuefalse%
    \else%
      \ifdim\dimexpr\tcb@fit@@h>\tcb@fit@@target\relax%
        \ifdim\tcbfitdim<18000sp\relax%
          \count@\kvtcb@fit@maxstep\relax%
          \tcb@continuefalse%
        \fi%
      \else%
        \tcb@continuefalse%
      \fi%
    \fi%
  \iftcb@continue \repeat%
  \ifnum\count@<\kvtcb@fit@maxstep\relax%
    \tcbdimto\tcb@fit@@gap{\tcb@fit@@target-\tcb@fit@@h}%
    \tcb@lowerfitdim\tcbfitdim%
    \tcb@upperfitdim2\tcbfitdim%
    \tcbfitdim1.5\tcbfitdim%
    \loop%
      \tcb@fit@@box%
      \tcb@continuetrue%
      \ifnum\count@<\kvtcb@fit@maxstep\relax%
        \ifdim\dimexpr\tcb@upperfitdim-\tcb@lowerfitdim<\kvtcb@fit@maxfontdiff\relax%
          \tcb@continuefalse%
        \else%
          \ifdim\dimexpr\tcb@upperfitdim-\tcb@lowerfitdim<\kvtcb@fit@maxfontdiffgap\relax%
            \ifdim\dimexpr\tcb@fit@@gap<\tcb@fit@@line\relax%
              \tcb@continuefalse%
            \fi%
          \fi%
        \fi%
      \else%
        \tcb@continuefalse%
      \fi%
      \iftcb@continue%
        \ifdim\dimexpr\tcb@fit@@h>\tcb@fit@@target\relax%
          \tcb@upperfitdim\tcbfitdim%
          \advance\tcbfitdim\tcb@lowerfitdim%
          \tcbfitdim0.5\tcbfitdim%
        \else%
          \tcbdimto\tcb@fit@@gap{\tcb@fit@@target-\tcb@fit@@h}%
          \tcb@lowerfitdim\tcbfitdim%
          \advance\tcbfitdim\tcb@upperfitdim%
          \tcbfitdim0.5\tcbfitdim%
        \fi%
      \else%
        \ifdim\dimexpr\tcb@fit@@h>\tcb@fit@@target\relax%
          \tcbfitdim\tcb@lowerfitdim%
          \tcb@fit@@box%
        \fi%
      \fi%
    \iftcb@continue \repeat%
  \fi%
}

\def\tcbox@fitalgorithm@fontsize@star{%
  \tcbox@fitalgorithm@fontsize%
  \tcb@resize@box{\tcb@upperbox}{\tcb@w@upper}{\tcb@fit@@target}%
  \tcbdimto\tcb@fit@@h{\ht\tcb@upperbox+\dp\tcb@upperbox}%
}

\def\tcbox@fitalgorithm@areasize@core{%
  \pgfmathdivide{\tcb@fit@@h}{\tcb@fit@@target}%
  \pgfmathsqrt{\pgfmathresult}%
  \let\tcb@temp=\pgfmathresult%
  \tcbdimto\tcb@w@upper@temp{\pgfmathresult\dimexpr\tcb@w@upper}%
  \tcb@fit@@boxsave{\tcb@w@upper@temp}%
  %
  \tcbdimto\tcb@fit@@h{\ht\tcb@upperbox+\dp\tcb@upperbox}%
  \pgfmathdivide{\tcb@fit@@h}{\tcb@fit@@target}%
  \pgfmathdivide{\pgfmathresult}{\tcb@temp}%
  \pgfmathsqrt{\pgfmathresult}%
  \ifdim\dimexpr\pgfmathresult pt<0.98pt\relax
    \tcbdimto\tcb@w@upper@temp{\pgfmathresult\dimexpr\tcb@w@upper@temp}%
    \tcb@fit@@boxsave{\tcb@w@upper@temp}%
  \else\ifdim\dimexpr\pgfmathresult pt>1.02pt\relax
    \tcbdimto\tcb@w@upper@temp{\pgfmathresult\dimexpr\tcb@w@upper@temp}%
    \tcb@fit@@boxsave{\tcb@w@upper@temp}%
  \fi\fi%
  %
  \tcbdimto\tcb@fit@@h{\ht\tcb@upperbox+\dp\tcb@upperbox}%
}

\def\tcbox@fitalgorithm@areasize{%
  \tcbox@fitalgorithm@areasize@core%
  \pgfmathdivide{\tcb@w@upper}{\tcb@w@upper@temp}%
  \tcbdimto\tcb@fit@@h{\pgfmathresult\dimexpr\tcb@fit@@h}%
  \ifdim\dimexpr\tcb@fit@@h>\tcb@fit@@target\relax%
    \let\tcb@fit@@h=\tcb@fit@@target%
  \fi
  \tcb@resize@box{\tcb@upperbox}{\tcb@w@upper}{\tcb@fit@@h}%
  %
  \tcbdimto\tcb@fit@@h{\ht\tcb@upperbox+\dp\tcb@upperbox}%
}

\def\tcbox@fitalgorithm@areasize@star{%
  \tcbox@fitalgorithm@areasize@core%
  \tcb@resize@box{\tcb@upperbox}{\tcb@w@upper}{\tcb@fit@@target}%
  \tcbdimto\tcb@fit@@h{\ht\tcb@upperbox+\dp\tcb@upperbox}%
}

\def\tcbox@fitalgorithm@squeeze{%
  \tcb@resize@box{\tcb@upperbox}{\tcb@w@upper}{\tcb@fit@@target}%
  \tcbdimto\tcb@fit@@h{\ht\tcb@upperbox+\dp\tcb@upperbox}%
}

\def\tcbox@fitalgorithm@hybrid@core{%
  \pgfmathdivide{\tcb@fit@@target}{\tcb@fit@@h}%
  \pgfmathsqrt{\pgfmathresult}%
  \tcbfitdim=\pgfmathresult\tcbfitdim%
  \tcb@fit@@box%
  %
  \pgfmathdivide{\tcb@fit@@target}{\tcb@fit@@h}%
  \pgfmathsqrt{\pgfmathresult}%
  \ifdim\dimexpr\pgfmathresult pt<0.85pt\relax
    \tcbfitdim=\pgfmathresult\tcbfitdim%
    \tcb@fit@@box%
  \else\ifdim\dimexpr\pgfmathresult pt>1.15pt\relax
    \tcbfitdim=\pgfmathresult\tcbfitdim%
    \tcb@fit@@box%
  \fi\fi%
}

\def\tcbox@fitalgorithm@hybrid{%
  \tcbox@fitalgorithm@hybrid@core%
  \tcbox@fitalgorithm@areasize%
}

\def\tcbox@fitalgorithm@hybrid@star{%
  \tcbox@fitalgorithm@hybrid@core%
  \tcbox@fitalgorithm@areasize@star%
}

\def\tcb@fit@@box{%
  \iftcb@hasTitle%
    \tcbdimto\tcb@w@title{\kvtcb@width-(\kvtcb@left@rule)-(\kvtcb@right@rule)-(\kvtcb@boxsep)*2-(\kvtcb@lefttitle)-(\kvtcb@righttitle)}%
    \begin{tcb@savebox}{\tcb@titlebox}{\tcb@w@title}\color{tcbcol@title}\kvtcb@fonttitle\kvtcb@haligntitle\kvtcb@before@title\kvtcb@title\kvtcb@after@title\end{tcb@savebox}%
    \tcbdimto\tcb@h@titletotal{\ht\tcb@titlebox+\dp\tcb@titlebox+\kvtcb@title@rule+(\kvtcb@boxsep)*2+\kvtcb@toptitle+\kvtcb@bottomtitle}%
  \else%
    \let\tcb@h@titletotal=\tcb@zpt%
  \fi%
  \tcbdimto\tcb@fit@@line{\kvtcb@fit@skip\tcbfitdim}%
  \tcbdimto\tcb@w@upper{\kvtcb@width-(\kvtcb@left@rule)-(\kvtcb@right@rule)-(\kvtcb@boxsep)*2-(\kvtcb@leftupper)-(\kvtcb@rightupper)}%
  \tcb@fit@@boxsave{\tcb@w@upper}%
  \tcbdimto\tcb@fit@@h{\ht\tcb@upperbox+\dp\tcb@upperbox}%
  \tcbdimto\tcb@fit@@target{\kvtcb@height@fixed-(\kvtcb@top@rule@stand)-(\kvtcb@bottom@rule@stand)-(\kvtcb@top)-(\kvtcb@bottom)-(\kvtcb@boxsep)*2-\tcb@h@titletotal}%
}%

\long\def\tcbox@inner@fitbox#1{%
  \tcbset{breakable@false,sidebyside=false}%
  \let\tcb@val@raisebase=\tcb@zpt%
  \unless\ifdefined\kvtcb@height@fixed%
    \tcbset{height=\kvtcb@width}%
  \fi%
  \tcb@hasLowerfalse%
  %
  \count@\z@%
  \tcbfitdim\kvtcb@fit@basedim%
  \tcb@fit@warn@begin%
  %
  \def\tcb@fit@@boxsave##1{%
    \tcbdimto\tcb@innerwidth{\kvtcb@width-\kvtcb@left@rule-\kvtcb@right@rule}%
    \colorlet{tcbcol@origin}{.}%
    \tcb@set@color{tcbcol@upper}%
    \begin{tcb@savebox}{\tcb@upperbox}{##1}%
      \kvtcb@fontupper\fontsize{\tcbfitdim}{\tcb@fit@@line}\selectfont%
%      \kvtcb@halignupper\kvtcb@before@upper\ignorespaces#1\unskip\kvtcb@after@upper%
      \kvtcb@halignupper\kvtcb@before@upper\ignorespaces#1\kvtcb@after@upper%
    \end{tcb@savebox}%
    \tcb@reset@color%
    \advance\count@ 1\relax%
  }%
  %
  \tcb@set@@phantom%
  \tcb@set@@title%
  \tcb@fit@@box%
  %
  % height fit
  \ifdim\kvtcb@height@fixed@plus>0pt\relax%
    \let\tcb@fit@@minheight=\kvtcb@height@fixed%
    \ifdim\dimexpr\tcb@fit@@h>\tcb@fit@@target\relax%
      \ifdim\dimexpr\tcb@fit@@h>\dimexpr\tcb@fit@@target+\kvtcb@height@fixed@plus\relax%
        \tcbdimto\kvtcb@height@fixed{\kvtcb@height@fixed+\kvtcb@height@fixed@plus}%
        \tcbdimto\tcb@fit@@target{\tcb@fit@@target+\kvtcb@height@fixed@plus}%
      \else%
        \tcbdimto\kvtcb@height@fixed{\kvtcb@height@fixed+\tcb@fit@@h-\tcb@fit@@target}%
        \let\tcb@fit@@target=\tcb@fit@@h%
      \fi%
    \fi%
  \fi%
  %
  % width fit
  \ifdim\kvtcb@fit@plus@width>0pt\relax%
    \ifnum\count@<\kvtcb@fit@maxstep\relax%
      \ifdim\dimexpr\tcb@fit@@h>\tcb@fit@@target\relax%
        \tcb@lowerfitdim\dimexpr\kvtcb@width\relax%
        \tcb@upperfitdim\dimexpr\kvtcb@width+\kvtcb@fit@plus@width\relax%
        \tcbdimto\kvtcb@width{\tcb@upperfitdim}%
        \tcb@fit@@box%
        \ifdim\dimexpr\tcb@fit@@h>\tcb@fit@@target\relax%
        \else%
          \ifnum\count@<\kvtcb@fit@maxstep\relax%
            \tcbdimto\tcb@fit@@gap{\tcb@fit@@target-\tcb@fit@@h}%
            \tcbdimto\kvtcb@width{(\tcb@lowerfitdim+\tcb@upperfitdim)/2}%
            \loop%
              \tcb@fit@@box%
              \tcb@continuetrue%
              \ifnum\count@<\kvtcb@fit@maxstep\relax%
                \ifdim\dimexpr\tcb@upperfitdim-\tcb@lowerfitdim<\kvtcb@fit@maxwidthdiff\relax%
                  \tcb@continuefalse%
                \else%
                  \ifdim\dimexpr\tcb@upperfitdim-\tcb@lowerfitdim<\kvtcb@fit@maxwidthdiffgap\relax%
                    \ifdim\dimexpr\tcb@fit@@gap<\tcb@fit@@line\relax%
                      \tcb@continuefalse%
                    \fi%
                  \fi%
                \fi%
              \else%
                \tcb@continuefalse%
              \fi%
              \iftcb@continue%
                \ifdim\dimexpr\tcb@fit@@h>\tcb@fit@@target\relax%
                  \tcb@lowerfitdim\dimexpr\kvtcb@width\relax%
                  \tcbdimto\kvtcb@width{(\tcb@lowerfitdim+\tcb@upperfitdim)/2}%
                \else%
                  \tcb@upperfitdim\dimexpr\kvtcb@width\relax%
                  \tcbdimto\tcb@fit@@gap{\tcb@fit@@target-\tcb@fit@@h}%
                  \tcbdimto\kvtcb@width{(\tcb@lowerfitdim+\tcb@upperfitdim)/2}%
                \fi%
              \else%
                \ifdim\dimexpr\tcb@fit@@h>\tcb@fit@@target\relax%
                  \tcbdimto\kvtcb@width{\tcb@upperfitdim}%
                  \tcb@fit@@box%
                \fi%
              \fi%
            \iftcb@continue \repeat%
          \fi%
        \fi%
      \fi%
    \fi%
  \fi%
  %
  % (font) fit
  \ifnum\count@<\kvtcb@fit@maxstep\relax%
    \ifdim\dimexpr\tcb@fit@@h>\tcb@fit@@target\relax%
    \tcbox@fitalgorithm%
    \fi%
  \fi%
  %
  \tcb@fit@warn@end%
  %
  % last height fit
  \ifdim\kvtcb@height@fixed@plus>0pt\relax%
    \ifdim\dimexpr\tcb@fit@@h<\tcb@fit@@target\relax%
      \tcbdimto\tcb@temp{\kvtcb@height@fixed+\tcb@fit@@h-\tcb@fit@@target}%
      \ifdim\dimexpr\tcb@temp<\tcb@fit@@minheight\relax%
      \else%
        \let\kvtcb@height@fixed=\tcb@temp%
      \fi%
    \fi%
  \fi%
  %
  \edef\tcbfitsteps{\the\count@}%
  \tcb@set@@dimensions%
  \tcb@draw@color@box%
}

\newcommand{\tcboxfit}[2][]{%
  \tcb@ox{capture=fitbox,#1}{#2}%
}

\long\def\tcb@newtcboxfit#1#2{\expandafter\tcb@newcommand\csname#1\endcsname{\tcboxfit[#2,options@for=#1]}}

\long\def\tcb@newtcboxfit@#1[#2]#3{\expandafter\tcb@newcommand\csname#1\endcsname[#2]{\tcboxfit[#3,options@for=#1]}}

\long\def\tcb@newtcboxfit@@#1[#2][#3]#4{\expandafter\tcb@newcommand\csname#1\endcsname[#2][#3]{\tcboxfit[#4,options@for=#1]}}

\long\def\tcb@new@tcboxfit@#1[#2]{%
  \@ifnextchar[{\tcb@newtcboxfit@@{#1}[#2]}{\tcb@newtcboxfit@{#1}[#2]}}

\long\def\tcb@new@tcboxfit#1{%
  \@ifnextchar[{\tcb@new@tcboxfit@{#1}}{\tcb@newtcboxfit{#1}}}

\def\newtcboxfit{%
  \let\tcb@newcommand\newcommand%
  \let\tcb@process@newtcolorbox@continue\tcb@new@tcboxfit%
  \tcb@process@newcommand}

\def\renewtcboxfit{%
  \let\tcb@newcommand\renewcommand%
  \let\tcb@process@newtcolorbox@continue\tcb@new@tcboxfit%
  \tcb@process@newcommand}

\tcbset{%
  reset@fitting/.style={%
    fit algorithm=fontsize,%
    fit basedim=10pt,fit skip=1.2,
    height plus=0pt,fit width plus=0pt,
    fit maxstep=20,fit maxfontdiff=0.1pt,fit maxfontdiffgap=1pt,
    fit maxwidthdiff=1pt,fit maxwidthdiffgap=10pt,
    fit warning=off
  },
  initialize@reset=reset@fitting,
}



==> tcbhooks.code.tex <==
%% The LaTeX package tcolorbox - version 3.80 (2015/11/27)
%% tcbhooks.code.tex: Code for adding hooks
%%
%% -------------------------------------------------------------------------------------------
%% Copyright (c) 2006-2015 by Prof. Dr. Dr. Thomas F. Sturm <thomas dot sturm at unibw dot de>
%% -------------------------------------------------------------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2005/12/01 or later.
%%
%% This work has the LPPL maintenance status `author-maintained'.
%%
%% This work consists of all files listed in README
%%
%\makeatletter
\tcb@set@library@version{3.80}

\tcbset{%
  before upper app/.code={\appto\kvtcb@before@upper{#1}},%
  before upper pre/.code={\preto\kvtcb@before@upper{#1}},%
  after upper app/.code={\appto\kvtcb@after@upper{#1}},%
  after upper pre/.code={\preto\kvtcb@after@upper{#1}},%
  before lower app/.code={\appto\kvtcb@before@lower{#1}},%
  before lower pre/.code={\preto\kvtcb@before@lower{#1}},%
  after lower app/.code={\appto\kvtcb@after@lower{#1}},%
  after lower pre/.code={\preto\kvtcb@after@lower{#1}},%
  before title app/.code={\appto\kvtcb@before@title{#1}},%
  before title pre/.code={\preto\kvtcb@before@title{#1}},%
  after title app/.code={\appto\kvtcb@after@title{#1}},%
  after title pre/.code={\preto\kvtcb@after@title{#1}},%
  %
  % usable inside the document or in the preamble after setting before / after
  before app/.code={\appto\kvtcb@beforebox{#1}},%
  before pre/.code={\preto\kvtcb@beforebox{#1}},%
  after app/.code={\appto\kvtcb@afterbox{#1}},%
  after pre/.code={\preto\kvtcb@afterbox{#1}},%
  %
  overlay unbroken app/.code={\appto\tcb@overlay@unbroken{#1}},%
  overlay unbroken pre/.code={\preto\tcb@overlay@unbroken{#1}},%
  overlay first app/.code={\appto\tcb@overlay@first{#1}},%
  overlay first pre/.code={\preto\tcb@overlay@first{#1}},%
  overlay middle app/.code={\appto\tcb@overlay@middle{#1}},%
  overlay middle pre/.code={\preto\tcb@overlay@middle{#1}},%
  overlay last app/.code={\appto\tcb@overlay@last{#1}},%
  overlay last pre/.code={\preto\tcb@overlay@last{#1}},%
  %
  overlay app/.style={overlay unbroken app={#1},overlay first app={#1},overlay middle app={#1},overlay last app={#1}},%
  overlay pre/.style={overlay unbroken pre={#1},overlay first pre={#1},overlay middle pre={#1},overlay last pre={#1}},%
  overlay broken app/.style={overlay first app={#1},overlay middle app={#1},overlay last app={#1}},%
  overlay broken pre/.style={overlay first pre={#1},overlay middle pre={#1},overlay last pre={#1}},%
  overlay unbroken and first app/.style={overlay unbroken app={#1},overlay first app={#1}},%
  overlay unbroken and first pre/.style={overlay unbroken pre={#1},overlay first pre={#1}},%
  overlay unbroken and last app/.style={overlay unbroken app={#1},overlay last app={#1}},%
  overlay unbroken and last pre/.style={overlay unbroken pre={#1},overlay last pre={#1}},%
  overlay middle and last app/.style={overlay middle app={#1},overlay last app={#1}},%
  overlay middle and last pre/.style={overlay middle pre={#1},overlay last pre={#1}},%
  overlay first and middle app/.style={overlay first app={#1},overlay middle app={#1}},%
  overlay first and middle pre/.style={overlay first pre={#1},overlay middle pre={#1}},%
  %
  % skins:
  frame code app/.code={\appto\tcb@frame@code{#1}},%
  frame code pre/.code={\preto\tcb@frame@code{#1}},%
  interior titled code app/.code={\appto\tcb@interiortitled@code{#1}},%
  interior titled code pre/.code={\preto\tcb@interiortitled@code{#1}},%
  interior code app/.code={\appto\tcb@interior@code{#1}},%
  interior code pre/.code={\preto\tcb@interior@code{#1}},%
  segmentation code app/.code={\appto\tcb@segmentation@code{#1}},%
  segmentation code pre/.code={\preto\tcb@segmentation@code{#1}},%
  title code app/.code={\appto\tcb@title@code{#1}},%
  title code pre/.code={\preto\tcb@title@code{#1}},%
  %
  extras unbroken pre/.code={\preto\tcb@extras@unbroken{#1}},%
  extras first pre/.code={\preto\tcb@extras@first{#1}},%
  extras middle pre/.code={\preto\tcb@extras@middle{#1}},%
  extras last pre/.code={\preto\tcb@extras@last{#1}},%
  extras pre/.style={extras unbroken pre={#1},extras first pre={#1},extras middle pre={#1},extras last pre={#1}},%
  extras broken pre/.style={extras first pre={#1},extras middle pre={#1},extras last pre={#1}},%
  extras unbroken and first pre/.style={extras unbroken pre={#1},extras first pre={#1}},%
  extras unbroken and last pre/.style={extras unbroken pre={#1},extras last pre={#1}},%
  extras middle and last pre/.style={extras middle pre={#1},extras last pre={#1}},%
  extras first and middle pre/.style={extras first pre={#1},extras middle pre={#1}},%
  %
  underlay unbroken pre/.code={\preto\tcb@underlay@unbroken{#1}},%
  underlay first pre/.code={\preto\tcb@underlay@first{#1}},%
  underlay middle pre/.code={\preto\tcb@underlay@middle{#1}},%
  underlay last pre/.code={\preto\tcb@underlay@last{#1}},%
  underlay boxed title pre/.code={\preto\tcb@underlay@boxedtitle{#1}},%
  underlay pre/.style={underlay unbroken pre={#1},underlay first pre={#1},underlay middle pre={#1},underlay last pre={#1}},%
  underlay broken pre/.style={underlay first pre={#1},underlay middle pre={#1},underlay last pre={#1}},%
  underlay unbroken and first pre/.style={underlay unbroken pre={#1},underlay first pre={#1}},%
  underlay unbroken and last pre/.style={underlay unbroken pre={#1},underlay last pre={#1}},%
  underlay middle and last pre/.style={underlay middle pre={#1},underlay last pre={#1}},%
  underlay first and middle pre/.style={underlay first pre={#1},underlay middle pre={#1}},%
  finish unbroken pre/.code={\preto\tcb@finish@unbroken{#1}},%
  finish first pre/.code={\preto\tcb@finish@first{#1}},%
  finish middle pre/.code={\preto\tcb@finish@middle{#1}},%
  finish last pre/.code={\preto\tcb@finish@last{#1}},%
  finish pre/.style={finish unbroken pre={#1},finish first pre={#1},finish middle pre={#1},finish last pre={#1}},%
  finish broken pre/.style={finish first pre={#1},finish middle pre={#1},finish last pre={#1}},%
  finish unbroken and first pre/.style={finish unbroken pre={#1},finish first pre={#1}},%
  finish unbroken and last pre/.style={finish unbroken pre={#1},finish last pre={#1}},%
  finish middle and last pre/.style={finish middle pre={#1},finish last pre={#1}},%
  finish first and middle pre/.style={finish first pre={#1},finish middle pre={#1}},%
  %
  watermark tikz app/.style={overlay app={\tcb@drawspec@watermark@tikz{#1}}},
  watermark tikz pre/.style={overlay pre={\tcb@drawspec@watermark@tikz{#1}}},
  watermark tikz app on/.style args={#1 is #2}{overlay #1 app={\tcb@drawspec@watermark@tikz{#2}}},%
  watermark tikz pre on/.style args={#1 is #2}{overlay #1 pre={\tcb@drawspec@watermark@tikz{#2}}},%
  watermark graphics app/.style={overlay app={\tcb@drawspec@watermark@graphics{#1}}},
  watermark graphics pre/.style={overlay pre={\tcb@drawspec@watermark@graphics{#1}}},
  watermark graphics app on/.style args={#1 is #2}{overlay #1 app={\tcb@drawspec@watermark@graphics{#2}}},
  watermark graphics pre on/.style args={#1 is #2}{overlay #1 pre={\tcb@drawspec@watermark@graphics{#2}}},
  watermark text app/.style={overlay app={\tcb@drawspec@watermark@text{#1}}},
  watermark text pre/.style={overlay pre={\tcb@drawspec@watermark@text{#1}}},
  watermark text app on/.style args={#1 is #2}{overlay #1 app={\tcb@drawspec@watermark@text{#2}}},
  watermark text pre on/.style args={#1 is #2}{overlay #1 pre={\tcb@drawspec@watermark@text{#2}}},
}



==> tcblistings.code.tex <==
%% The LaTeX package tcolorbox - version 3.80 (2015/11/27)
%% tcblistings.code.tex: Code for colorboxes with listings
%%
%% -------------------------------------------------------------------------------------------
%% Copyright (c) 2006-2015 by Prof. Dr. Dr. Thomas F. Sturm <thomas dot sturm at unibw dot de>
%% -------------------------------------------------------------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2005/12/01 or later.
%%
%% This work has the LPPL maintenance status `author-maintained'.
%%
%% This work consists of all files listed in README
%%
%\makeatletter
\tcb@set@library@version{3.80}

\RequirePackage{listings}[2007/02/22]

\tcbuselibrary{listings@core}

\let\tcb@listing@MakeCaption@org=\lst@MakeCaption

\def\tcb@listing@set@MakeCaption@org{%
  \let\lst@MakeCaption\tcb@listing@MakeCaption@org}
\def\tcb@listing@set@MakeCaption@empty{%
  \lst@HRefStepCounter{lstlisting}%
  \let\lst@MakeCaption\@gobble}

\lstdefinestyle{tcblatex}{language={[LaTeX]TeX},
     aboveskip={0\p@ \@plus 6\p@}, belowskip={0\p@ \@plus 6\p@},
     columns=fullflexible, keepspaces=true,
     breaklines=true, breakatwhitespace=true,
     basicstyle=\ttfamily\small, extendedchars=true, nolol,
     inputencoding=\kvtcb@listingencoding}

\def\tcb@listing@input@listing#1#2{%
  \begingroup%
  \toks@=\expandafter{#1}%
  \edef\tcb@temp{\noexpand\lstinputlisting[nolol,\the\toks@]}%
  \tcb@listing@set@MakeCaption%
  \tcb@temp{#2}%
  \endgroup%
}%


\def\tcb@listing@uselistinglisting{%
  \tcb@listing@input@listing{\kvtcb@listingoptions}{\kvtcb@listingfile}%
}%

\def\tcb@listing@usetemplisting{%
  \tcb@listing@input@listing{\kvtcb@listingoptions}{\kvtcb@tempfile}%
}%

\def\tcb@listing@doc@usetemplisting{%
  \tcb@listing@input@listing{\kvtcb@doclistingoptions}{\kvtcb@tempfile}%
}

\tcbset{%
  listing options/.store in=\kvtcb@listingoptions,%
  listing style/.style={listing options={style=#1}},%
  no listing options/.style={listing options=},%
  listing inputencoding/.store in=\kvtcb@listingencoding,%
  listing remove caption/.is choice,
  listing remove caption/true/.code={\let\tcb@listing@set@MakeCaption\tcb@listing@set@MakeCaption@empty},
  listing remove caption/false/.code={\let\tcb@listing@set@MakeCaption\tcb@listing@set@MakeCaption@org},
  listing remove caption/.default=true,
  listing engine/listings/.code={\let\tcbuselistinglisting\tcb@listing@uselistinglisting%
    \let\tcbusetemplisting\tcb@listing@usetemplisting%
    \let\tcb@doc@usetemplisting\tcb@listing@doc@usetemplisting},
  every listing line/.code={%
    \def\lst@NewLine{%
      \ifx\lst@OutputBox\@gobble\else
          \par\noindent \hbox{}#1%
      \fi
      \global\advance\lst@newlines\m@ne
      \lst@newlinetrue}},%
  every listing line*/.style={every listing line={#1},%
    code={\setbox\z@=\hbox{#1}\tcbdimto\kvtcb@rightupper{\kvtcb@rightupper+\wd\z@}}},%
}


\tcbset{%
  reset@listings/.style={%
    listing style=tcblatex,
    listing inputencoding=\inputencodingname,
    listing remove caption,
    listing engine=listings,
  },
  initialize@reset=reset@listings,
}



==> tcblistingscore.code.tex <==
%% The LaTeX package tcolorbox - version 3.80 (2015/11/27)
%% tcblistingscode.code.tex: Auxiliary code for colorboxes with listings
%%
%% -------------------------------------------------------------------------------------------
%% Copyright (c) 2006-2015 by Prof. Dr. Dr. Thomas F. Sturm <thomas dot sturm at unibw dot de>
%% -------------------------------------------------------------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2005/12/01 or later.
%%
%% This work has the LPPL maintenance status `author-maintained'.
%%
%% This work consists of all files listed in README
%%
%\makeatletter
\tcb@set@library@version{3.80}

\RequirePackage{pdftexcmds}

\def\tcbuselistingtext@input{\input{\kvtcb@listingfile}}%
\def\tcbuselistingtext{\tcbuselistingtext@input}%
\def\tcbuselistingcomment{\kvtcb@listingcomment}%
\def\tcb@listing@listing{\tcbuselistinglisting}

\def\tcb@listing@listingAndOther{%
   \tcbuselistinglisting%
   \tcblower%
   \tcb@use@listing@other%
}

\def\tcb@listing@otherAndListing{%
   \tcb@use@listing@other%
   \tcblower%
   \tcbuselistinglisting%
}

\newenvironment{tcb@lower@outside}[1]{%
  \tcbset{savedelimiter=tcb@lower@outside}\tcb@minipage{#1}%
  \color{tcbcol@lower}\kvtcb@fontlower\kvtcb@halignlower\kvtcb@before@lower\ignorespaces}%
%  {\unskip\kvtcb@after@lower\endminipage}
  {\kvtcb@after@lower\endminipage}

\def\tcb@use@listing@other@reset{%
  \tcbset{every box on layer 1/.style={reset,every box}}%
  \tcb@use@listing@other}

\def\tcb@use@lower@outside#1{%
  \setbox\z@=\hbox{\begin{tcb@lower@outside}{#1}%
    \tcb@use@listing@other@reset%
  \end{tcb@lower@outside}}%
  \tcbdimto{\tcb@temp@wd}{\wd\z@}%
  \unhbox\z@%
}

\def\tcb@inputlisting@out@otherAboveListing{%
  {\kvtcb@beforebox}\noindent%
  \iftcb@lowervisible%
    \tcb@use@lower@outside{\kvtcb@width}%
    \par\vskip-\parskip\vspace*{\kvtcb@middle}\noindent%
  \fi%
  \begin{tcolorbox}[before=,savedelimiter=tcolorbox]\tcbuselistinglisting\end{tcolorbox}%
}

\def\tcb@inputlisting@out@otherAboveListing@Decoupled{%
  \iftcb@lowervisible%
    {\par\tcb@use@listing@other@reset\par}%
  \fi%
  \begin{tcolorbox}[savedelimiter=tcolorbox]\tcbuselistinglisting\end{tcolorbox}%
}

\def\tcb@inputlisting@out@listingAboveOther{%
  \begin{tcolorbox}[after=,savedelimiter=tcolorbox]\tcbuselistinglisting\end{tcolorbox}%
  \iftcb@lowervisible\par\vskip-\parskip\vspace*{\kvtcb@middle}\noindent%
    \tcb@use@lower@outside{\kvtcb@width}%
  \fi%
  {\kvtcb@afterbox}%
}

\def\tcb@inputlisting@out@listingAboveOther@Decoupled{%
  \begin{tcolorbox}[savedelimiter=tcolorbox]\tcbuselistinglisting\end{tcolorbox}%
  \iftcb@lowervisible%
    {\par\tcb@use@listing@other@reset\par}%
  \fi%
}


\newenvironment{tcb@outside@environment}{%
  \tcb@before@unbroken%
  \begin{minipage}{\tcb@width}}%
{%
  \end{minipage}%
  \tcb@after@unbroken}

\def\tcb@inputlisting@out@prepare{%
  \tcbdimto\tcb@width{\kvtcb@width}%
  \tcbdimto\tcb@innerwidth{\tcb@width-\kvtcb@left@rule-\kvtcb@right@rule}%
  \tcbdimto\tcb@temp{\tcb@innerwidth-\kvtcb@boxsep*2}%
  \tcbdimto\tcb@w@upper{\tcb@temp-\kvtcb@leftupper-\kvtcb@rightupper}%
  \tcbset{breakable@false}%
  \def\tcb@minipage{\csname tcb@minipage@\kvtcb@sbs@align\endcsname}%
  \tcbdimto\tcb@w@upper@real{\tcb@w@upper}%
  \tcbdimto\tcb@w@sbs{\tcb@w@upper@real-\kvtcb@sbs@gap}%
  \tcb@sbs@quota%
  \ifx\kvtcb@float\@empty%
    \let\tcb@before@unbroken=\kvtcb@beforebox%
    \let\tcb@after@unbroken=\kvtcb@afterbox%
  \else%
    \edef\tcb@before@unbroken{\noexpand\tcb@float@env@begin{tcbfloat}[\kvtcb@float]}%
    \let\tcb@after@unbroken=\tcb@float@env@end%
  \fi%
}

\def\tcb@use@lower@outside@side#1{%
  \setbox\z@=\hbox{\begin{tcb@lower@outside}{#1}%
    \tcb@use@listing@other@reset%
  \end{tcb@lower@outside}}%
  \tcb@box@align\z@%
  \tcbdimto{\tcb@temp@wd}{\wd\z@}%
  \unhbox\z@%
}

\def\tcb@inputlisting@out@listingAndOther{%
  \tcb@inputlisting@out@prepare%
  \tcbdimto\tcb@w@outside{\tcb@w@lower}%
  \tcbdimto\tcb@w@inside{\tcb@width-\tcb@w@lower-\kvtcb@sbs@gap}%
  \begin{tcb@outside@environment}%
  \setbox\z@=\hbox{\tcb@minipage{\tcb@w@inside}%
  \begin{tcolorbox}[width=\tcb@w@inside,nobeforeafter,nofloat,sidebyside=false,savedelimiter=tcolorbox]\tcbuselistinglisting\end{tcolorbox}%
  \endminipage}%
  \tcb@box@align\z@%
  \unhbox\z@%
  \kern\kvtcb@sbs@gap%
  \iftcb@lowervisible%
    \tcb@use@lower@outside@side{\tcb@w@outside}%
  \fi%
  \end{tcb@outside@environment}%
}

\def\tcb@inputlisting@out@otherAndListing{%
  \tcb@inputlisting@out@prepare%
  \tcbdimto\tcb@w@outside{\tcb@w@upper}%
  \tcbdimto\tcb@w@inside{\tcb@width-\tcb@w@upper-\kvtcb@sbs@gap}%
  \begin{tcb@outside@environment}%
  \iftcb@lowervisible%
    \tcb@use@lower@outside@side{\tcb@w@outside}%
    \tcbdimto{\tcb@temp@wd}{\tcb@w@outside-\tcb@temp@wd+\kvtcb@sbs@gap}%
  \else%
    \tcbdimto{\tcb@temp@wd}{\tcb@w@outside+\kvtcb@sbs@gap}%
  \fi%
  \kern\tcb@temp@wd%
  \setbox\z@=\hbox{\tcb@minipage{\tcb@w@inside}%
  \begin{tcolorbox}[width=\tcb@w@inside,nobeforeafter,nofloat,sidebyside=false,savedelimiter=tcolorbox]\tcbuselistinglisting\end{tcolorbox}%
  \endminipage}%
  \tcb@box@align\z@%
  \unhbox\z@%
  \end{tcb@outside@environment}%
}

\def\tcb@inputlisting@inside{%
  \begin{tcolorbox}[capture=\tcb@listing@capture,savedelimiter=tcolorbox]\tcb@listing@process\end{tcolorbox}%
}

\long\def\tcb@run@system@command#1{%
  \ifcase\pdf@shellescape\relax
    \tcb@error{You must invoke LaTeX with the -shell-escape flag}{Pass the -shell-escape flag to LaTeX.}%
  \or\or
    \tcb@warning{System call with restricted shell escape may fail}%
  \fi%
  \filename@parse{\kvtcb@listingfile}\immediate\write18{#1}%
  \relax%
}


\tcbset{%
  listing file/.store in=\kvtcb@listingfile,%
  comment/.store in=\kvtcb@listingcomment,%
  listing@process@inside/.code 2 args={%
    \let\tcb@inputlisting\tcb@inputlisting@inside%
    \let\tcb@listing@process=#1%
    \let\tcb@use@listing@other=#2},%
  listing@process@outside/.code 2 args={%
    \let\tcb@inputlisting=#1%
    \let\tcb@use@listing@other=#2},%
  listing only/.style={listing@process@inside={\tcb@listing@listing}{\tcbuselistingtext}},%
  text only/.style={listing@process@inside={\tcbuselistingtext}{\tcbuselistingtext}},%
  comment only/.style={listing@process@inside={\tcbuselistingcomment}{\tcbuselistingcomment}},%
  listing and text/.style={listing@process@inside={\tcb@listing@listingAndOther}{\tcbuselistingtext}},%
  text and listing/.style={listing@process@inside={\tcb@listing@otherAndListing}{\tcbuselistingtext}},%
  text above listing/.style={listing@process@outside={\tcb@inputlisting@out@otherAboveListing}{\tcbuselistingtext}},%
  text above* listing/.style={listing@process@outside={\tcb@inputlisting@out@otherAboveListing@Decoupled}{\tcbuselistingtext}},%
  listing above text/.style={listing@process@outside={\tcb@inputlisting@out@listingAboveOther}{\tcbuselistingtext}},%
  listing above* text/.style={listing@process@outside={\tcb@inputlisting@out@listingAboveOther@Decoupled}{\tcbuselistingtext}},%
  text outside listing/.style={listing@process@outside={\tcb@inputlisting@out@otherAndListing}{\tcbuselistingtext}},%
  listing outside text/.style={listing@process@outside={\tcb@inputlisting@out@listingAndOther}{\tcbuselistingtext}},%
  text side listing/.style={sidebyside,text and listing},%
  listing side text/.style={sidebyside,listing and text},%
  listing and comment/.style={listing@process@inside={\tcb@listing@listingAndOther}{\tcbuselistingcomment}},%
  comment and listing/.style={listing@process@inside={\tcb@listing@otherAndListing}{\tcbuselistingcomment}},%
  comment above listing/.style={listing@process@outside={\tcb@inputlisting@out@otherAboveListing}{\tcbuselistingcomment}},%
  comment above* listing/.style={listing@process@outside={\tcb@inputlisting@out@otherAboveListing@Decoupled}{\tcbuselistingcomment}},%
  listing above comment/.style={listing@process@outside={\tcb@inputlisting@out@listingAboveOther}{\tcbuselistingcomment}},%
  listing above* comment/.style={listing@process@outside={\tcb@inputlisting@out@listingAboveOther@Decoupled}{\tcbuselistingcomment}},%
  comment outside listing/.style={listing@process@outside={\tcb@inputlisting@out@otherAndListing}{\tcbuselistingcomment}},%
  listing outside comment/.style={listing@process@outside={\tcb@inputlisting@out@listingAndOther}{\tcbuselistingcomment}},%
  comment side listing/.style={sidebyside,comment and listing},%
  listing side comment/.style={sidebyside,listing and comment},%
  listing engine/.is choice,%
  image comment/.style 2 args={comment={\includegraphics[#1]{#2}}},%
  comment style/.store in=\kvtcb@commentstyle,%
  tcbimage comment/.style={comment={\let\tcb@trans@commentstyle\kvtcb@commentstyle\tcbincludegraphics[code={\pgfkeysalsofrom\tcb@trans@commentstyle}]{#1}}},
  pdf extension/.store in=\kvtcb@pdf@extension,%
  pdf comment/.style={comment={\let\tcb@trans@commentstyle\kvtcb@commentstyle\filename@parse{#1}\edef\tcb@trans@commentfile{\filename@area\filename@base.\kvtcb@pdf@extension}%
    \begin{tcbraster}[raster halign=center,sharp corners,size=tight,colback=white,code={\pgfkeysalsofrom\tcb@trans@commentstyle}]\tcbincludepdf{\tcb@trans@commentfile}\end{tcbraster}}},
  pdf comment/.default={\kvtcb@listingfile},
  process code/.code={\appto\tcb@listing@process@hook{#1}},%
  no process/.code={\def\tcb@listing@process@hook{}},%
  compilable listing/.style={listing file={\jobname-listing-\thetcblistingcount}},
  run system command/.style={process code={\tcb@run@system@command{#1}}},%
  run@system@command/.style 2 args={run system command={#1\space#2\space\filename@area\filename@base}},%
  run pdflatex/.style={run@system@command={pdflatex}{#1}},%
  run xelatex/.style={run@system@command={xelatex}{#1}},%
  run lualatex/.style={run@system@command={lualatex}{#1}},%
  run makeindex/.style={run@system@command={makeindex}{#1}},%
  run bibtex/.style={run@system@command={bibtex}{#1}},%
  run biber/.style={run@system@command={biber}{#1}},%
  run arara/.style={run@system@command={arara}{#1}},%
  run latex/.style={run@system@command={latex}{#1}},%
  run dvips/.style={run@system@command={dvips}{#1}},%
  run ps2pdf/.style={run system command={ps2pdf\space#1\space\filename@area\filename@base.ps}},%
}

\def\tcbinputlisting@core{%
  \tcb@listing@process@hook%
  \let\tcb@listing@capture=\kvtcb@capture%
  \tcb@inputlisting%
}

\newcounter{tcblisting}

\newenvironment{tcblisting}[1]{%
  \stepcounter{tcblisting}\edef\thetcblistingcount{\thetcblisting}%
  \tcb@layer@pushup%
  \tcb@apply@box@options{capture=minipage,#1}%
  \begingroup\tcbverbatimwrite{\kvtcb@listingfile}%
}{\endtcbverbatimwrite\endgroup%
  \tcbinputlisting@core%
}

\long\def\tcbinputlisting#1{%
  \begingroup%
  \stepcounter{tcblisting}\edef\thetcblistingcount{\thetcblisting}%
  \tcb@layer@pushup%
  \tcb@apply@box@options{capture=minipage,#1}%
  \tcbinputlisting@core%
  \endgroup%
}

\newenvironment{tcboutputlisting}{%
  \begingroup\tcbverbatimwrite{\kvtcb@listingfile}%
}{\endtcbverbatimwrite\endgroup}

\long\def\tcb@newtcblisting#1#2{\tcb@newenvironment{#1}{\tcblisting{#2,options@for=#1}}{\endtcblisting}}

\long\def\tcb@newtcblisting@#1[#2]#3{\tcb@newenvironment{#1}[#2]{\tcblisting{#3,options@for=#1}}{\endtcblisting}}

\long\def\tcb@newtcblisting@@#1[#2][#3]#4{\tcb@newenvironment{#1}[#2][#3]{\tcblisting{#4,options@for=#1}}{\endtcblisting}}

\long\def\tcb@new@tcblisting@#1[#2]{%
  \@ifnextchar[{\tcb@newtcblisting@@{#1}[#2]}{\tcb@newtcblisting@{#1}[#2]}}

\def\tcb@new@tcblisting#1{%
  \@ifnextchar[{\tcb@new@tcblisting@{#1}}{\tcb@newtcblisting{#1}}}

\def\newtcblisting{%
  \let\tcb@newenvironment\newenvironment%
  \let\tcb@process@newtcolorbox@continue\tcb@new@tcblisting%
  \tcb@process@newenvironment}

\def\renewtcblisting{%
  \let\tcb@newenvironment\renewenvironment%
  \let\tcb@process@newtcolorbox@continue\tcb@new@tcblisting%
  \tcb@process@newenvironment}

\long\def\tcb@newtcbinputlisting#1#2{\expandafter\tcb@newcommand\csname#1\endcsname{\tcbinputlisting{#2,options@for=#1}}}

\long\def\tcb@newtcbinputlisting@#1[#2]#3{\expandafter\tcb@newcommand\csname#1\endcsname[#2]{\tcbinputlisting{#3,options@for=#1}}}

\long\def\tcb@newtcbinputlisting@@#1[#2][#3]#4{\expandafter\tcb@newcommand\csname#1\endcsname[#2][#3]{\tcbinputlisting{#4,options@for=#1}}}

\long\def\tcb@new@tcbinputlisting@#1[#2]{%
  \@ifnextchar[{\tcb@newtcbinputlisting@@{#1}[#2]}{\tcb@newtcbinputlisting@{#1}[#2]}}

\def\tcb@new@tcbinputlisting#1{%
  \@ifnextchar[{\tcb@new@tcbinputlisting@{#1}}{\tcb@newtcbinputlisting{#1}}}

\def\newtcbinputlisting{%
  \let\tcb@newcommand\newcommand%
  \let\tcb@process@newtcolorbox@continue\tcb@new@tcbinputlisting%
  \tcb@process@newcommand}

\def\renewtcbinputlisting{%
  \let\tcb@newcommand\renewcommand%
  \let\tcb@process@newtcolorbox@continue\tcb@new@tcbinputlisting%
  \tcb@process@newcommand}

\tcbset{%
  reset@listingscore/.style={%
    listing file=\jobname.listing,
    comment=, listing and text,
    no process,comment style=,pdf extension=pdf,
  },
  initialize@reset=reset@listingscore,
}



==> tcblistingsutf8.code.tex <==
%% The LaTeX package tcolorbox - version 3.80 (2015/11/27)
%% tcblistingsutf8.code.tex: Code for colorboxes with listings in UTF-8
%%
%% -------------------------------------------------------------------------------------------
%% Copyright (c) 2006-2015 by Prof. Dr. Dr. Thomas F. Sturm <thomas dot sturm at unibw dot de>
%% -------------------------------------------------------------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2005/12/01 or later.
%%
%% This work has the LPPL maintenance status `author-maintained'.
%%
%% This work consists of all files listed in README
%%
\tcb@set@library@version{3.80}

\RequirePackage{listingsutf8}[2011/11/10]
\tcbuselibrary{listings}

\tcbset{
  listing utf8/.style={listing inputencoding=utf8/#1},
}

\tcbset{%
  reset@listingsutf8/.style={listing utf8=latin1},
  initialize@reset=reset@listingsutf8,
}



==> tcbmagazine.code.tex <==
%% The LaTeX package tcolorbox - version 3.80 (2015/11/27)
%% tcbmagazine.code.tex: Code for box sets and magazine styles
%%
%% -------------------------------------------------------------------------------------------
%% Copyright (c) 2006-2015 by Prof. Dr. Dr. Thomas F. Sturm <thomas dot sturm at unibw dot de>
%% -------------------------------------------------------------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2005/12/01 or later.
%%
%% This work has the LPPL maintenance status `author-maintained'.
%%
%% This work consists of all files listed in README
%%
\tcb@set@library@version{3.80}

\tcbuselibrary{breakable}

\def\newboxarray#1{%
  \ifcsdef{tcb@boxarray@#1@allocated}{%
    \tcb@warning{box array '#1' is allocated again by \string\newboxarray. Memory and registers are wasted}%
  }{}%
  \global\csdef{tcb@boxarray@#1@size}{0}%
  \global\csdef{tcb@boxarray@#1@allocated}{0}%
}

\newboxarray{default}

\newrobustcmd*{\boxarraygetsize}[2][default]{%
  \letcs#2{tcb@boxarray@#1@size}%
  \ifdef{#2}{}{%
    \tcb@error{undefined box array '#1'}%
    {You have to say \string\newboxarray{#1}, before '#1' can be used as box array.}%
  }%
}

\newrobustcmd*{\boxarrayreset}[1][default]{%
  \boxarraygetsize[#1]\tcb@box@array@size%
  \global\csdef{tcb@boxarray@#1@size}{0}%
}

\newrobustcmd*{\boxarrayclear}[1][default]{%
  \boxarraygetsize[#1]\tcb@box@array@size%
  \global\csdef{tcb@boxarray@#1@size}{0}%
  \letcs\tcb@box@array@allocated{tcb@boxarray@#1@allocated}%
  \begingroup%
    \count@=0%
    \loop%
    \ifnum\count@<\tcb@box@array@allocated\relax%
      \advance\count@ 1\relax%
      \letcs\tcb@box@array@box{tcb@boxarray@#1@\number\count@ @box}%
      \setbox0=\box\tcb@box@array@box%
    \repeat%
  \endgroup%
}

\newrobustcmd*{\boxarraygetbox}[3][default]{%
  \boxarraygetsize[#1]\tcb@box@array@size%
  \let#2\@undefined%
  \ifnum\numexpr#3>0\relax%
    \ifnum\numexpr#3>\tcb@box@array@size\relax%
    \else%
      \letcs#2{tcb@boxarray@#1@#3@box}%
    \fi%
  \fi%
}

\newrobustcmd*{\boxarraygetwidth}[3][default]{%
  \boxarraygetbox[#1]{\tcb@box@array@box}{#3}%
  \ifdefined\tcb@box@array@box%
    \tcbdimto#2{\wd\tcb@box@array@box}%
  \else%
    \let#2\tcb@zpt%
  \fi%
}

\newrobustcmd*{\boxarraygetheight}[3][default]{%
  \boxarraygetbox[#1]{\tcb@box@array@box}{#3}%
  \ifdefined\tcb@box@array@box%
    \tcbdimto#2{\ht\tcb@box@array@box}%
  \else%
    \let#2\tcb@zpt%
  \fi%
}

\newrobustcmd*{\boxarraygetdepth}[3][default]{%
  \boxarraygetbox[#1]{\tcb@box@array@box}{#3}%
  \ifdefined\tcb@box@array@box%
    \tcbdimto#2{\dp\tcb@box@array@box}%
  \else%
    \let#2\tcb@zpt%
  \fi%
}

\newrobustcmd*{\boxarraygettotalheight}[3][default]{%
  \boxarraygetbox[#1]{\tcb@box@array@box}{#3}%
  \ifdefined\tcb@box@array@box%
    \tcbdimto#2{\ht\tcb@box@array@box+\dp\tcb@box@array@box}%
  \else%
    \let#2\tcb@zpt%
  \fi%
}

\newrobustcmd*{\useboxarray}[2][default]{%
  \boxarraygetbox[#1]{\tcb@box@array@box}{#2}%
  \ifdefined\tcb@box@array@box%
    \usebox{\tcb@box@array@box}%
  \fi%
}

\newrobustcmd{\usetcboxarray}[3][default]{%
  \boxarraygetbox[#1]{\tcb@box@array@box}{#2}%
  \ifdefined\tcb@box@array@box%
    \tcbox[#3]{\usebox{\tcb@box@array@box}}%
  \fi%
}

\newrobustcmd*{\consumeboxarray}[2][default]{%
  \boxarraygetbox[#1]{\tcb@box@array@box}{#2}%
  \ifdefined\tcb@box@array@box%
    \leavevmode\box\tcb@box@array@box\relax%
  \fi%
}

\newrobustcmd{\consumetcboxarray}[3][default]{%
  \boxarraygetbox[#1]{\tcb@box@array@box}{#2}%
  \ifdefined\tcb@box@array@box%
    \tcbox[#3]{\leavevmode\box\tcb@box@array@box\relax}%
  \fi%
}

\def\boxarraystore#1{%
  \boxarraygetsize[#1]\tcb@box@array@size%
  \numdef\tcb@box@array@size{\tcb@box@array@size+1}%
  \global\cslet{tcb@boxarray@#1@size}{\tcb@box@array@size}%
  \letcs\tcb@box@array@allocated{tcb@boxarray@#1@allocated}%
  \ifnum\tcb@box@array@allocated<\tcb@box@array@size\relax%
    \newbox\tcb@box@array@box\csxdef{tcb@boxarray@#1@\tcb@box@array@size @box}{\the\tcb@box@array@box}%
    \global\cslet{tcb@boxarray@#1@allocated}{\tcb@box@array@size}%
  \else%
    \letcs\tcb@box@array@box{tcb@boxarray@#1@\tcb@box@array@size @box}%
  \fi%
  \edef\reserved@a{%
    \endgroup
    \global\setbox\tcb@box@array@box\hbox{%
      \begingroup\aftergroup}%
        \def\noexpand\@currenvir{\@currenvir}%
        \def\noexpand\@currenvline{\on@line}}%
  \reserved@a
    \@endpefalse
    \color@setgroup
      \ignorespaces}

\def\endboxarraystore{\unskip\color@endgroup}

\def\tcb@storetoboxarray@begin#1#2[#3]{\begin{boxarraystore}{#1}}
\def\tcb@storetoboxarray@end{\end{boxarraystore}}

\tcbset{
  store to box array/.code={%
    \def\kvtcb@float{S}\def\tcb@float@env@begin{\tcb@storetoboxarray@begin{#1}}\def\tcb@float@env@end{\tcb@storetoboxarray@end}},
  store to box array/.default=default,
  reset box array/.code={\boxarrayreset[#1]},
  reset box array/.default=default,
  reset and store to box array/.style={reset box array={#1},store to box array={#1}},%
  reset and store to box array/.default=default,
  do not store to box array/.style={nofloat},
}



==> tcbminted.code.tex <==
%% The LaTeX package tcolorbox - version 3.80 (2015/11/27)
%% tcbminted.code.tex: Code for colorboxes with listings
%%
%% -------------------------------------------------------------------------------------------
%% Copyright (c) 2006-2015 by Prof. Dr. Dr. Thomas F. Sturm <thomas dot sturm at unibw dot de>
%% -------------------------------------------------------------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2005/12/01 or later.
%%
%% This work has the LPPL maintenance status `author-maintained'.
%%
%% This work consists of all files listed in README
%%
%\makeatletter
\tcb@set@library@version{3.80}

\RequirePackage{minted}[2011/09/17]

\tcbuselibrary{listings@core}

\def\tcb@minted@input@listing#1#2#3#4{%
  \edef\temp@a{#4}%
  \ifx\temp@a\@empty%
  \else
    %\usemintedstyle{\temp@a}%
    \toks@=\expandafter{#4}%
    \edef\tcb@temp{\noexpand\usemintedstyle{\the\toks@}}%
    \tcb@temp%
  \fi%
  \toks@=\expandafter{#1}%
  \edef\tcb@temp{\noexpand\inputminted[\the\toks@]}%
  \tcb@temp{#2}{#3}%
}

\def\tcb@minted@uselistinglisting{%
  \tcb@minted@input@listing{\kvtcb@minted@options}{\kvtcb@minted@language}{\kvtcb@listingfile}{\kvtcb@minted@style}%
}%

\def\tcb@minted@usetemplisting{%
  \tcb@minted@input@listing{\kvtcb@minted@options}{\kvtcb@minted@language}{\kvtcb@tempfile}{\kvtcb@minted@style}%
}%

\def\tcb@minted@doc@usetemplisting{%
  \tcb@minted@input@listing{\kvtcb@docmintoptions}{latex}{\kvtcb@tempfile}{\kvtcb@docmintstyle}%
}

\tcbset{%
  minted language/.store in=\kvtcb@minted@language,
  minted options/.store in=\kvtcb@minted@options,
  minted style/.store in=\kvtcb@minted@style,
  listing engine/minted/.code={\let\tcbuselistinglisting\tcb@minted@uselistinglisting%
    \let\tcbusetemplisting\tcb@minted@usetemplisting%
    \let\tcb@doc@usetemplisting\tcb@minted@doc@usetemplisting},
}


\tcbset{%
  reset@minted/.style={%
    minted language=latex,
    minted options={tabsize=2,fontsize=\small},
    minted style=,
    listing engine=minted,
  },
  initialize@reset=reset@minted,
}



==> tcbraster.code.tex <==
%% The LaTeX package tcolorbox - version 3.80 (2015/11/27)
%% tcbskinsjigsaw.code.tex: Code for colorboxes with different skins
%%
%% -------------------------------------------------------------------------------------------
%% Copyright (c) 2006-2015 by Prof. Dr. Dr. Thomas F. Sturm <thomas dot sturm at unibw dot de>
%% -------------------------------------------------------------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2005/12/01 or later.
%%
%% This work has the LPPL maintenance status `author-maintained'.
%%
%% This work consists of all files listed in README
%%
\tcb@set@library@version{3.80}

\newcounter{tcbrastercolumn}
\newcounter{tcbrasterrow}
\newcounter{tcbraster}

\newrobustcmd{\thetcbrasternum}{\the\numexpr(\c@tcbrasterrow-1)*\kvtcb@raster@columns+\c@tcbrastercolumn\relax}

\def\tcb@raster@ehg@all{%
  \tcbset{equal height group={\kvtcb@raster@ehgid}}%
}

\def\tcb@raster@ehg@row{%
  \tcbset{equal height group={\kvtcb@raster@ehgid @\number\c@tcbrasterrow}}%
}


\tcbset{%
  raster columns/.store in=\kvtcb@raster@columns,
  raster rows/.store in=\kvtcb@raster@rows,
  raster width/.store in=\kvtcb@raster@width,
  raster height/.store in=\kvtcb@raster@height,
  %
  raster before skip/.store in=\kvtcb@raster@skip@before,
  raster after skip/.store in=\kvtcb@raster@skip@after,
  raster left skip/.store in=\kvtcb@raster@skip@left,
  raster right skip/.store in=\kvtcb@raster@skip@right,
  %
  raster column skip/.store in=\kvtcb@raster@xskip,
  raster row skip/.store in=\kvtcb@raster@yskip,
  %
  raster equal skip/.style={raster before skip=#1,raster after skip=#1,
    raster column skip=#1,raster row skip=#1},
  %
  raster@halign/.store in=\kvtcb@raster@halign,
  raster halign/.is choice,
  raster halign/center/.style={raster@halign=\centering},
  raster halign/left/.style={raster@halign=\raggedright},
  raster halign/right/.style={raster@halign=\raggedleft},
  %
  raster valign/.store in=\kvtcb@raster@valign,
  %
  raster equal height group/.store in=\kvtcb@raster@ehgid,%
  raster equal height/.is choice,
  raster equal height/.default=all,
  raster equal height/none/.code={\let\tcb@raster@ehg@start\@empty%
    \let\tcb@raster@ehg@continue\@empty},%
  raster equal height/rows/.code={\let\tcb@raster@ehg@start\tcb@raster@ehg@row%
    \let\tcb@raster@ehg@continue\tcb@raster@ehg@row},%
  raster equal height/all/.code={\let\tcb@raster@ehg@start\tcb@raster@ehg@all%
    \let\tcb@raster@ehg@continue\@empty},%
  %
  raster force size/.is choice,%
  raster force size/.default=true,%
  raster force size/true/.code={\let\tcb@raster@set@size\tcbset@late@options},%
  raster force size/false/.code={\let\tcb@raster@set@size\tcbset},%
}

\tcbset{
  raster reset/.style={
    raster width=\linewidth,raster height=0pt,
    raster equal skip=2mm,
    raster columns=2,raster rows=2,
    raster left skip=0pt,raster right skip=0pt,
    raster halign=left,raster valign=center,
    raster equal height=none,
    raster equal height group={REG@\tcb@raster@number},
    raster force size,},
  raster reset
}

\setcounter{tcbraster}{0}

\let\tcb@raster@change@minipage\@empty
\let\tcb@raster@change@fitbox\@empty
\def\tcb@raster@change@hbox{\tcbset{capture=minipage}}

\newenvironment{tcbraster}[1][]{%
  \tcb@layer@pushup%
  \stepcounter{tcbraster}%
  \edef\tcb@raster@number{\number\c@tcbraster}%
  \edef\tcb@raster@save@column{\number\c@tcbrastercolumn}%
  \edef\tcb@raster@save@row{\number\c@tcbrasterrow}%
  \let\tcb@raster@change@fitbox\@empty%
  \setcounter{tcbrastercolumn}{1}%
  \setcounter{tcbrasterrow}{1}%
  \tcbset{every box on layer \the\numexpr\number\c@tcblayer+1\relax/.code={%
    \tcbset{raster every box/.try}%
    \ifodd\c@tcbrastercolumn\relax%
      \tcbset{raster odd column/.try}%
    \else%
      \tcbset{raster even column/.try}%
    \fi%
    \tcbset{raster column \number\c@tcbrastercolumn/.try}%
    \ifodd\c@tcbrasterrow\relax%
      \tcbset{raster odd row/.try}%
    \else%
      \tcbset{raster even row/.try}%
    \fi%
    \tcbset{raster row \number\c@tcbrasterrow/.try}%
    \ifodd\thetcbrasternum\relax%
      \tcbset{raster odd number/.try}%
    \else%
      \tcbset{raster even number/.try}%
    \fi%
    \tcbset{raster row \number\c@tcbrasterrow\space column \number\c@tcbrastercolumn/.try}%
    \tcbset{raster number \thetcbrasternum/.try}%
  }}%
  \tcbset{#1}%
  \tcbset@late@options{%
    before={\ifhmode\unskip\fi\ifnum\c@tcbrastercolumn>1 \kern\kvtcb@raster@xskip\else%
      \ifnum\c@tcbrasterrow>1 \parindent\z@\parskip\z@\par\nointerlineskip\addvspace{\the\dimexpr\kvtcb@raster@yskip\relax}\noindent\fi%
      \kern\kvtcb@raster@skip@left\fi},
    after={%
      \ifnum\c@tcbrastercolumn=\kvtcb@raster@columns\relax%
        \kern\kvtcb@raster@skip@right%
        \setcounter{tcbrastercolumn}{1}\addtocounter{tcbrasterrow}{1}%
        \aftergroup\tcb@raster@ehg@continue%
      \else%
        \stepcounter{tcbrastercolumn}%
      \fi},%
    box align=\kvtcb@raster@valign,%
  }%
  \tcbdimto\tcb@raster@box@width{(\kvtcb@raster@width+\kvtcb@raster@xskip-\kvtcb@raster@skip@left-\kvtcb@raster@skip@right)/\kvtcb@raster@columns-\kvtcb@raster@xskip}%
  \tcb@raster@set@size{%
    code={\csuse{tcb@raster@change@\kvtcb@capture}},
    width=\tcb@raster@box@width,
  }%
  \ifdim\dimexpr\kvtcb@raster@height>0pt\relax%
    \tcbdimto\tcb@raster@box@height{(\kvtcb@raster@height+\kvtcb@raster@yskip-0.001pt)/\kvtcb@raster@rows-\kvtcb@raster@yskip}%
    \tcb@raster@set@size{height=\tcb@raster@box@height}%
  \fi%
  \tcb@raster@ehg@start%
  \let\tcb@end@raster\@empty%
  \ifinner\ifhmode%
    \color@vbox%
    \hsize=\kvtcb@raster@width%
    \let\tcb@end@raster\color@endbox%
  \fi\fi%&
  \if@nobreak%
    \iftcb@ignorenobreak%
      {\par\nointerlineskip%
      \addvspace{\glueexpr\kvtcb@raster@skip@before-\parskip}}%
    \fi%
  \else%
    {\par\nointerlineskip%
    \addvspace{\glueexpr\kvtcb@raster@skip@before-\parskip}}%
  \fi%
  \kvtcb@raster@halign\noindent%
}{%
  \ifhmode\unskip\fi%
  \ifnum\c@tcbrastercolumn>1 %
    \kern\kvtcb@raster@skip@right%
  \fi%
  \begingroup%
  \par\nointerlineskip%
  \addvspace{\glueexpr\kvtcb@raster@skip@after-\parskip}%
  \endgroup%
  \tcb@end@raster%
  \setcounter{tcbrastercolumn}{\tcb@raster@save@column}%
  \setcounter{tcbrasterrow}{\tcb@raster@save@row}%
}

\newcommand{\tcbitem@following}[1][]{%
  \end{tcolorbox}\begin{tcolorbox}[#1]%
}

\newcommand{\tcbitem@first}[1][]{%
  \let\tcbitem=\tcbitem@following%
  \begin{tcolorbox}[#1]%
}

\newenvironment{tcbitemize}[1][]{%
  \begin{tcbraster}[#1]%
  \let\tcb@raster@change@fitbox=\tcb@raster@change@hbox%
  \let\tcbitem=\tcbitem@first%
}{\end{tcolorbox}\end{tcbraster}}


==> tcbskins.code.tex <==
%% The LaTeX package tcolorbox - version 3.80 (2015/11/27)
%% tcbskins.code.tex: Code for colorboxes with different skins
%%
%% -------------------------------------------------------------------------------------------
%% Copyright (c) 2006-2015 by Prof. Dr. Dr. Thomas F. Sturm <thomas dot sturm at unibw dot de>
%% -------------------------------------------------------------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2005/12/01 or later.
%%
%% This work has the LPPL maintenance status `author-maintained'.
%%
%% This work consists of all files listed in README
%%
\tcb@set@library@version{3.80}

\RequirePackage{tikz}[2010/10/13]

\newenvironment{tikzpicture@tcb@hooked}{%
  \edef\tcb@tikzpicture@begin{\noexpand\tikzpicture[\expandonce\tcb@tikz@option@hook]}%
  \tcb@tikzpicture@begin\tcb@tikz@begin@hook}{\tcb@tikz@end@hook\endtikzpicture}

\def\tcb@creategeonodes@true{%
  \begin{scope}[every node/.style={line width=0mm,inner sep=0mm,outer sep=0mm,draw=none,fill=none,rectangle}]
    \node[name=frame,at={(0,0)},above right,minimum width=\tcb@width,minimum height=\tcb@height]{};
    \node[name=interior,at={({\kvtcb@left@rule},{\kvtcb@bottom@rule})},above right,minimum width=\tcb@innerwidth,minimum height=\tcb@innerheight]{};
    \ifnum\tcb@segment@state=1%
    \node[name=segmentation,at={({\kvtcb@left@rule},{\the\dimexpr\kvtcb@bottom@rule+\kvtcb@boxsep*2+\tcb@break@bottomsep+\kvtcb@bottom+\tcb@height@lower\relax})},above right,
       minimum width=\tcb@innerwidth,minimum height=\the\dimexpr\kvtcb@middle*2\relax]{};
    \else\iftcb@sidebyside%
    \node[name=segmentation,at={({\the\dimexpr\kvtcb@left@rule+\kvtcb@boxsep+\kvtcb@leftupper+\tcb@w@upper\relax},{\the\dimexpr\kvtcb@bottom@rule\relax})},above right,
       minimum width=\the\dimexpr\kvtcb@sbs@gap\relax,minimum height=\tcb@innerheight]{};
    \fi\fi%
    \iftcb@hasTitle%
    \node[name=title,at={({\kvtcb@left@rule},{\the\dimexpr\kvtcb@bottom@rule+\tcb@innerheight+\kvtcb@title@rule\relax})},above right,
       minimum width=\tcb@innerwidth,minimum height=\the\dimexpr\tcb@h@title+\kvtcb@toptitle+\kvtcb@bottomtitle+\kvtcb@boxsep*2\relax]{};
    \fi%
    \tcb@specialgeonodes@hook%
  \end{scope}%
}

\def\tcbsettowidthofnode#1#2{%
  \pgfpointanchor{#2}{east}\unskip%
  #1\pgf@x%
  \pgfpointanchor{#2}{west}\unskip%
  \advance #1 by -\pgf@x\relax%
}

\def\tcbsetmacrotowidthofnode#1#2{%
  \tcbsettowidthofnode\pgf@xa{#2}%
  \edef#1{\the\pgf@xa}%
}

\def\tcbsettoheightofnode#1#2{%
  \pgfpointanchor{#2}{north}\unskip%
  #1\pgf@y%
  \pgfpointanchor{#2}{south}\unskip%
  \advance #1 by -\pgf@y\relax%
}

\def\tcbsetmacrotoheightofnode#1#2{%
  \tcbsettoheightofnode\pgf@ya{#2}%
  \edef#1{\the\pgf@ya}%
}

\def\tcb@spec#1{\tikzset{tcb@spec/.style={#1}}}

\def\tcb@gettikzxy#1#2#3{%
  \tikz@scan@one@point\pgfutil@firstofone#1\relax%
  \edef#2{\the\pgf@x}%
  \edef#3{\the\pgf@y}%
}

\def\tcb@boundary@tikzbase#1#2#3#4#5#6{%
  \tcb@gettikzxy{(#1)}{\tcb@xa}{\tcb@ya}%
  \tcb@gettikzxy{(#2)}{\tcb@xb}{\tcb@yb}%
  \pgfpathmoveto{\pgfqpoint{\tcb@xa}{\tcb@ya}}%
  #4\pgfpathlineto{\pgfqpoint{\tcb@xa}{\tcb@yb}}%
  #5\pgfpathlineto{\pgfqpoint{\tcb@xb}{\tcb@yb}}%
  #6\pgfpathlineto{\pgfqpoint{\tcb@xb}{\tcb@ya}}%
  #3\pgfpathclose%
}

\def\tcb@pathboundary#1#2{\path[#1]\pgfextra{#2};}

\def\tcb@pathbase#1#2#3#4#5#6#7{\tcb@pathboundary{#1}{\tcb@boundary@tikzbase{#2}{#3}{#4}{#5}{#6}{#7}}}

\def\tcb@boundaryframe@pathfirst{%
  \tcb@boundary@base{0pt}{0pt}%
    {\tcb@width}{\tcb@height}%
    {\tcb@arc@zpt}{\tcb@arc@out@NW}{\tcb@arc@out@NE}{\tcb@arc@zpt}%
}

\def\tcb@boundaryframe@pathmiddle{%
  \tcb@boundary@base{0pt}{0pt}%
    {\tcb@width}{\tcb@height}%
    {\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}%
}

\def\tcb@boundaryframe@pathlast{%
  \tcb@boundary@base{0pt}{0pt}%
    {\tcb@width}{\tcb@height}%
    {\tcb@arc@out@SW}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@out@SE}%
}

\tikzset{%
  tcb fill frame/.style={fill=tcbcol@frame,fill opacity=\kvtcb@opacityframe,tcb@spec,frame@style},%
  tcb fill interior/.style={fill=tcbcol@back,fill opacity=\kvtcb@opacityback,tcb@spec,interior@style},%
  tcb fill title/.style={fill=tcbcol@backtitle,fill opacity=\kvtcb@opacitybacktitle,tcb@spec,title@style},%
}

% fill frame
\def\tcb@drawframe@path{\tcb@pathboundary{tcb fill frame}{\tcb@outerboundary}}
\let\tcb@drawframe@pathfirst=\tcb@drawframe@path
\let\tcb@drawframe@pathmiddle=\tcb@drawframe@path
\let\tcb@drawframe@pathlast=\tcb@drawframe@path


% fill inner box with title
\def\tcb@drawwithtitle@path{\tcb@pathboundary{tcb fill interior}{\tcb@boundaryinterior@title@standard}}

\def\tcb@drawwithtitle@pathfirst{%
  \tcb@pathbase{tcb fill interior}{interior.west|-frame.south}{interior.north east}%
    {\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}%
}

\let\tcb@drawwithtitle@pathmiddle=\tcb@drawwithtitle@pathfirst

\let\tcb@drawwithtitle@pathlast=\tcb@drawwithtitle@path

% fill inner box without title
\def\tcb@drawwithouttitle@path{\tcb@pathboundary{tcb fill interior}{\tcb@boundaryinterior@notitle@standard}}

\def\tcb@drawwithouttitle@pathfirst{%
  \tcb@pathbase{tcb fill interior}{interior.west|-frame.south}{interior.north east}%
    {\tcb@arc@zpt}{\tcb@arc@ins@NW}{\tcb@arc@ins@NE}{\tcb@arc@zpt}%
}

\def\tcb@drawwithouttitle@pathmiddle{%
  \tcb@pathbase{tcb fill interior}{interior.west|-frame.south}{interior.east|-frame.north}%
    {\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}%
}

\def\tcb@drawwithouttitle@pathlast{%
  \tcb@pathbase{tcb fill interior}{interior.south west}{interior.east|-frame.north}%
    {\tcb@arc@ins@SW}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@ins@SE}%
}

% draw title box
\def\tcb@drawtitle@path{\tcb@pathboundary{tcb fill title}{\tcb@boundarytitle@standard}}

\let\tcb@drawtitle@pathfirst=\tcb@drawtitle@path

\def\tcb@drawtitle@pathmiddle{%
  \tcb@pathbase{tcb fill title}{title.south west}{title.north east}%
    {\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}%
}

\let\tcb@drawtitle@pathlast=\tcb@drawtitle@pathmiddle

% draw segmentation line
\def\tcb@drawlower@path{%
  \iftcb@sidebyside%
    \path[draw=tcbcol@frame,fill opacity=\kvtcb@opacityframe,dash pattern=on 1mm off 1mm,dash phase=0.5mm,tcb@spec,segmentation@style]
    (segmentation.north)--(segmentation.south);%
  \else%
    \path[draw=tcbcol@frame,fill opacity=\kvtcb@opacityframe,dash pattern=on 1mm off 1mm,dash phase=0.5mm,tcb@spec,segmentation@style]
    (segmentation.west)--(segmentation.east);%
  \fi%
}

\def\tcb@draw@pseudo@segmentation#1{%
\begingroup\tcb@shield@externalize\begin{tikzpicture}%
  \path[use as bounding box] (0,{\the\dimexpr-\kvtcb@middle-\kvtcb@boxsep\relax})
     rectangle (\linewidth,{\the\dimexpr\kvtcb@middle+\kvtcb@boxsep\relax});
  \node[line width=0mm,inner sep=0mm,draw=none,fill=none,rectangle,
        name=segmentation,at={({\the\dimexpr-\kvtcb@boxsep-(#1)\relax},0)},right,%
        minimum width=\tcb@innerwidth,minimum height=\the\dimexpr\kvtcb@middle*2\relax]{};
  \tcb@drawlower@path%
\end{tikzpicture}\endgroup}

\def\tcbline@star#1{%
{\parskip\z@\par\nointerlineskip}%
\xleaders\vbox{\tcb@draw@pseudo@segmentation{#1}}\vskip\dimexpr(\kvtcb@middle+\kvtcb@boxsep)*2\relax%
{\parskip\z@\par\nointerlineskip}}

\def\tcbline@#1{%
{\parskip\z@\par\nointerlineskip}%
\tcb@draw@pseudo@segmentation{#1}%
{\parskip\z@\par\nointerlineskip}}

\def\tcbline{%
  \@ifstar{\iftcb@hasLower\tcbline@star{\kvtcb@leftlower}\else\tcbline@star{\kvtcb@leftupper}\fi}%
  {\iftcb@hasLower\tcbline@{\kvtcb@leftlower+\@totalleftmargin}\else\tcbline@{\kvtcb@leftupper+\@totalleftmargin}\fi}}


% draw special versions
\def\tcb@drawspec@UT{%
  \tcb@pathbase{tcb fill interior}{segmentation.west}{interior.north east}%
    {\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}%
}

\def\tcb@drawspec@UR{%
  \tcb@pathbase{tcb fill interior}{segmentation.west}{interior.north east}%
    {\tcb@arc@zpt}{\tcb@arc@ins@NW}{\tcb@arc@ins@NE}{\tcb@arc@zpt}%
}

\def\tcb@drawspec@US{%
  \tcb@pathbase{tcb fill interior}{segmentation.west}{interior.east|-frame.north}%
    {\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}%
}

\def\tcb@drawspec@LR#1{%
  \tcb@pathbase{#1,segmentation@style}{interior.south west}{[yshift=0.1mm]segmentation.east}%
    {\tcb@arc@ins@SW}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@ins@SE}%
}

\def\tcb@drawspec@LS#1{%
  \tcb@pathbase{#1,segmentation@style}{interior.west|-frame.south}{[yshift=0.1mm]segmentation.east}%
    {\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}%
}

\def\tcb@drawspec@sbs@A#1{%
  \tcb@pathbase{#1,segmentation@style}{segmentation.south}{interior.north east}%
    {\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@ins@NE}{\tcb@arc@ins@SE}%
}

\def\tcb@drawspec@sbs@B#1{%
  \tcb@pathbase{#1,segmentation@style}{segmentation.south}{interior.north east}%
    {\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@ins@SE}%
}

\def\tcb@drawspec@sbs@C#1{%
  \tcb@pathbase{#1,segmentation@style}{segmentation.south|-frame.south}{interior.north east}%
    {\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@ins@NE}{\tcb@arc@zpt}%
}

\def\tcb@drawspec@sbs@D#1{%
  \tcb@pathbase{#1,segmentation@style}{segmentation.south|-frame.south}{interior.north east}%
    {\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}%
}

\def\tcb@drawspec@sbs@E#1{%
  \tcb@pathbase{#1,segmentation@style}{segmentation.south|-frame.south}{interior.east|-frame.north}%
  {\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}%
}

\def\tcb@drawspec@sbs@F#1{%
  \tcb@pathbase{#1,segmentation@style}{segmentation.south}{interior.east|-frame.north}%
  {\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@ins@SE}%
}

\def\tcb@drawspec@T{%
  \tcb@pathbase{top color=tcbcol@frame,bottom color=tcbcol@back,fill opacity=\kvtcb@opacitybacktitle}{[yshift=-0.01pt]interior.north west}{[yshift=0.01pt]title.south east}%
  {\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}%
}

\def\tcb@drawframe@freelance{\tcb@frame@code}
\def\tcb@drawwithtitle@freelance{\tcb@interiortitled@code}
\def\tcb@drawwithouttitle@freelance{\tcb@interior@code}
\def\tcb@drawlower@freelance{\tcb@segmentation@code}
\def\tcb@drawtitle@freelance{\tcb@title@code}


\def\tcb@drawframe@spartan{%
  \begin{pgfscope}%
  \pgfpathrectangle{\pgfpointorigin}{\pgfqpoint{\tcb@width}{\tcb@height}}%
  \pgfsetfillcolor{tcbcol@frame}%
  \pgfsetfillopacity{\kvtcb@opacityframe}%
  \pgfusepath{fill}%
  \end{pgfscope}%
}

\def\tcb@drawwithtitle@spartan{%
  \begin{pgfscope}%
  \pgfpathrectanglecorners{\pgfqpoint{\kvtcb@left@rule}{\kvtcb@bottom@rule}}%
   {\pgfqpoint{\the\dimexpr\tcb@width-\kvtcb@right@rule\relax}{\the\dimexpr\kvtcb@bottom@rule+\tcb@innerheight\relax}}%
  \pgfsetfillcolor{tcbcol@back}%
  \pgfsetfillopacity{\kvtcb@opacityback}%
  \pgfusepath{fill}%
  \end{pgfscope}%
}

\def\tcb@drawwithouttitle@spartan{%
  \begin{pgfscope}%
  \pgfpathrectanglecorners{\pgfqpoint{\kvtcb@left@rule}{\kvtcb@bottom@rule}}%
   {\pgfqpoint{\the\dimexpr\tcb@width-\kvtcb@right@rule\relax}{\the\dimexpr\tcb@height-\kvtcb@top@rule\relax}}%
  \pgfsetfillcolor{tcbcol@back}%
  \pgfsetfillopacity{\kvtcb@opacityback}%
  \pgfusepath{fill}%
  \end{pgfscope}%
}

\def\tcb@drawtitle@spartan{%
  \begin{pgfscope}%
  \pgfpathrectanglecorners{\pgfqpoint{\kvtcb@left@rule}{\the\dimexpr\kvtcb@bottom@rule+\tcb@innerheight+\kvtcb@title@rule\relax}}%
   {\pgfqpoint{\the\dimexpr\tcb@width-\kvtcb@right@rule\relax}{\the\dimexpr\tcb@height-\kvtcb@top@rule\relax}}%
  \pgfsetfillcolor{tcbcol@backtitle}%
  \pgfsetfillopacity{\kvtcb@opacitybacktitle}%
  \pgfusepath{fill}%
  \end{pgfscope}%
}

\def\tcb@drawlower@spartan{%
  \begin{pgfscope}%
  \iftcb@sidebyside%
  \tcbdimto\tcb@seg@pos{\kvtcb@left@rule+\kvtcb@boxsep+\kvtcb@leftupper+\tcb@w@upper+\kvtcb@sbs@gap/2}%
  \pgfpathmoveto{\pgfqpoint{\tcb@seg@pos}{\the\dimexpr\kvtcb@bottom@rule+\tcb@innerheight\relax}}%
  \pgfpathlineto{\pgfqpoint{\tcb@seg@pos}{\kvtcb@bottom@rule}}%
  \else%
  \tcbdimto\tcb@seg@pos{\kvtcb@bottom@rule+\kvtcb@boxsep*2+\tcb@break@bottomsep+\kvtcb@middle+\kvtcb@bottom+\tcb@height@lower}%
  \pgfpathmoveto{\pgfqpoint{\kvtcb@left@rule}{\tcb@seg@pos}}%
  \pgfpathlineto{\pgfqpoint{\the\dimexpr\tcb@width-\kvtcb@right@rule\relax}{\tcb@seg@pos}}%
  \fi%
  \pgfsetcolor{tcbcol@frame}%
  \pgfsetstrokeopacity{\kvtcb@opacityframe}%
  \pgfusepath{stroke}%
  \end{pgfscope}%
}


\tcbset{%
  frame style/.code={\tikzset{frame@style/.style={#1}}},%
  frame hidden/.style={frame style={draw=none,fill=none}},
  frame engine/path/.style={frame code=\tcb@drawframe@path},
  frame engine/pathfirst/.style={frame code=\tcb@drawframe@pathfirst},
  frame engine/pathmiddle/.style={frame code=\tcb@drawframe@pathmiddle},
  frame engine/pathlast/.style={frame code=\tcb@drawframe@pathlast},
  frame engine/freelance/.style={frame code=\tcb@drawframe@standard},
  frame engine/spartan/.style={frame code=\tcb@drawframe@spartan},
  frame engine/empty/.style={frame code=},
  %
  interior titled engine/path/.style={interior titled code=\tcb@drawwithtitle@path},
  interior titled engine/pathfirst/.style={interior titled code=\tcb@drawwithtitle@pathfirst},
  interior titled engine/pathmiddle/.style={interior titled code=\tcb@drawwithtitle@pathmiddle},
  interior titled engine/pathlast/.style={interior titled code=\tcb@drawwithtitle@pathlast},
  interior titled engine/freelance/.style={interior titled code=\tcb@drawwithtitle@standard},
  interior titled engine/spartan/.style={interior titled code=\tcb@drawwithtitle@spartan},
  interior titled engine/empty/.style={interior titled code=},
  %
  interior engine/path/.style={interior code=\tcb@drawwithouttitle@path},
  interior engine/pathfirst/.style={interior code=\tcb@drawwithouttitle@pathfirst},
  interior engine/pathmiddle/.style={interior code=\tcb@drawwithouttitle@pathmiddle},
  interior engine/pathlast/.style={interior code=\tcb@drawwithouttitle@pathlast},
  interior engine/freelance/.style={interior code=\tcb@drawwithouttitle@standard},
  interior engine/spartan/.style={interior code=\tcb@drawwithouttitle@spartan},
  interior engine/empty/.style={interior code=},
  %
  segmentation engine/path/.style={segmentation code=\tcb@drawlower@path},
  segmentation engine/freelance/.style={segmentation code=\tcb@drawlower@standard},
  segmentation engine/spartan/.style={segmentation code=\tcb@drawlower@spartan},
  segmentation engine/empty/.style={segmentation code=},
  %
  title engine/path/.style={@title code=\tcb@drawtitle@path},
  title engine/pathfirst/.style={@title code=\tcb@drawtitle@pathfirst},
  title engine/pathmiddle/.style={@title code=\tcb@drawtitle@pathmiddle},
  title engine/pathlast/.style={@title code=\tcb@drawtitle@pathlast},
  title engine/freelance/.style={@title code=\tcb@drawtitle@standard},
  title engine/spartan/.style={@title code=\tcb@drawtitle@spartan},
  title engine/empty/.style={@title code=},
  %
  interior style/.code={\tikzset{interior@style/.style={#1}}},%
  interior hidden/.style={interior style={draw=none,fill=none}},
  segmentation style/.code={\tikzset{segmentation@style/.style={#1}}},%
  segmentation hidden/.style={segmentation style={draw=none,fill=none}},
  @title style/.code={\tikzset{title@style/.style={#1}}},%
  title style/.style={title filled,@title style={#1}},
  title hidden/.style={title style={draw=none,fill=none}},
  titlerule style/.style={%
    underlay={\iftcb@hasTitle%
      \path[draw,line width=\kvtcb@title@rule+1000sp,#1]
        ([yshift=-\kvtcb@title@rule/2]title.south west)--([yshift=-\kvtcb@title@rule/2]title.south east);
    \fi}},%
  colbacklower/.colorlet=tcbcol@backlower,%
  clear@spec/.code={\tcb@spec{}},%
  tikz/.code={\appto\tcb@tikz@option@hook{,#1}},%
  tikz reset/.code={\let\tcb@tikz@option@hook\@empty},%
  at begin tikz/.code={\appto\tcb@tikz@begin@hook{#1}},%
  at begin tikz reset/.code={\let\tcb@tikz@begin@hook\@empty},%
  at end tikz/.code={\appto\tcb@tikz@end@hook{#1}},%
  at end tikz reset/.code={\let\tcb@tikz@end@hook\@empty},%
  rotate/.style={tikz={rotate=#1,transform shape}},%
  scale/.style={tikz={scale=#1,transform shape},%
    at begin tikz={%
    \tcbdimto\kvtcb@arc{#1\dimexpr\kvtcb@arc}%
    \tcbdimto\tcb@outer@arc{#1\dimexpr\tcb@outer@arc}%
    \def\tcb@shadow@comp@arc{%
      \tcbdimto\tcb@shadow@ts{#1\dimexpr\tcb@shadow@ts}%
      \ifdim\dimexpr\tcb@outer@arc>\tcb@arc@scale\dimexpr\tcb@shadow@ts\relax%
        \tcbdimto\tcb@shadow@arc{\tcb@outer@arc-\tcb@arc@scale\dimexpr\tcb@shadow@ts\relax}%
      \else%
        \let\tcb@shadow@arc=\tcb@zpt%
      \fi%
    }%
    }},%
  remember/.style={tikz={remember picture}},%
  remember as/.style={tikz={remember picture},at end tikz={\pgfnodealias{#1}{frame}}},%
}

\tcbset{%
  base@unbroken/.style={%
    clear@spec,graphical environment=tikzpicture@tcb@hooked,geometry nodes,%
    set@outerboundary=\tcb@boundaryframe@standard,%
    shape@of@skin=unbroken,%
    set@extensions@preframe={\kvtcb@shadow},%
    set@extensions@postframe={\tcb@draw@border@unbroken\tcb@apply@underlay\tcb@apply@overlay},%
    set@extensions@final={\tcb@apply@finish}%
  },%
  base@first/.style={%
    clear@spec,graphical environment=tikzpicture@tcb@hooked,geometry nodes,%
    set@outerboundary=\tcb@boundaryframe@pathfirst,%
    shape@of@skin=first,%
    set@extensions@preframe={\kvtcb@shadow},%
    set@extensions@postframe={\tcb@draw@border@first\tcb@apply@underlay\tcb@apply@overlay},%
    set@extensions@final={\tcb@apply@finish}%
  },%
  base@middle/.style={%
    clear@spec,graphical environment=tikzpicture@tcb@hooked,geometry nodes,%
    set@outerboundary=\tcb@boundaryframe@pathmiddle,%
    shape@of@skin=middle,%
    set@extensions@preframe={\kvtcb@shadow},%
    set@extensions@postframe={\tcb@draw@border@middle\tcb@apply@underlay\tcb@apply@overlay},%
    set@extensions@final={\tcb@apply@finish}%
  },%
  base@last/.style={%
    clear@spec,graphical environment=tikzpicture@tcb@hooked,geometry nodes,%
    set@outerboundary=\tcb@boundaryframe@pathlast,%
    shape@of@skin=last,%
    set@extensions@preframe={\kvtcb@shadow},%
    set@extensions@postframe={\tcb@draw@border@last\tcb@apply@underlay\tcb@apply@overlay},%
    set@extensions@final={\tcb@apply@finish}%
  },%
}

\tcb@new@skin{enhanced}{base@unbroken,%
  frame engine=path,interior titled engine=path,interior engine=path,segmentation engine=path,title engine=path,%
  skin first=enhancedfirst,skin middle=enhancedmiddle,skin last=enhancedlast}

\tcb@new@skin{enhancedfirst}{base@first,%
  frame engine=pathfirst,interior titled engine=pathfirst,interior engine=pathfirst,segmentation engine=path,title engine=pathfirst,%
  skin first=enhancedfirst,skin middle=enhancedmiddle,skin last=enhancedmiddle}

\tcb@new@skin{enhancedmiddle}{base@middle,%
  frame engine=pathmiddle,interior titled engine=pathmiddle,interior engine=pathmiddle,segmentation engine=path,title engine=pathmiddle,%
  skin first=enhancedmiddle,skin middle=enhancedmiddle,skin last=enhancedmiddle}

\tcb@new@skin{enhancedlast}{base@last,%
  frame engine=pathlast,interior titled engine=pathlast,interior engine=pathlast,segmentation engine=path,title engine=pathlast,%
  skin first=enhancedmiddle,skin middle=enhancedmiddle,skin last=enhancedlast}

\tcbset{enhanced/.style={skin=enhanced},%
  enhanced standard/.style={skin=enhanced,
    skin first=enhanced,skin middle=enhanced,skin last=enhanced},%
  blank/.style={enhanced,frame hidden,interior hidden,segmentation hidden,%
    arc=0pt,outer arc=0pt,boxsep=0pt,top=0pt,bottom=0pt,left=0pt,right=0pt,boxrule=0pt,%
    bottomtitle=6pt,middle=3pt}}

\tcb@new@skin{empty}{base@unbroken,%
  frame engine=empty,interior titled engine=empty,interior engine=empty,segmentation engine=empty,title engine=empty,%
  skin first=emptyfirst,skin middle=emptymiddle,skin last=emptylast}

\tcb@new@skin{emptyfirst}{base@first,%
  frame engine=empty,interior titled engine=empty,interior engine=empty,segmentation engine=empty,title engine=empty,%
  skin first=emptyfirst,skin middle=emptymiddle,skin last=emptymiddle}

\tcb@new@skin{emptymiddle}{base@middle,%
  frame engine=empty,interior titled engine=empty,interior engine=empty,segmentation engine=empty,title engine=empty,%
  skin first=emptymiddle,skin middle=emptymiddle,skin last=emptymiddle}

\tcb@new@skin{emptylast}{base@last,%
  frame engine=empty,interior titled engine=empty,interior engine=empty,segmentation engine=empty,title engine=empty,%
  skin first=emptymiddle,skin middle=emptymiddle,skin last=emptylast}

\tcbset{empty/.style={skin=empty},%
  blanker/.style={empty,arc=0pt,outer arc=0pt,boxsep=0pt,top=0pt,bottom=0pt,left=0pt,right=0pt,boxrule=0pt,%
    bottomtitle=6pt,middle=3pt}}

\tcb@new@skin{freelance}{base@unbroken,%
  frame engine=freelance,interior titled engine=freelance,interior engine=freelance,segmentation engine=freelance,title engine=freelance,%
  skin first=freelancefirst,skin middle=freelancemiddle,skin last=freelancelast}%

\tcb@new@skin{freelancefirst}{base@first,%
  frame engine=freelance,interior titled engine=freelance,interior engine=freelance,segmentation engine=freelance,title engine=freelance,%
  skin first=freelancefirst,skin middle=freelancemiddle,skin last=freelancemiddle}%

\tcb@new@skin{freelancemiddle}{base@middle,%
  frame engine=freelance,interior titled engine=freelance,interior engine=freelance,segmentation engine=freelance,title engine=freelance,%
  skin first=freelancemiddle,skin middle=freelancemiddle,skin last=freelancemiddle}%

\tcb@new@skin{freelancelast}{base@last,%
  frame engine=freelance,interior titled engine=freelance,interior engine=freelance,segmentation engine=freelance,title engine=freelance,%
  skin first=freelancemiddle,skin middle=freelancemiddle,skin last=freelancelast}%

\tcbset{freelance/.style={skin=freelance},
  % for backward compatibility:
  extend freelance/.style={#1},%
  extend freelancefirst/.style={skin first is subskin of={freelancefirst}{#1}},%
  extend freelancemiddle/.style={skin middle is subskin of={freelancemiddle}{#1}},%
  extend freelancelast/.style={skin last is subskin of={freelancelast}{#1}}}

\tcb@new@skin{bicolor}{base@unbroken,%
  frame engine=path,interior titled engine=empty,interior engine=empty,segmentation engine=empty,title engine=path,%
  interior titled code={%
    \iftcb@lowerseparated%
      \ifcase\tcb@segment@state%
      {\tcb@spec{fill=tcbcol@back}\tcb@drawwithtitle@path}%
      \or%
      \tcb@spec{fill=tcbcol@back}\tcb@drawspec@UT%
      \else%
      {\tcb@spec{fill=tcbcol@backlower}\tcb@drawwithtitle@path}%
      \fi%
    \else%
      {\tcb@spec{fill=tcbcol@back}\tcb@drawwithtitle@path}%
    \fi\tcb@spec{}},
  interior code={%
    \iftcb@lowerseparated%
      \ifcase\tcb@segment@state%
      {\tcb@spec{fill=tcbcol@back}\tcb@drawwithouttitle@path}%
      \or%
      \tcb@spec{fill=tcbcol@back}\tcb@drawspec@UR%
      \else%
      {\tcb@spec{fill=tcbcol@backlower}\tcb@drawwithouttitle@path}%
      \fi%
    \else%
      {\tcb@spec{fill=tcbcol@back}\tcb@drawwithouttitle@path}%
    \fi\tcb@spec{}},
  segmentation code={\iftcb@sidebyside%
    \iftcb@hasTitle\tcb@drawspec@sbs@B{fill=tcbcol@backlower}\else%
    \tcb@drawspec@sbs@A{fill=tcbcol@backlower}\fi\else\tcb@drawspec@LR{fill=tcbcol@backlower}\fi\tcb@spec{}},%
  skin first=bicolorfirst,skin middle=bicolormiddle,skin last=bicolorlast}

\tcbset{bicolor/.style={skin=bicolor}}

\tcb@new@skin{bicolorfirst}{base@first,%
  frame engine=pathfirst,interior titled engine=empty,interior engine=empty,segmentation engine=empty,title engine=pathfirst,%
  interior titled code={%
    \iftcb@lowerseparated%
      \ifcase\tcb@segment@state%
      {\tcb@spec{fill=tcbcol@back}\tcb@drawwithtitle@pathfirst}%
      \or%
      \tcb@spec{fill=tcbcol@back}\tcb@drawspec@UT%
      \else%
      {\tcbset{interior style=}\tcb@spec{fill=tcbcol@backlower}\tcb@drawwithtitle@pathfirst}%
      \fi%
    \else%
      {\tcb@spec{fill=tcbcol@back}\tcb@drawwithtitle@pathfirst}%
    \fi\tcb@spec{}},
  interior code={%
    \iftcb@lowerseparated%
      \ifcase\tcb@segment@state%
      {\tcb@spec{fill=tcbcol@back}\tcb@drawwithouttitle@pathfirst}%
      \or%
      \tcb@spec{fill=tcbcol@back}\tcb@drawspec@UR%
      \else%
      {\tcbset{interior style=}\tcb@spec{fill=tcbcol@backlower}\tcb@drawwithouttitle@pathfirst}%
      \fi%
    \else%
      {\tcb@spec{fill=tcbcol@back}\tcb@drawwithouttitle@pathfirst}%
    \fi\tcb@spec{}},
  segmentation code={\iftcb@sidebyside%
    \iftcb@hasTitle\tcb@drawspec@sbs@D{fill=tcbcol@backlower}\else%
    \tcb@drawspec@sbs@C{fill=tcbcol@backlower}\fi\else\tcb@drawspec@LS{fill=tcbcol@backlower}\fi\tcb@spec{}},%
  skin first=bicolorfirst,skin middle=bicolormiddle,skin last=bicolormiddle}

\tcb@new@skin{bicolormiddle}{base@middle,%
  frame engine=pathmiddle,interior titled engine=empty,interior engine=empty,segmentation engine=empty,title engine=pathmiddle,%
  interior titled code={%
    \iftcb@lowerseparated%
      \ifcase\tcb@segment@state%
      {\tcb@spec{fill=tcbcol@back}\tcb@drawwithtitle@pathmiddle}%
      \or%
      \tcb@spec{fill=tcbcol@back}\tcb@drawspec@UT%
      \else%
      {\tcbset{interior style=}\tcb@spec{fill=tcbcol@backlower}\tcb@drawwithtitle@pathmiddle}%
      \fi%
    \else%
      {\tcb@spec{fill=tcbcol@back}\tcb@drawwithtitle@pathmiddle}%
    \fi\tcb@spec{}},%
  interior code={%
    \iftcb@lowerseparated%
      \ifcase\tcb@segment@state%
      {\tcb@spec{fill=tcbcol@back}\tcb@drawwithouttitle@pathmiddle}%
      \or%
      \tcb@spec{fill=tcbcol@back}\tcb@drawspec@US%
      \else%
      {\tcbset{interior style=}\tcb@spec{fill=tcbcol@backlower}\tcb@drawwithouttitle@pathmiddle}%
      \fi%
    \else%
      {\tcb@spec{fill=tcbcol@back}\tcb@drawwithouttitle@pathmiddle}%
    \fi\tcb@spec{}},
  segmentation code={\iftcb@sidebyside%
    \iftcb@hasTitle\tcb@drawspec@sbs@D{fill=tcbcol@backlower}\else%
    \tcb@drawspec@sbs@E{fill=tcbcol@backlower}\fi\else\tcb@drawspec@LS{fill=tcbcol@backlower}\fi\tcb@spec{}},%
  skin first=bicolormiddle,skin middle=bicolormiddle,skin last=bicolormiddle}

\tcb@new@skin{bicolorlast}{base@last,%
  frame engine=pathlast,interior titled engine=empty,interior engine=empty,segmentation engine=empty,title engine=pathlast,%
  interior titled code={%
    \iftcb@lowerseparated%
      \ifcase\tcb@segment@state
      {\tcb@spec{fill=tcbcol@back}\tcb@drawwithtitle@pathlast}%
      \or%
      \tcb@spec{fill=tcbcol@back}\tcb@drawspec@UT%
      \else%
      {\tcbset{interior style=}\tcb@spec{fill=tcbcol@backlower}\tcb@drawwithtitle@pathlast}%
      \fi%
    \else%
      {\tcb@spec{fill=tcbcol@back}\tcb@drawwithtitle@pathlast}%
    \fi\tcb@spec{}},
  interior code={%
    \iftcb@lowerseparated%
      \ifcase\tcb@segment@state%
      {\tcb@spec{fill=tcbcol@back}\tcb@drawwithouttitle@pathlast}%
      \or%
      \tcb@spec{fill=tcbcol@back}\tcb@drawspec@US%
      \else
      {\tcbset{interior style=}\tcb@spec{fill=tcbcol@backlower}\tcb@drawwithouttitle@pathlast}%
      \fi%
    \else%
      {\tcb@spec{fill=tcbcol@back}\tcb@drawwithouttitle@pathlast}%
    \fi\tcb@spec{}},%
  segmentation code={\iftcb@sidebyside%
    \iftcb@hasTitle\tcb@drawspec@sbs@B{fill=tcbcol@backlower}\else%
    \tcb@drawspec@sbs@F{fill=tcbcol@backlower}\fi\else\tcb@drawspec@LR{fill=tcbcol@backlower}\fi\tcb@spec{}},%
  skin first=bicolormiddle,skin middle=bicolormiddle,skin last=bicolorlast}


\tikzset{beamer@color/.style={fill=none,top color=tcbcol@back,bottom color=tcbcol@back!85!black}}

\tcb@new@skin{beamer}{base@unbroken,%
  frame engine=path,interior titled engine=empty,interior engine=empty,segmentation engine=empty,title engine=path,%
  interior titled code={%
    \iftcb@lowerseparated%
      \ifnum\tcb@segment@state=1%
      \tcb@spec{beamer@color}\tcb@drawspec@UT%
      \else%
      {\tcb@spec{beamer@color}\tcb@drawwithtitle@path}%
      \fi%
    \else%
      {\tcb@spec{beamer@color}\tcb@drawwithtitle@path}%
    \fi%
    \tcb@drawspec@T\tcb@spec{}},
  interior code={%
    \iftcb@lowerseparated%
      \ifnum\tcb@segment@state=1
      \tcb@spec{beamer@color}\tcb@drawspec@UR%
      \else%
      {\tcb@spec{beamer@color}\tcb@drawwithouttitle@path}%
      \fi%
    \else%
      {\tcb@spec{beamer@color}\tcb@drawwithouttitle@path}%
    \fi\tcb@spec{}},
  segmentation code={\iftcb@sidebyside\tcb@drawlower@path\else\tcb@drawspec@LR{beamer@color}\fi\tcb@spec{}},%
  skin first=beamerfirst,skin middle=beamermiddle,skin last=beamerlast}

\tcbset{beamer/.style={skin=beamer,boxrule=0mm,titlerule=1mm,toptitle=0.5mm,arc=2mm,fonttitle=\bfseries,drop fuzzy shadow}}

\tcb@new@skin{beamerfirst}{base@first,%
  frame engine=pathfirst,interior titled engine=empty,interior engine=empty,segmentation engine=empty,title engine=pathfirst,%
  interior titled code={%
    \iftcb@lowerseparated%
      \ifnum\tcb@segment@state=1%
      \tcb@spec{beamer@color}\tcb@drawspec@UT%
      \else%
      {\tcb@spec{beamer@color}\tcb@drawwithtitle@pathfirst}%
      \fi%
    \else%
      {\tcb@spec{beamer@color}\tcb@drawwithtitle@pathfirst}%
    \fi%
    \tcb@drawspec@T\tcb@spec{}},%
  interior code={%
    \iftcb@lowerseparated%
      \ifnum\tcb@segment@state=1
      \tcb@spec{beamer@color}\tcb@drawspec@UR%
      \else%
      {\tcb@spec{beamer@color}\tcb@drawwithouttitle@pathfirst}%
      \fi%
    \else%
      {\tcb@spec{beamer@color}\tcb@drawwithouttitle@pathfirst}%
    \fi\tcb@spec{}},
  segmentation code={\iftcb@sidebyside\tcb@drawlower@path\else\tcb@drawspec@LS{beamer@color}\fi\tcb@spec{}},%
  skin first=beamerfirst,skin middle=beamermiddle,skin last=beamermiddle}

\tcb@new@skin{beamermiddle}{base@middle,%
  frame engine=pathmiddle,interior titled engine=empty,interior engine=empty,segmentation engine=empty,title engine=pathmiddle,%
  interior titled code={%
    \iftcb@lowerseparated%
      \ifnum\tcb@segment@state=1%
      \tcb@spec{beamer@color}\tcb@drawspec@UT%
      \else%
      {\tcb@spec{beamer@color}\tcb@drawwithtitle@pathmiddle}%
      \fi%
    \else%
      {\tcb@spec{beamer@color}\tcb@drawwithtitle@pathmiddle}%
    \fi%
    \tcb@drawspec@T\tcb@spec{}},%
  interior code={%
    \iftcb@lowerseparated%
      \ifnum\tcb@segment@state=1
      \tcb@spec{beamer@color}\tcb@drawspec@US%
      \else%
      {\tcb@spec{beamer@color}\tcb@drawwithouttitle@pathmiddle}%
      \fi%
    \else%
      {\tcb@spec{beamer@color}\tcb@drawwithouttitle@pathmiddle}%
    \fi\tcb@spec{}},
  segmentation code={\iftcb@sidebyside\tcb@drawlower@path\else\tcb@drawspec@LS{beamer@color}\fi\tcb@spec{}},%
  skin first=beamermiddle,skin middle=beamermiddle,skin last=beamermiddle}

\tcb@new@skin{beamerlast}{base@last,%
  frame engine=pathlast,interior titled engine=empty,interior engine=empty,segmentation engine=empty,title engine=pathlast,%
  interior titled code={%
    \iftcb@lowerseparated%
      \ifnum\tcb@segment@state=1%
      \tcb@spec{beamer@color}\tcb@drawspec@UT%
      \else%
      {\tcb@spec{beamer@color}\tcb@drawwithtitle@pathlast}%
      \fi%
    \else%
      {\tcb@spec{beamer@color}\tcb@drawwithtitle@pathlast}%
    \fi%
    \tcb@drawspec@T\tcb@spec{}},%
  interior code={%
    \iftcb@lowerseparated%
      \ifnum\tcb@segment@state=1
      \tcb@spec{beamer@color}\tcb@drawspec@US%
      \else%
      {\tcb@spec{beamer@color}\tcb@drawwithouttitle@pathlast}%
      \fi%
    \else%
      {\tcb@spec{beamer@color}\tcb@drawwithouttitle@pathlast}%
    \fi\tcb@spec{}},
  segmentation code={\iftcb@sidebyside\tcb@drawlower@path\else\tcb@drawspec@LR{beamer@color}\fi\tcb@spec{}},%
  skin first=beamermiddle,skin middle=beamermiddle,skin last=beamerlast}

\def\tcb@drawspec@widgetsegment{%
  \iftcb@sidebyside%
  \tcb@drawlower@path%
  \else%
  \path[left color=tcbcol@frame!75!white,right color=tcbcol@frame!75!white!25!tcbcol@back,segmentation@style]
    ([yshift={-\kvtcb@middle/4}]segmentation.west) rectangle ([yshift={\kvtcb@middle/4}]segmentation.east);
  \fi%
}

\tikzset{widget@color/.style={left color=tcbcol@frame!75!white,right color=tcbcol@frame!75!white!25!tcbcol@back}}

\tcb@new@skin{widget}{base@unbroken,%
  frame engine=path,interior titled engine=path,interior engine=path,segmentation engine=empty,title engine=empty,%
  title code={{\tcb@spec{widget@color}\tcb@drawtitle@path}},
  segmentation code={\tcb@drawspec@widgetsegment},%
  skin first=widgetfirst,skin middle=widgetmiddle,skin last=widgetlast}

\tcbset{widget/.style={skin=widget,arc=0.5mm,fonttitle=\bfseries,titlerule=0mm,toprule at break=0mm}}

\tcb@new@skin{widgetfirst}{base@first,%
  frame engine=pathfirst,interior titled engine=pathfirst,interior engine=pathfirst,segmentation engine=empty,title engine=empty,%
  title code={{\tcb@spec{widget@color}\tcb@drawtitle@pathfirst}},%
  segmentation code={\tcb@drawspec@widgetsegment},%
  skin first=widgetfirst,skin middle=widgetmiddle,skin last=widgetmiddle}

\tcb@new@skin{widgetmiddle}{base@middle,%
  frame engine=pathmiddle,interior titled engine=pathmiddle,interior engine=pathmiddle,segmentation engine=empty,title engine=empty,%
  title code={{\tcb@spec{widget@color}\tcb@drawtitle@pathmiddle}},%
  segmentation code={\tcb@drawspec@widgetsegment},%
  skin first=widgetmiddle,skin middle=widgetmiddle,skin last=widgetmiddle}

\tcb@new@skin{widgetlast}{base@last,%
  frame engine=pathlast,interior titled engine=pathlast,interior engine=pathlast,segmentation engine=empty,title engine=empty,%
  title code={{\tcb@spec{widget@color}\tcb@drawtitle@pathlast}},
  segmentation code={\tcb@drawspec@widgetsegment},%
  skin first=widgetmiddle,skin middle=widgetmiddle,skin last=widgetlast}

\tcb@new@skin{spartan}{graphical environment=tikzpicture@tcb@hooked,geometry nodes=true,shape@of@skin=unbroken,%
  set@extensions@preframe=,set@extensions@postframe={\tcb@apply@underlay},set@extensions@final=,%
  frame engine=spartan,interior titled engine=spartan,interior engine=spartan,title engine=spartan,segmentation engine=spartan,%
  set@outerboundary=\tcb@boundaryframe@standard,%
  skin first=spartan,skin middle=spartan,skin last=spartan}

\tcbset{spartan/.style={skin=spartan}}

\tcb@new@skin{draft}{clear@spec,graphical environment=tikzpicture@tcb@hooked,geometry nodes,shape@of@skin=unbroken,%
  frame engine=empty,interior titled engine=empty,interior engine=empty,segmentation engine=path,title empty,%
  segmentation style={draw=black,dashed},
  set@extensions@postframe=,
  set@extensions@final={\tcb@apply@finish},no finish,%
  colupper=black!50!white,collower=black!50!white,coltitle=black!50!white,
  frame code={%
    \path[draw=blue!10!white,double,line width=1pt,dashed] (current bounding box.south west) rectangle (current bounding box.north east);
    {\tcb@spec{fill=black!15!white,draw=black}\tcb@drawframe@path}%
    \iftcb@hasTitle%
      \path[fill=red!10!white,draw,dotted,rounded corners=\kvtcb@arc]
        ([xshift={\kvtcb@left@rule},yshift={\kvtcb@bottom@rule}]frame.south west) rectangle
        (interior.north east);
      \path[fill=red!10!white,draw,dotted,rounded corners=\kvtcb@arc]
        ([yshift={\kvtcb@title@rule}]interior.north west) rectangle
        ([xshift={-\kvtcb@right@rule},yshift={-\kvtcb@top@rule}]frame.north east);
      \path[fill=white,draw,dotted]
        ([xshift={\kvtcb@boxsep},yshift={\kvtcb@boxsep}]title.south west) rectangle
        ([xshift={-\kvtcb@boxsep},yshift={-\kvtcb@boxsep}]title.north east);
      \path[fill=green!20!white,draw=green!75!black,dashed]
        ([xshift={\kvtcb@boxsep+\kvtcb@lefttitle},yshift={\kvtcb@boxsep+\kvtcb@bottomtitle}]title.south west)
         rectangle node[font=\scriptsize] {title: w=\tcb@w@title, h=\tcb@h@title}
        +(\tcb@w@title,\tcb@h@title);
      \path[draw=red,opacity=0.5] (title.south west) rectangle (title.north east);
    \else%
      \path[fill=red!10!white,draw,dotted,rounded corners=\kvtcb@arc]
        ([xshift={\kvtcb@left@rule},yshift={\kvtcb@bottom@rule}]frame.south west) rectangle
        ([xshift={-\kvtcb@right@rule},yshift={-\kvtcb@top@rule}]frame.north east);
    \fi%
    \ifcase\tcb@segment@state
      \path[fill=white,draw,dotted]
        ([xshift={\kvtcb@boxsep},yshift={\kvtcb@boxsep+\tcb@break@bottomsep}]interior.south west) rectangle
        ([xshift={-\kvtcb@boxsep},yshift={-\kvtcb@boxsep-\tcb@break@topsep}]interior.north east);
      \path[fill=green!20!white,draw=green!75!black,dashed]
        ([xshift={\kvtcb@boxsep+\kvtcb@leftupper},yshift={\kvtcb@boxsep+\kvtcb@bottom+\tcb@break@bottomsep}]interior.south west)
        rectangle node[font=\scriptsize] {upper: w=\tcb@w@upper, h=\tcb@height@upper}
        +(\tcb@w@upper,\tcb@height@upper);
      \iftcb@sidebyside%
      \path[fill=green!20!white,draw=green!75!black,dashed]
        ([yshift={\kvtcb@boxsep+\kvtcb@bottom+\tcb@break@bottomsep}]segmentation.south east)
        rectangle node[font=\scriptsize] {lower: w=\tcb@w@lower, h=\tcb@height@upper}
        +(\tcb@w@lower,\tcb@height@upper);
      \fi%
    \or%
      \ifdim\wd\tcb@upperbox=0pt\relax
        \path[fill=white,draw,dotted]
          ([xshift={\kvtcb@boxsep},yshift={\kvtcb@boxsep+\tcb@break@bottomsep}]interior.south west) rectangle
          ([xshift={-\kvtcb@boxsep},yshift={-\kvtcb@boxsep-\tcb@break@topsep}]interior.north east);
      \else
        \path[fill=white,draw,dotted]
          ([xshift={\kvtcb@boxsep},yshift={\kvtcb@boxsep+\tcb@break@bottomsep}]interior.south west) rectangle
          ([xshift={-\kvtcb@boxsep},yshift={-\kvtcb@boxsep}]segmentation.east);
        \path[fill=white,draw,dotted]
           ([xshift={\kvtcb@boxsep},yshift={\kvtcb@boxsep}]segmentation.west)
           rectangle ([xshift={-\kvtcb@boxsep},yshift={-\kvtcb@boxsep-\tcb@break@topsep}]interior.north east);
        \path[fill=green!20!white,draw=green!75!black,dashed]
          ([xshift={\kvtcb@boxsep+\kvtcb@leftupper},yshift={\kvtcb@boxsep}]segmentation.north west)
           rectangle node[font=\scriptsize] {upper: w=\tcb@w@upper, h=\tcb@height@upper}
           +(\tcb@w@upper,\tcb@height@upper);
      \fi%
      \path[fill=green!20!white,draw=green!75!black,dashed]
        ([xshift={\kvtcb@boxsep+\kvtcb@leftlower},yshift={\kvtcb@boxsep+\kvtcb@bottom+\tcb@break@bottomsep}]interior.south west)
        rectangle  node[font=\scriptsize] {lower: w=\tcb@w@lower, h=\tcb@height@lower}
        +(\tcb@w@lower,\tcb@height@lower);
      \path[draw=red,opacity=0.5] (segmentation.south west) rectangle (segmentation.north east);
    \else
      \path[fill=white,draw,dotted]
        ([xshift={\kvtcb@boxsep},yshift={\kvtcb@boxsep+\tcb@break@bottomsep}]interior.south west) rectangle
        ([xshift={-\kvtcb@boxsep},yshift={-\kvtcb@boxsep-\tcb@break@topsep}]interior.north east);
      \path[fill=green!20!white,draw=green!75!black,dashed]
        ([xshift={\kvtcb@boxsep+\kvtcb@leftlower},yshift={\kvtcb@boxsep+\kvtcb@bottom+\tcb@break@bottomsep}]interior.south west)
        rectangle  node[font=\scriptsize] {lower: w=\tcb@w@lower, h=\tcb@height@lower}
        +(\tcb@w@lower,\tcb@height@lower);
    \fi%
    \path[draw=red,opacity=0.5] (interior.south west) rectangle (interior.north east);
    \path[draw=red,opacity=0.5] (frame.south west) rectangle (frame.north east);
    \node[above,font=\scriptsize,red!50!black] at (interior.south) {interior: w=\tcb@innerwidth, h=\tcb@innerheight};
    \node[above,font=\scriptsize,red!50!black] at (frame.north) {frame: w=\the\dimexpr\tcb@width\relax, h=\tcb@height};
    \path[draw=blue!10!white,double,line width=1pt,dashed,opacity=0.3] (current bounding box.south west) rectangle (current bounding box.north east);
    \pgfsetfillopacity{0.3}
  },
  skin first=draft,skin middle=draft,skin last=draft}

\tcbset{draft/.style={skin=draft}}

\tikzset{%
  tcb@forced@clip/.code={\tikz@addmode{\tikz@mode@cliptrue}\let\tikz@options=\pgfutil@empty},%
  tcb@invclip/.style={clip,insert path={{[reset cm]\pgfextra{%
    \pgfpathmoveto{\pgfqpoint{-16383.99999pt}{-16383.99999pt}}%
    \pgfpathlineto{\pgfqpoint{16383.99999pt}{-16383.99999pt}}%
    \pgfpathlineto{\pgfqpoint{16383.99999pt}{16383.99999pt}}%
    \pgfpathlineto{\pgfqpoint{-16383.99999pt}{16383.99999pt}}%
    \pgfpathclose}}}}%
}%

\def\tcb@clip@frame{\tcb@pathboundary{clip}{\tcb@outerboundary}}

\def\tcb@invclip@frame{\tcb@pathboundary{tcb@invclip}{\tcb@outerboundary}}

\def\tcb@clip@interior{%
  \begingroup%
  \tcbset{interior hidden}%
  \tcb@spec{tcb@forced@clip}%
  \def\tcb@spec##1{}%
  \iftcb@hasTitle%
    \tcb@interiortitled@code%
  \else%
    \tcb@interior@code%
  \fi%
  \endgroup%
}

\def\tcb@clip@title{%
  \begingroup%
  \tcbset{title hidden}%
  \tcb@spec{tcb@forced@clip}%
  \def\tcb@spec##1{}%
    \iftcb@hasTitle%
      \tcb@title@code%
    \fi%
  \endgroup%
}

\newenvironment{tcbclipframe}{\begin{scope}\tcb@clip@frame}{\end{scope}}
\newenvironment{tcbinvclipframe}{\begin{scope}\tcb@invclip@frame}{\end{scope}}
\newenvironment{tcbclipinterior}{\begin{scope}\tcb@clip@interior}{\end{scope}}
\newenvironment{tcbcliptitle}{\begin{scope}\tcb@clip@title}{\end{scope}}

\def\tcb@apply@underlay{\csname tcb@underlay@\tcb@split@state\endcsname}%
\def\tcb@apply@finish{\csname tcb@finish@\tcb@split@state\endcsname}%

\tcbset{%
  underlay unbroken/.code={\appto\tcb@underlay@unbroken{#1}},%
  underlay first/.code={\appto\tcb@underlay@first{#1}},%
  underlay middle/.code={\appto\tcb@underlay@middle{#1}},%
  underlay last/.code={\appto\tcb@underlay@last{#1}},%
  underlay boxed title/.code={\appto\tcb@underlay@boxedtitle{#1}},%
  underlay/.style={underlay unbroken={#1},underlay first={#1},underlay middle={#1},underlay last={#1}},%
  underlay broken/.style={underlay first={#1},underlay middle={#1},underlay last={#1}},%
  underlay unbroken and first/.style={underlay unbroken={#1},underlay first={#1}},%
  underlay unbroken and last/.style={underlay unbroken={#1},underlay last={#1}},%
  underlay middle and last/.style={underlay middle={#1},underlay last={#1}},%
  underlay first and middle/.style={underlay first={#1},underlay middle={#1}},%
  no underlay unbroken/.code={\let\tcb@underlay@unbroken\@empty},%
  no underlay first/.code={\let\tcb@underlay@first\@empty},%
  no underlay middle/.code={\let\tcb@underlay@middle\@empty},%
  no underlay last/.code={\let\tcb@underlay@last\@empty},%
  no underlay boxed title/.code={\let\tcb@underlay@boxedtitle\@empty},%
  no underlay/.style={no underlay unbroken,no underlay first,no underlay middle,no underlay last,no underlay boxed title},%
  finish unbroken/.code={\appto\tcb@finish@unbroken{#1}},%
  finish first/.code={\appto\tcb@finish@first{#1}},%
  finish middle/.code={\appto\tcb@finish@middle{#1}},%
  finish last/.code={\appto\tcb@finish@last{#1}},%
  finish/.style={finish unbroken={#1},finish first={#1},finish middle={#1},finish last={#1}},%
  finish broken/.style={finish first={#1},finish middle={#1},finish last={#1}},%
  finish unbroken and first/.style={finish unbroken={#1},finish first={#1}},%
  finish unbroken and last/.style={finish unbroken={#1},finish last={#1}},%
  finish middle and last/.style={finish middle={#1},finish last={#1}},%
  finish first and middle/.style={finish first={#1},finish middle={#1}},%
  no finish unbroken/.code={\let\tcb@finish@unbroken\@empty},%
  no finish first/.code={\let\tcb@finish@first\@empty},%
  no finish middle/.code={\let\tcb@finish@middle\@empty},%
  no finish last/.code={\let\tcb@finish@last\@empty},%
  no finish/.style={no finish unbroken,no finish first,no finish middle,no finish last},%
}


\tcbset{%
  before@boxed@title/.store in=\kvtcb@before@boxedtitle,%
  after@boxed@title/.store in=\kvtcb@after@boxedtitle,%
  boxed title style/.store in=\kvtcb@style@boxedtitle,%
  %
  varwidth boxed title/.style={before@boxed@title={\tcbdimto\tcb@w@title{#1}\begin{varwidth}{\tcb@w@title}},after@boxed@title={\end{varwidth}}},%
  varwidth boxed title/.default={\kvtcb@width-\kvtcb@left@rule-\kvtcb@right@rule-\kvtcb@boxsep*2-\kvtcb@lefttitle-\kvtcb@righttitle},
  varwidth boxed title*/.style={varwidth boxed title={\kvtcb@width+#1}},
  varwidth boxed title*/.default={-\kvtcb@left@rule-\kvtcb@right@rule-\kvtcb@boxsep*2-\kvtcb@lefttitle-\kvtcb@righttitle},
  %
  minipage boxed title/.style={before@boxed@title={\tcbdimto\tcb@w@title{#1}\begin{minipage}{\tcb@w@title}},after@boxed@title={\end{minipage}}},%
  minipage boxed title/.default={\kvtcb@width-\kvtcb@left@rule-\kvtcb@right@rule-\kvtcb@boxsep*2-\kvtcb@lefttitle-\kvtcb@righttitle},
  minipage boxed title*/.style={minipage boxed title={\kvtcb@width+#1}},
  minipage boxed title*/.default={-\kvtcb@left@rule-\kvtcb@right@rule-\kvtcb@boxsep*2-\kvtcb@lefttitle-\kvtcb@righttitle},
  %
  tikznode boxed title/.style={before@boxed@title={\centering\tcb@shield@externalize\begin{tikzpicture}\node[align=center,inner sep=0pt,outer sep=0pt,#1]\bgroup},after@boxed@title={\egroup;\end{tikzpicture}}},%
  hbox boxed title/.style={before@boxed@title=,after@boxed@title=},%
  %
  boxtitle/xshift/.dimstore in=\kvtcb@xshift@boxedtitle,%
  boxtitle/yshift/.dimstore in=\kvtcb@yshift@boxedtitle,%
  boxtitle/yshifttext/.dimstore in=\kvtcb@yinnershift@boxedtitle,%
  %
  boxtitle/yshift*@top/.style={yshift*/.code={%
    \tcbdimto\kvtcb@yshift@boxedtitle{##1}%
    \tcbdimto\kvtcb@yinnershift@boxedtitle{\kvtcb@yshift@boxedtitle+\kvtcb@top@rule@stand}%
    \ifdim\dimexpr\kvtcb@yinnershift@boxedtitle>0pt\relax\let\kvtcb@yinnershift@boxedtitle\tcb@zpt\fi%
  }},
  boxtitle/yshift*@bottom/.style={yshift*/.code={%
    \tcbdimto\kvtcb@yshift@boxedtitle{##1}%
    \tcbdimto\kvtcb@yinnershift@boxedtitle{\kvtcb@yshift@boxedtitle-\kvtcb@bottom@rule@stand}%
    \ifdim\dimexpr\kvtcb@yinnershift@boxedtitle<0pt\relax\let\kvtcb@yinnershift@boxedtitle\tcb@zpt\fi%
  }},
  boxtitle/adapt@top/.code={%
    \ifdim\dimexpr\tcboxedtitleheight+\kvtcb@yshift@boxedtitle>0pt\relax
      \tcbdimto\kvtcb@bbtop@stand{\kvtcb@bbtop@stand+\tcboxedtitleheight+\kvtcb@yshift@boxedtitle}%
    \fi%
    \tcbdimto\kvtcb@top{\kvtcb@top-\kvtcb@yinnershift@boxedtitle}%
  },
  boxtitle/adapt@bottom/.code={%
    \ifdim\dimexpr\tcboxedtitleheight-\kvtcb@yshift@boxedtitle>0pt\relax
      \tcbdimto\kvtcb@bbbottom@stand{\kvtcb@bbbottom@stand+\tcboxedtitleheight-\kvtcb@yshift@boxedtitle}%
    \fi%
    \tcbdimto\kvtcb@bottom{\kvtcb@bottom+\kvtcb@yinnershift@boxedtitle}%
  },
  attach@title@boxed/.style n args={5}{%
    detach title,
    code={\def\tcb@specialtitle@hook{%
      \ifx\tcbtitletext\@empty\else%
      \colorlet{tcbtranscol@frame}{tcbcol@frame}%
      \colorlet{tcbtranscol@back}{tcbcol@backtitle}%
      \let\tcb@trans@boxedstyle\kvtcb@style@boxedtitle%
      \setbox\tcb@titlebox\color@hbox\bgroup\color{tcbcol@title}\kvtcb@fonttitle\kvtcb@haligntitle\kvtcb@before@boxedtitle\kvtcb@before@title\tcbtitletext\kvtcb@after@title\kvtcb@after@boxedtitle\egroup\color@endbox%
      \setbox\tcb@titlebox\color@hbox\tcbox[colframe=tcbtranscol@frame,colback=tcbtranscol@back,size=title,code={\pgfkeysalsofrom\tcb@trans@boxedstyle}]{\box\tcb@titlebox}\color@endbox%
      %
      \tcbdimto\tcboxedtitleheight{\ht\tcb@titlebox+\dp\tcb@titlebox}%
      \tcbdimto\tcboxedtitlewidth{\wd\tcb@titlebox}%
      \tcbset{boxtitle/.cd,xshift=0pt,yshift=0pt,yshifttext=0pt,yshift*@#2,#1,adapt@#2}%
      \let\tcb@specialgeonodes@first\relax%
      \let\tcb@specialgeonodes@middle\relax%
      \let\tcb@specialgeonodes@last\relax%
      \def\tcb@specialgeonodes@unbroken{%
        \node[#4,name=title,at={([xshift=\kvtcb@xshift@boxedtitle,yshift=\kvtcb@yshift@boxedtitle]frame.#5)},
                minimum width=\tcboxedtitlewidth,minimum height=\tcboxedtitleheight]{};}%
      \cslet{tcb@specialgeonodes@#3}{\tcb@specialgeonodes@unbroken}%
      \def\tcb@specialgeonodes@hook{\csname tcb@specialgeonodes@\tcb@split@state\endcsname}%
      \preto\tcb@underlay@unbroken{\tcb@underlay@boxedtitle\pgftext[at={\pgfpointanchor{title}{center}}]{\box\tcb@titlebox}}%
      \cspreto{tcb@underlay@#3}{\tcb@underlay@boxedtitle\pgftext[at={\pgfpointanchor{title}{center}}]{\box\tcb@titlebox}}%
      \fi}}%
    },
  attach@title@boxed@top/.style n args={3}{attach@title@boxed={#1}{top}{first}{#2}{#3}},%
  attach@title@boxed@bottom/.style n args={3}{attach@title@boxed={#1}{bottom}{last}{#2}{#3}},%
  %
  attach boxed title to top left/.style={attach@title@boxed@top={#1}{above right}{north west}},
  attach boxed title to top center/.style={attach@title@boxed@top={#1}{above}{north}},
  attach boxed title to top right/.style={attach@title@boxed@top={#1}{above left}{north east}},
  attach boxed title to bottom left/.style={attach@title@boxed@bottom={#1}{below right}{south west}},
  attach boxed title to bottom center/.style={attach@title@boxed@bottom={#1}{below}{south}},
  attach boxed title to bottom right/.style={attach@title@boxed@bottom={#1}{below left}{south east}},
}


\newbox\tcb@waterbox

\def\tcb@setratio#1#2#3{\edef#1{\strip@pt\dimexpr\number\numexpr\number\dimexpr#2\relax*65536/\number\dimexpr#3\relax\relax sp\relax}}

\def\tcb@setratiorobust#1#2#3{\ifdim\dimexpr#3<1pt\tcb@setratio#1{#2}{1pt}\else\tcb@setratio#1{#2}{#3}\fi}

\def\tcb@comp@waterbox@stretch#1#2#3{%
  \tcb@setratiorobust\tcb@scale@x{#1\dimexpr#2}{\wd\tcb@waterbox}%
  \tcb@setratiorobust\tcb@scale@y{#1\dimexpr#3}{\ht\tcb@waterbox+\dp\tcb@waterbox}%
}

\def\tcb@comp@waterbox@zoom#1#2#3{%
  \tcb@comp@waterbox@stretch{#1}{#2}{#3}%
  \ifdim\dimexpr\tcb@scale@x pt\relax<\dimexpr\tcb@scale@y pt\relax\let\tcb@scale@y=\tcb@scale@x\else\let\tcb@scale@x=\tcb@scale@y\fi%
}

\def\tcb@comp@waterbox@overzoom#1#2#3{%
  \tcb@comp@waterbox@stretch{#1}{#2}{#3}%
  \ifdim\dimexpr\tcb@scale@x pt\relax>\dimexpr\tcb@scale@y pt\relax\let\tcb@scale@y=\tcb@scale@x\else\let\tcb@scale@x=\tcb@scale@y\fi%
}

\def\tcb@comp@waterbox@shrink#1#2#3{%
  \tcb@comp@waterbox@zoom{#1}{#2}{#3}%
  \ifdim\dimexpr\tcb@scale@x pt\relax>1pt\relax%
    \edef\tcb@scale@x{1}\edef\tcb@scale@y{1}%
  \fi%
}

\def\tcb@box@scaled@waterbox{\scalebox{\tcb@scale@x}[\tcb@scale@y]{\box\tcb@waterbox}}

\def\tcb@drawspec@watermark@@noclip{%
  \tcb@comp@wm%
  \node[opacity=\kvtcb@watermark@opacity,anchor=center] at (interior) {\tcb@box@scaled@waterbox};%
}

\def\tcb@drawspec@watermark@@clip{%
  \begin{tcbclipinterior}%
  \tcb@drawspec@watermark@@noclip%
  \end{tcbclipinterior}%
}

\def\tcb@drawspec@watermark@tikz#1{%
  \setbox\tcb@waterbox=\color@hbox\pgfinterruptpicture{\pgfsetbaseline{0pt}\begin{tikzpicture}[color=\kvtcb@watermark@color]#1\end{tikzpicture}}\endpgfinterruptpicture\color@endbox%
  \tcb@drawspec@watermark%
}

\def\tcb@drawspec@watermark@graphics#1{%
  \setbox\tcb@waterbox=\color@hbox\pgfinterruptpicture{\includegraphics{#1}}\endpgfinterruptpicture\color@endbox%
  \tcb@drawspec@watermark%
}

\def\tcb@drawspec@watermark@text#1{%
  \tcb@drawspec@watermark@tikz{\node[inner sep=0pt,align=flush center]{#1};}%
}


\tcbset{%
  watermark opacity/.store in=\kvtcb@watermark@opacity,%
  watermark color/.store in=\kvtcb@watermark@color,%
%
  watermark stretch/.code={\def\tcb@comp@wm{\tcb@comp@waterbox@stretch{#1}{\tcb@innerwidth}{\tcb@innerheight}}},%
  watermark zoom/.code={\def\tcb@comp@wm{\tcb@comp@waterbox@zoom{#1}{\tcb@innerwidth}{\tcb@innerheight}}},%
  watermark overzoom/.code={\def\tcb@comp@wm{\tcb@comp@waterbox@overzoom{#1}{\tcb@innerwidth}{\tcb@innerheight}}},%
  watermark shrink/.code={\def\tcb@comp@wm{\tcb@comp@waterbox@shrink{#1}{\tcb@innerwidth}{\tcb@innerheight}}},%
%
  watermark tikz/.style={overlay={\tcb@drawspec@watermark@tikz{#1}}},
  watermark tikz on/.style args={#1 is #2}{overlay #1={\tcb@drawspec@watermark@tikz{#2}}},%
  watermark graphics/.style={overlay={\tcb@drawspec@watermark@graphics{#1}}},
  watermark graphics on/.style args={#1 is #2}{overlay #1={\tcb@drawspec@watermark@graphics{#2}}},
  watermark text/.style={overlay={\tcb@drawspec@watermark@text{#1}}},
  watermark text on/.style args={#1 is #2}{overlay #1={\tcb@drawspec@watermark@text{#2}}},
  no watermark/.style={no overlay},
  clip watermark/.is choice,
  clip watermark/true/.code={\let\tcb@drawspec@watermark=\tcb@drawspec@watermark@@clip},
  clip watermark/false/.code={\let\tcb@drawspec@watermark=\tcb@drawspec@watermark@@noclip},
  clip watermark/.default=true,
  show bounding box/.style={border@line app={%
    \path[preaction={draw,line width=0.1pt,#1},draw,double=white,line width=1pt,dashed,opacity=0.5,#1]
    (current bounding box.south west) rectangle (current bounding box.north east);}},%
  show bounding box/.default={red},%
}

\def\tcb@tdraw@title@clip{%
  \begin{tcbcliptitle}%
  \tcb@tdraw@title@core%
  \end{tcbcliptitle}%
}

\def\tcb@tdraw@upper@clip{%
  \begin{tcbclipinterior}%
  \tcb@tdraw@upper@core%
  \end{tcbclipinterior}%
}

\def\tcb@tdraw@lower@clip{%
  \begin{tcbclipinterior}%
  \tcb@tdraw@lower@core%
  \end{tcbclipinterior}%
}


\def\tcb@process@ppbb{%
  \pgf@process{\pgfpointanchor{path picture bounding box}{south west}}%
  \pgf@xa\pgf@x\pgf@ya\pgf@y%
  \pgf@process{\pgfpointanchor{path picture bounding box}{north east}}%
  \pgf@xb\pgf@x\pgf@yb\pgf@y%
  \pgfsetfillopacity{\tcb@tikz@fill@graphics@opacity}%
  \pgfsetstrokeopacity{\tcb@tikz@fill@graphics@opacity}%
}

\def\tcb@process@ppbb@wh{%
  \tcb@process@ppbb%
  \tcbdimto\tcb@ppbb@width{\pgf@xb-\pgf@xa}%
  \tcbdimto\tcb@ppbb@height{\pgf@yb-\pgf@ya}%
}

\def\tcb@set@waterbox@to@graphics#1{%
  \setbox\tcb@waterbox=\color@hbox\pgfinterruptpicture{\expandafter\includegraphics\expandafter[\tcb@tikz@fill@graphics@options]{#1}}\endpgfinterruptpicture\color@endbox%
}

\def\tcb@set@waterbox@to@picture#1{%
  \setbox\tcb@waterbox=\color@hbox\pgfinterruptpicture{\pgfsetbaseline{0pt}\begin{tikzpicture}#1\end{tikzpicture}}\endpgfinterruptpicture\color@endbox%
}

\tikzset{%
  fill image opacity/.store in=\tcb@tikz@fill@graphics@opacity,%
  fill image opacity=1,%
  fill image scale/.store in=\tcb@tikz@fill@graphics@scale,%
  fill image scale=1,%
  fill image options/.store in=\tcb@tikz@fill@graphics@options,%
  fill image options=,%
  fill plain image/.style={path picture={%
    \node at (path picture bounding box.center) {\expandafter\includegraphics\expandafter[\tcb@tikz@fill@graphics@options]{#1}};
  }},
  fill plain picture/.style={path picture={%
    \tcb@set@waterbox@to@picture{#1}%
    \node at (path picture bounding box.center) {\box\tcb@waterbox};
  }},
  fill stretch image/.style={path picture={%
    \tcb@process@ppbb@wh%
    \node at (path picture bounding box.center) {\expandafter\includegraphics\expandafter[\tcb@tikz@fill@graphics@options,%
      width=\the\dimexpr\tcb@tikz@fill@graphics@scale\dimexpr\tcb@ppbb@width\relax,%
      height=\the\dimexpr\tcb@tikz@fill@graphics@scale\dimexpr\tcb@ppbb@height\relax]{#1}};
  }},
  fill stretch picture/.style={path picture={%
    \tcb@process@ppbb@wh%
    \tcb@set@waterbox@to@picture{#1}%
    \tcb@comp@waterbox@stretch{\tcb@tikz@fill@graphics@scale}{\tcb@ppbb@width}{\tcb@ppbb@height}%
    \node at (path picture bounding box.center) {\tcb@box@scaled@waterbox};%
  }},
  fill@overzoom/.style={path picture={%
    \tcb@process@ppbb@wh%
    #1%
    \tcb@comp@waterbox@overzoom{\tcb@tikz@fill@graphics@scale}{\tcb@ppbb@width}{\tcb@ppbb@height}%
    \node at (path picture bounding box.center) {\tcb@box@scaled@waterbox};%
  }},
  fill overzoom image/.style={fill@overzoom={\tcb@set@waterbox@to@graphics{#1}}},%
  fill overzoom picture/.style={fill@overzoom={\tcb@set@waterbox@to@picture{#1}}},%
  fill@zoom/.style={path picture={%
    \tcb@process@ppbb@wh%
    #1%
    \tcb@comp@waterbox@zoom{\tcb@tikz@fill@graphics@scale}{\tcb@ppbb@width}{\tcb@ppbb@height}%
    \node at (path picture bounding box.center) {\tcb@box@scaled@waterbox};%
  }},
  fill zoom image/.style={fill@zoom={\tcb@set@waterbox@to@graphics{#1}}},%
  fill zoom picture/.style={fill@zoom={\tcb@set@waterbox@to@picture{#1}}},%
  fill@shrink/.style={path picture={%
    \tcb@process@ppbb@wh%
    #1%
    \tcb@comp@waterbox@shrink{\tcb@tikz@fill@graphics@scale}{\tcb@ppbb@width}{\tcb@ppbb@height}%
    \node at (path picture bounding box.center) {\tcb@box@scaled@waterbox};%
  }},
  fill shrink image/.style={fill@shrink={\tcb@set@waterbox@to@graphics{#1}}},%
  fill shrink picture/.style={fill@shrink={\tcb@set@waterbox@to@picture{#1}}},%
  fill@tile/.style={path picture={%
    \tcb@process@ppbb%
    #1%
    \tcbdimto\tcb@ppbb@tilew{\wd\tcb@waterbox}%
    \tcbdimto\tcb@ppbb@tileh{\ht\tcb@waterbox+\dp\tcb@waterbox}%
    \pgf@xc\pgf@xa\pgf@yc\pgf@yb%
    \pgfutil@loop%
      \pgfutil@loop%
        \pgftext[x=\pgf@xc,y=\pgf@yc,left,top]{\copy\tcb@waterbox}%
        \ifdim\pgf@xc<\pgf@xb%
        \advance\pgf@xc\tcb@ppbb@tilew%
      \pgfutil@repeat%
      \ifdim\pgf@yc>\pgf@ya%
      \advance\pgf@yc-\tcb@ppbb@tileh%
      \pgf@xc\pgf@xa%
    \pgfutil@repeat%
  }},%
  fill tile image/.style={fill@tile={\tcb@set@waterbox@to@graphics{#1}}},%
  fill tile picture/.style={fill@tile={\tcb@set@waterbox@to@picture{#1}}},%
  fill tile picture*/.style 2 args={fill@tile={\tcb@set@waterbox@to@picture{#2}%
    \setbox\tcb@waterbox=\color@hbox\scalebox{#1}{\box\tcb@waterbox}\color@endbox}},%
  %
  fill plain image*/.style 2 args={fill image options={#1},fill plain image={#2}},%
  fill stretch image*/.style 2 args={fill image options={#1},fill stretch image={#2}},%
  fill overzoom image*/.style 2 args={fill image options={#1},fill overzoom image={#2}},%
  fill zoom image*/.style 2 args={fill image options={#1},fill zoom image={#2}},%
  fill shrink image*/.style 2 args={fill image options={#1},fill shrink image={#2}},%
  fill tile image*/.style 2 args={fill image options={#1},fill tile image={#2}},%
}

\tcbset{%
  frame style image/.style={frame style={fill=none,fill stretch image={#1}}},
  frame style tile/.style 2 args={frame style={fill=none,fill tile image*={#1}{#2}}},
  interior style image/.style={interior style={fill=none,fill stretch image={#1}}},
  interior style tile/.style 2 args={interior style={fill=none,fill tile image*={#1}{#2}}},
  title style image/.style={title style={fill=none,fill stretch image={#1}}},
  title style tile/.style 2 args={title style={fill=none,fill tile image*={#1}{#2}}},
}

\tcbset{%
  clip title/.is choice,
  clip title/true/.code={\let\tcb@tdraw@title=\tcb@tdraw@title@clip},
  clip title/false/.code={\let\tcb@tdraw@title=\tcb@tdraw@title@core},
  clip title/.default=true,
  clip upper/.is choice,
  clip upper/true/.code={\let\tcb@tdraw@upper=\tcb@tdraw@upper@clip},
  clip upper/false/.code={\let\tcb@tdraw@upper=\tcb@tdraw@upper@core},
  clip upper/.default=true,
  clip lower/.is choice,
  clip lower/true/.code={\let\tcb@tdraw@lower=\tcb@tdraw@lower@clip},
  clip lower/false/.code={\let\tcb@tdraw@lower=\tcb@tdraw@lower@core},
  clip lower/.default=true,
}


\tcbset{marker/.style={%
  skin=enhancedmiddle jigsaw,
  breakable,parbox=false,
  boxrule=0mm,leftrule=5mm,rightrule=5mm,boxsep=0mm,
  left=3mm,right=3mm,top=1mm,bottom=1mm,
  toptitle=1mm,bottomtitle=1mm,fonttitle=\bfseries,
  arc=0mm,outer arc=0mm,
  colback=yellow!10!white,colframe=red,
  watermark color=yellow!75!red!25!white,
  enlarge left by=-8mm,
  enlarge right by=-8mm,
  enlarge top by=0mm,
  enlarge bottom by=0mm,
  width=\the\dimexpr\linewidth+1.6cm\relax,
  frame style={top color=tcbcol@frame,bottom color=tcbcol@frame,middle color=yellow!75!tcbcol@frame},
  title style={left color=tcbcol@frame,right color=tcbcol@frame,middle color=yellow!75!tcbcol@frame},
  watermark tikz={\draw[line width=2mm] circle (1cm) node{\fontfamily{ptm}\fontseries{b}\fontsize{20mm}{20mm}\selectfont!};},
  watermark zoom=0.75,
}}


\def\tcb@arc@bor{\pgfsetcornersarced{\pgfqpoint{\tcb@border@arc}{\tcb@border@arc}}}%

\def\tcb@arc@bor@NW{\csname tcb@arc@bor@NW@\tcb@corner@mode@NW\endcsname}
\def\tcb@arc@bor@NE{\csname tcb@arc@bor@NE@\tcb@corner@mode@NE\endcsname}
\def\tcb@arc@bor@SW{\csname tcb@arc@bor@SW@\tcb@corner@mode@SW\endcsname}
\def\tcb@arc@bor@SE{\csname tcb@arc@bor@SE@\tcb@corner@mode@SE\endcsname}

\let\tcb@arc@bor@NW@sharp\tcb@arc@zpt
\let\tcb@arc@bor@NE@sharp\tcb@arc@zpt
\let\tcb@arc@bor@SW@sharp\tcb@arc@zpt
\let\tcb@arc@bor@SE@sharp\tcb@arc@zpt

\let\tcb@arc@bor@NW@rounded\tcb@arc@bor
\let\tcb@arc@bor@NE@rounded\tcb@arc@bor
\let\tcb@arc@bor@SW@rounded\tcb@arc@bor
\let\tcb@arc@bor@SE@rounded\tcb@arc@bor

\def\tcb@border@prepare#1#2{%
  \tcbdimto\tcb@border@ts{#2+(#1)/2}%
  \ifdim\dimexpr\tcb@outer@arc>\tcb@arc@scale\dimexpr\tcb@border@ts\relax%
    \tcbdimto\tcb@border@arc{\tcb@outer@arc-\tcb@arc@scale\dimexpr\tcb@border@ts\relax}%
  \else%
    \let\tcb@border@arc=\tcb@zpt%
  \fi%
}

\def\tcb@border@unbroken#1#2#3{%
  \tcb@border@prepare{#1}{#2}%
  \tcb@pathbase{draw,line width=#1,#3}{[xshift=\tcb@border@ts,yshift=\tcb@border@ts]frame.south west}%
    {[xshift=-\tcb@border@ts,yshift=-\tcb@border@ts]frame.north east}%
    {\tcb@arc@bor@SW}{\tcb@arc@bor@NW}{\tcb@arc@bor@NE}{\tcb@arc@bor@SE}%
}

\def\tcb@border@first#1#2#3{%
  \tcb@border@prepare{#1}{#2}%
  \tcb@pathboundary{draw,line width=#1,#3}{%
    \tcb@gettikzxy{([xshift=\tcb@border@ts]frame.south west)}{\tcb@xa}{\tcb@ya}%
    \tcb@gettikzxy{([xshift=-\tcb@border@ts,yshift=-\tcb@border@ts]frame.north east)}{\tcb@xb}{\tcb@yb}%
    \pgfpathmoveto{\pgfqpoint{\tcb@xa}{\tcb@ya}}%
    \tcb@arc@bor@NW\pgfpathlineto{\pgfqpoint{\tcb@xa}{\tcb@yb}}%
    \tcb@arc@bor@NE\pgfpathlineto{\pgfqpoint{\tcb@xb}{\tcb@yb}}%
    \tcb@arc@zpt\pgfpathlineto{\pgfqpoint{\tcb@xb}{\tcb@ya}}%
  }%
}

\def\tcb@border@middle#1#2#3{%
  \tcb@border@prepare{#1}{#2}%
  \draw[line width=#1,#3]
    ([xshift=\tcb@border@ts]frame.north west) -- ([xshift=\tcb@border@ts]frame.south west);%
  \draw[line width=#1,#3]
    ([xshift=-\tcb@border@ts]frame.north east) -- ([xshift=-\tcb@border@ts]frame.south east);%
}

\def\tcb@border@last#1#2#3{%
  \tcb@border@prepare{#1}{#2}%
  \tcb@pathboundary{draw,line width=#1,#3}{%
    \tcb@gettikzxy{([xshift=\tcb@border@ts,yshift=\tcb@border@ts]frame.south west)}{\tcb@xa}{\tcb@ya}%
    \tcb@gettikzxy{([xshift=-\tcb@border@ts]frame.north east)}{\tcb@xb}{\tcb@yb}%
    \pgfpathmoveto{\pgfqpoint{\tcb@xa}{\tcb@yb}}%
    \tcb@arc@bor@SW\pgfpathlineto{\pgfqpoint{\tcb@xa}{\tcb@ya}}%
    \tcb@arc@bor@SE\pgfpathlineto{\pgfqpoint{\tcb@xb}{\tcb@ya}}%
    \tcb@arc@zpt\pgfpathlineto{\pgfqpoint{\tcb@xb}{\tcb@yb}}%
  }%
}

\def\tcb@draw@border@unbroken{%
  \let\tcb@border=\tcb@border@unbroken%
  \kvtcb@borderline%
}

\def\tcb@draw@border@first{%
  \let\tcb@border=\tcb@border@first%
  \kvtcb@borderline%
}

\def\tcb@draw@border@middle{%
  \let\tcb@border=\tcb@border@middle%
  \kvtcb@borderline%
}

\def\tcb@draw@border@last{%
  \let\tcb@border=\tcb@border@last%
  \kvtcb@borderline%
}

\def\tcb@bordernorth@draw#1#2#3{%
  \tcbdimto\tcb@border@ts{#2+(#1)/2}%
  \draw[line width=#1,#3] ([yshift=-\tcb@border@ts]frame.north west) -- ([yshift=-\tcb@border@ts]frame.north east);%
}

\def\tcb@bordernorth{%
  \ifdefstring{\tcb@split@state}{unbroken}{\tcb@bordernorth@draw}{%
    \ifdefstring{\tcb@split@state}{first}{\tcb@bordernorth@draw}{}}%
}

\def\tcb@bordersouth@draw#1#2#3{%
  \tcbdimto\tcb@border@ts{#2+(#1)/2}%
  \draw[line width=#1,#3] ([yshift=\tcb@border@ts]frame.south west) -- ([yshift=\tcb@border@ts]frame.south east);%
}

\def\tcb@bordersouth{%
  \ifdefstring{\tcb@split@state}{unbroken}{\tcb@bordersouth@draw}{%
    \ifdefstring{\tcb@split@state}{last}{\tcb@bordersouth@draw}{}}%
}

\def\tcb@borderwest#1#2#3{%
  \tcbdimto\tcb@border@ts{#2+(#1)/2}%
  \draw[line width=#1,#3] ([xshift=\tcb@border@ts]frame.north west) -- ([xshift=\tcb@border@ts]frame.south west);%
}

\def\tcb@bordereast#1#2#3{%
  \tcbdimto\tcb@border@ts{#2+(#1)/2}%
  \draw[line width=#1,#3] ([xshift=-\tcb@border@ts]frame.north east) -- ([xshift=-\tcb@border@ts]frame.south east);%
}

\tcbset{%
  border@line app/.code={\appto\kvtcb@borderline{#1}},%
  borderline/.style args={#1#2#3}{border@line app={\tcb@border{#1}{#2}{#3}}},%
  no borderline/.code={\def\kvtcb@borderline{}},%
  borderline north/.style args={#1#2#3}{border@line app={\tcb@bordernorth{#1}{#2}{#3}}},%
  borderline south/.style args={#1#2#3}{border@line app={\tcb@bordersouth{#1}{#2}{#3}}},%
  borderline west/.style args={#1#2#3}{border@line app={\tcb@borderwest{#1}{#2}{#3}}},%
  borderline east/.style args={#1#2#3}{border@line app={\tcb@bordereast{#1}{#2}{#3}}},%
  borderline horizontal/.style args={#1#2#3}{borderline north={#1}{#2}{#3},borderline south={#1}{#2}{#3}},%
  borderline vertical/.style args={#1#2#3}{borderline west={#1}{#2}{#3},borderline east={#1}{#2}{#3}},%
}


\def\tcb@shadow@comp@ts@smart#1#2{%
  \ifdim#2>0pt\relax\tcbdimto\tcb@shadow@ts{#1-#2/2}%%
  \else\tcbdimto\tcb@shadow@ts{#1+#2/2}\fi%
}

\def\tcb@shadow@comp@ts@copy#1#2{%
  \tcbdimto\tcb@shadow@ts{#1}%
}

\def\tcb@shadow@comp@arc{%
  \ifdim\dimexpr\tcb@outer@arc>\tcb@arc@scale\dimexpr\tcb@shadow@ts\relax%
    \tcbdimto\tcb@shadow@arc{\tcb@outer@arc-\tcb@arc@scale\dimexpr\tcb@shadow@ts\relax}%
  \else%
    \let\tcb@shadow@arc=\tcb@zpt%
  \fi%
}

\def\tcb@arc@sha{\pgfsetcornersarced{\pgfqpoint{\tcb@shadow@arc}{\tcb@shadow@arc}}}%

\def\tcb@arc@sha@NW{\csname tcb@arc@sha@NW@\tcb@corner@mode@NW\endcsname}
\def\tcb@arc@sha@NE{\csname tcb@arc@sha@NE@\tcb@corner@mode@NE\endcsname}
\def\tcb@arc@sha@SW{\csname tcb@arc@sha@SW@\tcb@corner@mode@SW\endcsname}
\def\tcb@arc@sha@SE{\csname tcb@arc@sha@SE@\tcb@corner@mode@SE\endcsname}

\let\tcb@arc@sha@NW@sharp\tcb@arc@zpt
\let\tcb@arc@sha@NE@sharp\tcb@arc@zpt
\let\tcb@arc@sha@SW@sharp\tcb@arc@zpt
\let\tcb@arc@sha@SE@sharp\tcb@arc@zpt

\let\tcb@arc@sha@NW@rounded\tcb@arc@sha
\let\tcb@arc@sha@NE@rounded\tcb@arc@sha
\let\tcb@arc@sha@SW@rounded\tcb@arc@sha
\let\tcb@arc@sha@SE@rounded\tcb@arc@sha

\def\tcb@shadow@unbroken#1#2#3#4{%
  \tcb@shadow@comp@ts{#3}{#1}%
  \tcb@shadow@comp@arc%
  \tcb@pathbase{fill,#4}{[xshift=#1+#3,yshift=#2+#3]frame.south west}{[xshift=#1-#3,yshift=#2-#3]frame.north east}%
    {\tcb@arc@sha@SW}{\tcb@arc@sha@NW}{\tcb@arc@sha@NE}{\tcb@arc@sha@SE}%
}

\def\tcb@shadow@first#1#2#3#4{%
  \tcb@shadow@comp@ts{#3}{#1}%
  \tcb@shadow@comp@arc%
  \tcb@pathbase{fill,#4}{[xshift=#1+#3,yshift=#2+#3]frame.south west}{[xshift=#1-#3,yshift=#2-#3]frame.north east}%
    {\tcb@arc@zpt}{\tcb@arc@sha@NW}{\tcb@arc@sha@NE}{\tcb@arc@zpt}%
}

\def\tcb@shadow@middle#1#2#3#4{%
  \tcb@shadow@comp@ts{#3}{#1}%
  \tcb@shadow@comp@arc%
  \tcb@pathbase{fill,#4}{[xshift=#1+#3,yshift=#2+#3]frame.south west}{[xshift=#1-#3,yshift=#2-#3]frame.north east}%
    {\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}%
}

\def\tcb@shadow@last#1#2#3#4{%
  \tcb@shadow@comp@ts{#3}{#1}%
  \tcb@shadow@comp@arc%
  \tcb@pathbase{fill,#4}{[xshift=#1+#3,yshift=#2+#3]frame.south west}{[xshift=#1-#3,yshift=#2-#3]frame.north east}%
    {\tcb@arc@sha@SW}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@sha@SE}%
}


\tcbset{%
  shad@w app/.code={\appto\kvtcb@shadow{#1}},%
  shadow/.style args={#1#2#3#4}{shad@w app={\csuse{tcb@shadow@\tcb@shapeofskin}{#1}{#2}{#3}{#4}}},%
  no shadow/.code={\def\kvtcb@shadow{}},%
  fuzzy shadow/.style args={#1#2#3#4#5}{shad@w app={%
    \begin{scope}[#5]%
      \letcs\tcb@shadow{tcb@shadow@\tcb@shapeofskin}%
      \tcb@shadow{#1}{#2}{\the\dimexpr#3-4\dimexpr#4\relax}{opacity=0.01}%
      \tcb@shadow{#1}{#2}{\the\dimexpr#3-3\dimexpr#4\relax}{opacity=0.02}%
      \tcb@shadow{#1}{#2}{\the\dimexpr#3-2\dimexpr#4\relax}{opacity=0.04}%
      \tcb@shadow{#1}{#2}{\the\dimexpr#3-#4\relax}{opacity=0.07}%
      \tcb@shadow{#1}{#2}{#3}{opacity=0.11}%
      \tcb@shadow{#1}{#2}{\the\dimexpr#3+#4\relax}{opacity=0.11}%
      \tcb@shadow{#1}{#2}{\the\dimexpr#3+2\dimexpr#4\relax}{opacity=0.07}%
      \tcb@shadow{#1}{#2}{\the\dimexpr#3+3\dimexpr#4\relax}{opacity=0.04}%
      \tcb@shadow{#1}{#2}{\the\dimexpr#3+4\dimexpr#4\relax}{opacity=0.02}%
      \tcb@shadow{#1}{#2}{\the\dimexpr#3+5\dimexpr#4\relax}{opacity=0.01}%
  \end{scope}}},%
  %
  drop shadow/.style={shadow={0.9mm}{-0.9mm}{0mm}{opacity=0.5,#1}},
  drop shadow/.default={black!50!white},%
  drop midday shadow/.style={shadow={0mm}{-0.8mm}{-0.4mm}{opacity=0.5,#1}},
  drop midday shadow/.default={black!50!white},%
  halo/.style args={#1 with #2}{shadow={0mm}{0mm}{-#1}{opacity=0.5,#2}},
  halo/.default={0.9mm with yellow},%
  drop fuzzy shadow/.style={fuzzy shadow={1.0mm}{-1.0mm}{0mm}{0.12mm}{#1}},
  drop fuzzy shadow/.default={black!50!white},%
  drop fuzzy midday shadow/.style={fuzzy shadow={0mm}{-1.0mm}{-0.5mm}{0.12mm}{#1}},
  drop fuzzy midday shadow/.default={black!50!white},%
  fuzzy halo/.style args={#1 with #2}{fuzzy shadow={0mm}{0mm}{-#1}{0.12mm}{#2}},
  fuzzy halo/.default={1.0mm with yellow},%
  %
  drop shadow southeast/.style={shadow={0.9mm}{-0.9mm}{0mm}{opacity=0.5,#1}},%
  drop shadow southeast/.default={black!50!white},%
  drop shadow south/.style={shadow={0mm}{-0.8mm}{-0.4mm}{opacity=0.5,#1}},%
  drop shadow south/.default={black!50!white},%
  drop shadow southwest/.style={shadow={-0.9mm}{-0.9mm}{0mm}{opacity=0.5,#1}},%
  drop shadow southwest/.default={black!50!white},%
  drop shadow west/.style={shadow={-0.8mm}{0mm}{-0.4mm}{opacity=0.5,#1}},%
  drop shadow west/.default={black!50!white},%
  drop shadow northwest/.style={shadow={-0.9mm}{0.9mm}{0mm}{opacity=0.5,#1}},%
  drop shadow northwest/.default={black!50!white},%
  drop shadow north/.style={shadow={0mm}{0.8mm}{-0.4mm}{opacity=0.5,#1}},%
  drop shadow north/.default={black!50!white},%
  drop shadow northeast/.style={shadow={0.9mm}{0.9mm}{0mm}{opacity=0.5,#1}},%
  drop shadow northeast/.default={black!50!white},%
  drop shadow east/.style={shadow={0.8mm}{0mm}{-0.4mm}{opacity=0.5,#1}},%
  drop shadow east/.default={black!50!white},%
  drop fuzzy shadow southeast/.style={fuzzy shadow={1.0mm}{-1.0mm}{0mm}{0.12mm}{#1}},
  drop fuzzy shadow southeast/.default={black!50!white},%
  drop fuzzy shadow south/.style={fuzzy shadow={0mm}{-1.0mm}{-0.5mm}{0.12mm}{#1}},
  drop fuzzy shadow south/.default={black!50!white},%
  drop fuzzy shadow southwest/.style={fuzzy shadow={-1.0mm}{-1.0mm}{0mm}{0.12mm}{#1}},
  drop fuzzy shadow southwest/.default={black!50!white},%
  drop fuzzy shadow west/.style={fuzzy shadow={-1.0mm}{0mm}{-0.5mm}{0.12mm}{#1}},
  drop fuzzy shadow west/.default={black!50!white},%
  drop fuzzy shadow northwest/.style={fuzzy shadow={-1.0mm}{1.0mm}{0mm}{0.12mm}{#1}},
  drop fuzzy shadow northwest/.default={black!50!white},%
  drop fuzzy shadow north/.style={fuzzy shadow={0mm}{1.0mm}{-0.5mm}{0.12mm}{#1}},
  drop fuzzy shadow north/.default={black!50!white},%
  drop fuzzy shadow northeast/.style={fuzzy shadow={1.0mm}{1.0mm}{0mm}{0.12mm}{#1}},
  drop fuzzy shadow northeast/.default={black!50!white},%
  drop fuzzy shadow east/.style={fuzzy shadow={1.0mm}{0mm}{-0.5mm}{0.12mm}{#1}},
  drop fuzzy shadow east/.default={black!50!white},%
  %
  smart shadow arc/.is choice,
  smart shadow arc/true/.code={\let\tcb@shadow@comp@ts=\tcb@shadow@comp@ts@smart},
  smart shadow arc/false/.code={\let\tcb@shadow@comp@ts=\tcb@shadow@comp@ts@copy},
  smart shadow arc/.default=true,
}

\def\tcb@boundary@tikzbendedbase#1#2#3#4#5#6#7#8{%
  \tcb@gettikzxy{(#1)}{\tcb@xa}{\tcb@ya}%
  \tcb@gettikzxy{(#2)}{\tcb@xb}{\tcb@yb}%
  \pgfpathmoveto{\pgfqpoint{\tcb@xa}{\tcb@yb}}%
  #5\pgfpathquadraticcurveto{\pgfqpoint{\dimexpr0.5\dimexpr\tcb@xa+\tcb@xb\relax}{\dimexpr\tcb@yb+#8}}{\pgfqpoint{\tcb@xb}{\tcb@yb}}%
  #6\pgfpathlineto{\pgfqpoint{\tcb@xb}{\tcb@ya}}%
  #3\pgfpathquadraticcurveto{\pgfqpoint{\dimexpr0.5\dimexpr\tcb@xa+\tcb@xb\relax}{\dimexpr\tcb@ya+#7}}{\pgfqpoint{\tcb@xa}{\tcb@ya}}%
  #4\pgfpathclose%
}

\def\tcb@pathbendedbase#1#2#3#4#5#6#7#8#9{\tcb@pathboundary{#1}{\tcb@boundary@tikzbendedbase{#2}{#3}{#4}{#5}{#6}{#7}{#8}{#9}}}

\def\tcb@shadowbended@prepare#1{%
  \tcbdimto\tcb@shadow@arc{\tcb@outer@arc-\tcb@arc@scale\dimexpr#1\relax}%
  \ifdim\dimexpr\tcb@shadow@arc<0pt\relax%
    \let\tcb@shadow@arc=\tcb@zpt%
  \fi%
}

\def\tcb@shadowlifted@unbroken#1#2#3#4#5{%
  \tcb@shadowbended@prepare{#3}%
  \tcb@pathbendedbase{fill,#5}{[xshift=#1+#3,yshift=#2+#3]frame.south west}{[xshift=-#1-#3,yshift=#2-#3]frame.north east}%
    {\tcb@arc@sha@SW}{\tcb@arc@sha@NW}{\tcb@arc@sha@NE}{\tcb@arc@sha@SE}{#4}{0pt}%
}

\def\tcb@shadowlifted@first#1#2#3#4#5{%
  \tcb@shadowbended@prepare{#3}%
  \tcb@pathbendedbase{fill,#5}{[xshift=#1+#3,yshift=#2+#3]frame.south west}{[xshift=-#1-#3,yshift=#2-#3]frame.north east}%
    {\tcb@arc@zpt}{\tcb@arc@sha@NW}{\tcb@arc@sha@NE}{\tcb@arc@zpt}{#4}{0pt}%
}

\def\tcb@shadowlifted@middle#1#2#3#4#5{%
  \tcb@shadowbended@prepare{#3}%
  \tcb@pathbendedbase{fill,#5}{[xshift=#1+#3,yshift=#2+#3]frame.south west}{[xshift=-#1-#3,yshift=#2-#3]frame.north east}%
    {\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@zpt}{#4}{0pt}%
}

\def\tcb@shadowlifted@last#1#2#3#4#5{%
  \tcb@shadowbended@prepare{#3}%
  \tcb@pathbendedbase{fill,#5}{[xshift=#1+#3,yshift=#2+#3]frame.south west}{[xshift=-#1-#3,yshift=#2-#3]frame.north east}%
    {\tcb@arc@sha@SW}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@sha@SE}{#4}{0pt}%
}

\tcbset{
  lifted shadow/.style n args={5}{shad@w app={%
    \begin{scope}[#5]%
      \letcs\tcb@shadowlifted{tcb@shadowlifted@\tcb@shapeofskin}%
      \tcb@shadowlifted{#1}{#2}{\dimexpr-4\dimexpr#4}{#3}{opacity=0.01}%
      \tcb@shadowlifted{#1}{#2}{\dimexpr-3\dimexpr#4}{#3}{opacity=0.02}%
      \tcb@shadowlifted{#1}{#2}{\dimexpr-2\dimexpr#4}{#3}{opacity=0.04}%
      \tcb@shadowlifted{#1}{#2}{\dimexpr-#4}{#3}{opacity=0.07}%
      \tcb@shadowlifted{#1}{#2}{0pt}{#3}{opacity=0.11}%
      \tcb@shadowlifted{#1}{#2}{\dimexpr+#4}{#3}{opacity=0.11}%
      \tcb@shadowlifted{#1}{#2}{\dimexpr+2\dimexpr#4}{#3}{opacity=0.07}%
      \tcb@shadowlifted{#1}{#2}{\dimexpr+3\dimexpr#4}{#3}{opacity=0.04}%
      \tcb@shadowlifted{#1}{#2}{\dimexpr+4\dimexpr#4}{#3}{opacity=0.02}%
      \tcb@shadowlifted{#1}{#2}{\dimexpr+5\dimexpr#4}{#3}{opacity=0.01}%
  \end{scope}}},%
  drop small lifted shadow/.style={lifted shadow={1mm}{-0.75mm}{1.3mm}{0.1mm}{#1}},
  drop small lifted shadow/.default={black!50!white},%
  drop lifted shadow/.style={lifted shadow={1.5mm}{-1.5mm}{2.7mm}{0.12mm}{#1}},
  drop lifted shadow/.default={black!50!white},%
  drop large lifted shadow/.style={lifted shadow={2mm}{-3mm}{5.7mm}{0.16mm}{#1}},
  drop large lifted shadow/.default={black!50!white},%
}

\newif\iftcb@isindraft
\def\tcb@draftmode{\tcbset{spartan,spartan@fit}}
\def\tcbstartdraftmode{\let\tcb@afteroptions@hook=\tcb@draftmode\tcb@isindrafttrue}
\def\tcbstopdraftmode{\let\tcb@afteroptions@hook=\@empty\tcb@isindraftfalse}

\def\tcbinterruptdraftmode{%
  \iftcb@isindraft%
    \tcbstopdraftmode%
    \let\tcbcontinuedraftmode=\tcbstartdraftmode%
  \else%
    \let\tcbcontinuedraftmode=\@empty%
  \fi}

\tcbset{%
  draftmode/.is choice,%
  draftmode/.default=true,%
  draftmode/true/.code=\tcbstartdraftmode,%
  draftmode/false/.code=\tcbstopdraftmode,%
}


\def\tcb@include@graphics{%
  \ifdefstring{\kvtcb@capture}{hbox}{%
    \tcbox{%
      \edef\tcb@temp{\noexpand\includegraphics[\expandonce\kvtcb@graphics@options]}%
      \tcb@temp{\imagepath}%
    }%
  }{%
    \iftcb@fixedheight%
      \begin{tcolorbox}[underlay={%
        \begin{tcbclipinterior}%
        \edef\tcb@temp{\noexpand\tikzset{fill image options={\expandonce\kvtcb@graphics@options}}}%
        \tcb@temp%
        \path[fill zoom image={\imagepath}]
          ([xshift=\kvtcb@boxsep+\kvtcb@leftupper,yshift=\kvtcb@boxsep+\kvtcb@bottom]interior.south west) rectangle
          ([xshift=-\kvtcb@boxsep-\kvtcb@rightupper,yshift=-\kvtcb@boxsep-\kvtcb@top]interior.north east);
        \end{tcbclipinterior}%
        }]%
      \end{tcolorbox}%
    \else%
      \begin{tcolorbox}%
        \edef\tcb@temp{\noexpand\includegraphics[\expandonce\kvtcb@graphics@options,width=\linewidth]}%
        \tcb@temp{\imagepath}%
      \end{tcolorbox}%
    \fi%
  }%
}

\def\tcb@scanfilename#1#2{%
  \begingroup%
    \everyeof{\noexpand}%
    \endlinechar -1%
    \catcode`\_=11%
    \catcode`\~=11%
    \edef\x{\scantokens\expandafter{#2}}%
  \expandafter\endgroup%
  \expandafter\def\expandafter #1\expandafter{\x}%
}%


\def\tcb@include@graphics@preparefile#1{%
  \tcb@scanfilename\tcb@temp{#1}%
  \filename@parse{\tcb@temp}%
  \ifx\filename@ext\relax%
    \let\imagename\filename@base%
  \else%
    \def\imagename{\filename@base\Gin@sepdefault\filename@ext}%
  \fi%
  \ifdefined\grffile@Ginclude@graphics%
    % grffile package loaded
    \ifx\kvtcb@graphics@directory\@empty%
      \def\imagepath{#1}%
    \else%
      \def\imagepath{\kvtcb@graphics@directory/#1}%
    \fi%
  \else%
    \ifx\kvtcb@graphics@directory\@empty%
      \edef\imagepath{#1}%
    \else%
      \edef\imagepath{\kvtcb@graphics@directory/#1}%
    \fi%
  \fi%
}

\newcommand{\tcbincludegraphics}[2][]{%
  \begingroup%
  \tcb@layer@pushup%
  \tcb@apply@box@options{enhanced,clip upper=true,valign=center,center upper,#1}%
  \tcb@include@graphics@preparefile{#2}%
  \edef\imagepage{1}%
  \tcb@include@graphics%
  \endgroup%
}

\def\tcb@set@pdfpages#1#2{%
  \IfFileExists{#2}{%
    \ifdef{\pdfximage}{%
      \pdfximage{#2}%
      \edef#1{\the\pdflastximagepages}%
    }{%
      \ifdef{\XeTeXpdfpagecount}{%
        \edef#1{\the\XeTeXpdfpagecount #2 }%
        \ifnum#1=0 %
          \edef#1{1}%
        \fi%
      }{\tcb@error{For PDF support run pdflatex, xelatex, or lualatex}{%
        Your compiler seems not to support PDF include files.}}%
    }%
  }{\tcb@error{PDF file `#2' not found}{The PDF file `#2' was not found}}%
  \relax%
}

\newcommand{\tcbincludepdf}[2][]{%
  \begingroup%
  \tcb@layer@pushup%
  \tcb@apply@box@options{enhanced,clip upper=true,valign=center,center upper,#1}%
  \appto\kvtcb@graphics@options{,page=\imagepage}%
  \tcb@include@graphics@preparefile{#2}%
  \tcb@set@pdfpages\pdfpages{\imagepath}%
  \foreach \imagepage in \kvtcb@graphics@pages%
  {%
    \tcb@include@graphics%
  }%
  \endgroup%
}

\tcbset{%
  graphics options/.store in=\kvtcb@graphics@options,
  graphics pages/.store in=\kvtcb@graphics@pages,
  graphics directory/.store in=\kvtcb@graphics@directory,
}


\tcbset{%
  reset@skins/.style={%
    frame style=,interior style=,segmentation style=,@title style=,%
    colbacklower=black!15!white,%
    extend freelance=,extend freelancefirst=,extend freelancemiddle=,extend freelancelast=,%
    clear@spec,%
    watermark opacity=1.00,watermark color=tcbcol@back!85!tcbcol@frame,%
    watermark zoom=0.75,clip watermark,%
    clip title=false,clip upper=false,clip lower=false,%
    no borderline,smart shadow arc,no shadow,no underlay,no finish,tikz reset,at begin tikz reset,at end tikz reset,%
    boxed title style=,hbox boxed title,code={\let\tcb@specialgeonodes@hook\relax},%
    graphics options=,graphics pages={1,...,\pdfpages},graphics directory=,%
  },
  initialize@reset=reset@skins,
}

\tcbuselibrary{skins@jigsaw}


==> tcbskinsjigsaw.code.tex <==
%% The LaTeX package tcolorbox - version 3.80 (2015/11/27)
%% tcbskinsjigsaw.code.tex: Code for colorboxes with different skins
%%
%% -------------------------------------------------------------------------------------------
%% Copyright (c) 2006-2015 by Prof. Dr. Dr. Thomas F. Sturm <thomas dot sturm at unibw dot de>
%% -------------------------------------------------------------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2005/12/01 or later.
%%
%% This work has the LPPL maintenance status `author-maintained'.
%%
%% This work consists of all files listed in README
%%
\tcb@set@library@version{3.80}

\tcbuselibrary{skins}

\def\tcb@drawframe@pathjigsaw{%
  \tcb@pathboundary{tcb fill frame}{\tcb@boundaryframe@standardjigsaw}%
}

\def\tcb@boundary@pathfirstjigsaw@A{%
  \tcbdimto\tcb@xa{\tcb@width-\kvtcb@right@rule}%
  \tcbdimto\tcb@ya{\tcb@height-\kvtcb@top@rule}%
  \pgfpathmoveto{\pgfpointorigin}%
  \tcb@arc@out@NW\pgfpathlineto{\pgfqpoint{0pt}{\tcb@height}}%
  \tcb@arc@out@NE\pgfpathlineto{\pgfqpoint{\tcb@width}{\tcb@height}}%
  \tcb@arc@zpt\pgfpathlineto{\pgfqpoint{\tcb@width}{0pt}}%
  \pgfpathlineto{\pgfqpoint{\tcb@xa}{0pt}}%
  \tcb@arc@ins@NE\pgfpathlineto{\pgfqpoint{\tcb@xa}{\tcb@ya}}%
  \tcb@arc@ins@NW\pgfpathlineto{\pgfqpoint{\kvtcb@left@rule}{\tcb@ya}}%
  \tcb@arc@zpt\pgfpathlineto{\pgfqpoint{\kvtcb@left@rule}{0pt}}%
  \pgfpathclose%
}

\def\tcb@boundary@pathfirstjigsaw@B{%
  \tcbdimto\tcb@xa{\tcb@width-\kvtcb@right@rule}%
  \tcbdimto\tcb@ya{\kvtcb@bottom@rule+\tcb@innerheight}%
  \pgfpathmoveto{\pgfpointorigin}%
  \tcb@arc@out@NW\pgfpathlineto{\pgfqpoint{0pt}{\tcb@height}}%
  \tcb@arc@out@NE\pgfpathlineto{\pgfqpoint{\tcb@width}{\tcb@height}}%
  \tcb@arc@zpt\pgfpathlineto{\pgfqpoint{\tcb@width}{0pt}}%
  \pgfpathlineto{\pgfqpoint{\tcb@xa}{0pt}}%
  \pgfpathlineto{\pgfqpoint{\tcb@xa}{\tcb@ya}}%
  \pgfpathlineto{\pgfqpoint{\kvtcb@left@rule}{\tcb@ya}}%
  \pgfpathlineto{\pgfqpoint{\kvtcb@left@rule}{0pt}}%
  \pgfpathclose%
}

\def\tcb@drawframe@pathfirstjigsaw{%
  \tcb@pathboundary{tcb fill frame}{%
    \pgfseteorule%
    \iftcb@hasTitle%
      \iftcb@titlefilled%
        \ifdim\dimexpr\kvtcb@title@rule>0pt\relax%
          \tcb@boundary@pathfirstjigsaw@B%
          \tcb@boundarytitle@standard%
        \else%
          \tcb@boundary@pathfirstjigsaw@A%
        \fi%
      \else%
        \tcb@boundary@pathfirstjigsaw@B%
      \fi%
    \else%
      \tcb@boundary@pathfirstjigsaw@A%
    \fi%
  }%
}

\def\tcb@boundary@pathmiddlejigsaw@A{%
  \tcbdimto\tcb@xa{\tcb@width-\kvtcb@right@rule}%
  \pgfpathrectangle{\pgfpointorigin}{\pgfqpoint{\kvtcb@left@rule}{\tcb@height}}%
  \pgfpathrectangle{\pgfqpoint{\tcb@xa}{0pt}}{\pgfqpoint{\kvtcb@right@rule}{\tcb@height}}%
}

\def\tcb@boundary@pathmiddlejigsaw@B{%
  \tcbdimto\tcb@xa{\tcb@width-\kvtcb@right@rule}%
  \tcbdimto\tcb@ya{\tcb@height-\kvtcb@top@rule}%
  \pgfpathmoveto{\pgfpointorigin}%
  \tcb@arc@zpt\pgfpathlineto{\pgfqpoint{0pt}{\tcb@height}}%
  \pgfpathlineto{\pgfqpoint{\tcb@width}{\tcb@height}}%
  \pgfpathlineto{\pgfqpoint{\tcb@width}{0pt}}%
  \pgfpathlineto{\pgfqpoint{\tcb@xa}{0pt}}%
  \pgfpathlineto{\pgfqpoint{\tcb@xa}{\tcb@ya}}%
  \pgfpathlineto{\pgfqpoint{\kvtcb@left@rule}{\tcb@ya}}%
  \pgfpathlineto{\pgfqpoint{\kvtcb@left@rule}{0pt}}%
  \pgfpathclose%
}

\def\tcb@boundary@pathmiddlejigsaw@C{%
  \tcbdimto\tcb@xa{\tcb@width-\kvtcb@right@rule}%
  \tcbdimto\tcb@ya{\kvtcb@bottom@rule+\tcb@innerheight}%
  \pgfpathmoveto{\pgfpointorigin}%
  \tcb@arc@zpt\pgfpathlineto{\pgfqpoint{0pt}{\tcb@height}}%
  \pgfpathlineto{\pgfqpoint{\tcb@width}{\tcb@height}}%
  \pgfpathlineto{\pgfqpoint{\tcb@width}{0pt}}%
  \pgfpathlineto{\pgfqpoint{\tcb@xa}{0pt}}%
  \pgfpathlineto{\pgfqpoint{\tcb@xa}{\tcb@ya}}%
  \pgfpathlineto{\pgfqpoint{\kvtcb@left@rule}{\tcb@ya}}%
  \pgfpathlineto{\pgfqpoint{\kvtcb@left@rule}{0pt}}%
  \pgfpathclose%
}

\def\tcb@drawframe@pathmiddlejigsaw{%
  \tcb@pathboundary{tcb fill frame}{%
    \pgfseteorule%
    \iftcb@hasTitle%
      \iftcb@titlefilled%
        \ifdim\dimexpr\kvtcb@title@rule>0pt\relax%
          \tcb@boundary@pathmiddlejigsaw@C%
          \tcb@arc@zpt%
          \tcbdimto\tcb@ya{\kvtcb@bottom@rule+\tcb@innerheight+\kvtcb@title@rule}%
          \tcbdimto\tcb@xb{\tcb@width-\kvtcb@right@rule}%
          \tcbdimto\tcb@yb{\tcb@height-\kvtcb@top@rule}%
          \pgfpathrectanglecorners{\pgfqpoint{\kvtcb@left@rule}{\tcb@ya}}{\pgfqpoint{\tcb@xb}{\tcb@yb}}%
        \else%
          \tcb@boundary@pathmiddlejigsaw@B%
        \fi%
      \else%
        \tcb@boundary@pathmiddlejigsaw@C%
      \fi%
    \else%
      \tcb@boundary@pathmiddlejigsaw@A%
    \fi%
  }%
}

\def\tcb@drawframe@pathlastjigsaw{%
  \tcb@pathboundary{tcb fill frame}{%
    \pgfseteorule%
    \iftcb@hasTitle%
      \iftcb@titlefilled%
        \ifdim\dimexpr\kvtcb@title@rule>0pt\relax%
          \tcb@boundaryframe@pathlast%
          \tcb@arc@zpt%
          \tcbdimto\tcb@ya{\kvtcb@bottom@rule+\tcb@innerheight+\kvtcb@title@rule}%
          \tcbdimto\tcb@xb{\tcb@width-\kvtcb@right@rule}%
          \tcbdimto\tcb@yb{\tcb@height-\kvtcb@top@rule}%
          \pgfpathrectanglecorners{\pgfqpoint{\kvtcb@left@rule}{\tcb@ya}}{\pgfqpoint{\tcb@xb}{\tcb@yb}}%
          \tcb@boundaryinterior@title@standard%
        \else%
          \tcb@boundaryframe@pathlast%
          \tcb@boundary@base{\kvtcb@left@rule}{\kvtcb@bottom@rule}%
            {\tcb@width-\kvtcb@right@rule}{\tcb@height-\kvtcb@top@rule}%
            {\tcb@arc@ins@SW}{\tcb@arc@zpt}{\tcb@arc@zpt}{\tcb@arc@ins@SE}%
        \fi%
      \else%
        \tcb@boundaryframe@pathlast%
      \fi%
    \else%
      \tcbdimto\tcb@xa{\tcb@width-\kvtcb@right@rule}%
      \pgfpathmoveto{\pgfpointorigin}%
      \tcb@arc@zpt\pgfpathlineto{\pgfqpoint{0pt}{\tcb@height}}%
      \pgfpathlineto{\pgfqpoint{\kvtcb@left@rule}{\tcb@height}}%
      \tcb@arc@ins@SW\pgfpathlineto{\pgfqpoint{\kvtcb@left@rule}{\kvtcb@bottom@rule}}%
      \tcb@arc@ins@SE\pgfpathlineto{\pgfqpoint{\tcb@xa}{\kvtcb@bottom@rule}}%
      \tcb@arc@zpt\pgfpathlineto{\pgfqpoint{\tcb@xa}{\tcb@height}}%
      \pgfpathlineto{\pgfqpoint{\tcb@width}{\tcb@height}}%
      \tcb@arc@out@SE\pgfpathlineto{\pgfqpoint{\tcb@width}{0pt}}%
      \tcb@arc@out@SW\pgfpathclose%
    \fi%
  }%
}


\def\tcb@draw@shadowjigsaw@unbroken{%
  \let\tcb@shadow=\tcb@shadow@unbroken%
  \begin{tcbinvclipframe}%
  \kvtcb@shadow%
  \end{tcbinvclipframe}%
}

\def\tcb@draw@shadowjigsaw@first{%
  \let\tcb@shadow=\tcb@shadow@first%
  \begin{tcbinvclipframe}%
  \kvtcb@shadow%
  \end{tcbinvclipframe}%
}

\def\tcb@draw@shadowjigsaw@middle{%
  \let\tcb@shadow=\tcb@shadow@middle%
  \begin{tcbinvclipframe}%
  \kvtcb@shadow%
  \end{tcbinvclipframe}%
}

\def\tcb@draw@shadowjigsaw@last{%
  \let\tcb@shadow=\tcb@shadow@last%
  \begin{tcbinvclipframe}%
  \kvtcb@shadow%
  \end{tcbinvclipframe}%
}

\tcb@new@skin{enhanced jigsaw}{base@unbroken,%
  frame engine=pathjigsaw,interior titled engine=path,interior engine=path,segmentation engine=path,title engine=path,%
  set@extensions@preframe={\tcb@draw@shadowjigsaw@unbroken},%
  skin first=enhancedfirst jigsaw,skin middle=enhancedmiddle jigsaw,skin last=enhancedlast jigsaw}

\tcb@new@skin{enhancedfirst jigsaw}{base@first,%
  frame engine=pathfirstjigsaw,interior titled engine=pathfirst,interior engine=pathfirst,segmentation engine=path,title engine=pathfirst,%
  set@extensions@preframe={\tcb@draw@shadowjigsaw@first},%
  skin first=enhancedfirst jigsaw,skin middle=enhancedmiddle jigsaw,skin last=enhancedmiddle jigsaw}

\tcb@new@skin{enhancedmiddle jigsaw}{base@middle,%
  frame engine=pathmiddlejigsaw,interior titled engine=pathmiddle,interior engine=pathmiddle,segmentation engine=path,title engine=pathmiddle,%
  set@extensions@preframe={\tcb@draw@shadowjigsaw@middle},%
  skin first=enhancedmiddle jigsaw,skin middle=enhancedmiddle jigsaw,skin last=enhancedmiddle jigsaw}

\tcb@new@skin{enhancedlast jigsaw}{base@last,%
  frame engine=pathlastjigsaw,interior titled engine=pathlast,interior engine=pathlast,segmentation engine=path,title engine=pathlast,%
  set@extensions@preframe={\tcb@draw@shadowjigsaw@last},%
  skin first=enhancedmiddle jigsaw,skin middle=enhancedmiddle jigsaw,skin last=enhancedlast jigsaw}

\tcbset{%
  enhanced jigsaw/.style={skin=enhanced jigsaw},%
  frame engine/pathjigsaw/.style={frame code=\tcb@drawframe@pathjigsaw},
  frame engine/pathfirstjigsaw/.style={frame code=\tcb@drawframe@pathfirstjigsaw},
  frame engine/pathmiddlejigsaw/.style={frame code=\tcb@drawframe@pathmiddlejigsaw},
  frame engine/pathlastjigsaw/.style={frame code=\tcb@drawframe@pathlastjigsaw},
}



==> tcbtheorems.code.tex <==
%% The LaTeX package tcolorbox - version 3.80 (2015/11/27)
%% tcbtheorems.code.tex: Code for theorems in colorboxes
%%
%% -------------------------------------------------------------------------------------------
%% Copyright (c) 2006-2015 by Prof. Dr. Dr. Thomas F. Sturm <thomas dot sturm at unibw dot de>
%% -------------------------------------------------------------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2005/12/01 or later.
%%
%% This work has the LPPL maintenance status `author-maintained'.
%%
%% This work consists of all files listed in README
%%
%\makeatletter
\tcb@set@library@version{3.80}

\RequirePackage{amsmath}

\def\tcb@hack@amsmath{\tcb@hack@currenvir\vskip-\abovedisplayskip}

\def\tcb@theo@form@namenumber#1#2{\hbox{#1~#2}}
\def\tcb@theo@form@numbername#1#2{\hbox{#2~#1}}
\def\tcb@theo@form@name#1#2{\hbox{#1}}

\def\tcb@theo@desc@form@std#1{\tcb@desc@col\kvtcb@desc@font\kvtcb@desc@delim@left#1\kvtcb@desc@delim@right}

\def\tcb@theo@title#1#2#3{%
  \ifdefempty{#2}{\setbox\z@=\color@hbox#1\color@endbox}{\setbox\z@=\tcb@theo@form{#1}{#2}}%
  \def\temp@a{#3}%
  \ifx\temp@a\@empty\relax%
    \unhbox\z@\kvtcb@terminatorsign%
  \else%
    \setbox\z@=\hbox{\unhbox\z@\kvtcb@separatorsign\ }%
    \hangindent\wd\z@%
    \hangafter=1%
    \mbox{\unhbox\z@}{\tcb@theo@desc@form{#3}}\kvtcb@terminatorsign%
  \fi%
}

\def\tcb@theo@listentry#1#2#3{%
  \def\kvtcb@listentry{\protect\numberline{#2}#3}%
}

\def\tcb@theo@label#1#2{%
  \def\temp@a{#2}%
  \ifx\temp@a\@empty%
  \else%
    \tcbset{label={#1:#2}}%
  \fi%
}

\if@fleqn%
\tcbset{%
  ams equation upper/.style={before upper=\tcb@hack@amsmath\equation,after upper=\endequation},%
  ams equation lower/.style={before lower=\tcb@hack@amsmath\equation,after lower=\endequation},%
  ams equation* upper/.style={before upper=\tcb@hack@amsmath\csname equation*\endcsname,after upper=\endequation},%
  ams equation* lower/.style={before lower=\tcb@hack@amsmath\csname equation*\endcsname,after lower=\endequation}%
}%
\else%
\tcbset{%
  ams equation upper/.style={before upper=\tcb@hack@currenvir\equation,after upper=\endequation},%
  ams equation lower/.style={before lower=\tcb@hack@currenvir\equation,after lower=\endequation},%
  ams equation* upper/.style={before upper=\tcb@hack@currenvir\csname equation*\endcsname,after upper=\endequation},%
  ams equation* lower/.style={before lower=\tcb@hack@currenvir\csname equation*\endcsname,after lower=\endequation},%
}%
\fi

\tcbset{
  theorem/.style args={#1#2#3#4}{%
    step and label={#2}{#4},%
    title={\letcs\tcb@temp{the#2}\tcb@theo@title{#1}{\tcb@temp}{#3}}},%
  math upper/.style={before upper=$\displaystyle,after upper=$},%
  math lower/.style={before lower=$\displaystyle,after lower=$},%
  math/.style={math upper,math lower},%
  ams equation/.style={ams equation upper,ams equation lower},%
  ams equation*/.style={ams equation* upper,ams equation* lower},%
  ams align upper/.style={before upper=\tcb@hack@amsmath\align,after upper=\endalign},%
  ams align lower/.style={before lower=\tcb@hack@amsmath\align,after lower=\endalign},%
  ams align/.style={ams align upper,ams align lower},%
  ams align* upper/.style={before upper=\tcb@hack@amsmath\csname align*\endcsname,after upper=\endalign},%
  ams align* lower/.style={before lower=\tcb@hack@amsmath\csname align*\endcsname,after lower=\endalign},%
  ams align*/.style={ams align* upper,ams align* lower},%
  ams gather upper/.style={before upper=\tcb@hack@amsmath\gather,after upper=\endgather},%
  ams gather lower/.style={before lower=\tcb@hack@amsmath\gather,after lower=\endgather},%
  ams gather/.style={ams gather upper,ams gather lower},%
  ams gather* upper/.style={before upper=\tcb@hack@amsmath\csname gather*\endcsname,after upper=\endgather},%
  ams gather* lower/.style={before lower=\tcb@hack@amsmath\csname gather*\endcsname,after lower=\endgather},%
  ams gather*/.style={ams gather* upper,ams gather* lower},%
  ams nodisplayskip upper/.style={before upper=\vskip-\abovedisplayskip},%
  ams nodisplayskip lower/.style={before lower=\vskip-\abovedisplayskip},%
  ams nodisplayskip/.style={ams nodisplayskip upper,ams nodisplayskip lower},%
  highlight math style/.style={highlight math/.style={notitle,nophantom,#1}},%
  separator sign/.store in=\kvtcb@separatorsign,%
  separator sign colon/.style={separator sign={:}},%
  separator sign dash/.style={separator sign={\ --}},%
  separator sign none/.style={separator sign=},%
  terminator sign/.store in=\kvtcb@terminatorsign,%
  terminator sign colon/.style={terminator sign={:}},%
  terminator sign dash/.style={terminator sign={\ --}},%
  terminator sign none/.style={terminator sign=},%
  description delimiters/.code 2 args={\def\kvtcb@desc@delim@left{#1}\def\kvtcb@desc@delim@right{#2}},%
  description delimiters parenthesis/.style={description delimiters=()},
  description delimiters none/.style={description delimiters={}{}},
  description color/.code={\def\temp@a{#1}\ifx\temp@a\@empty\relax%
    \def\tcb@desc@col{}\else\def\tcb@desc@col{\color{#1}}\fi},%
  description color/.default=,
  description font/.store in=\kvtcb@desc@font,
  description font/.default=,
  description formatter/.code={\let\tcb@theo@desc@form=#1},%
  description formatter/.default={\tcb@theo@desc@form@std},%
  theorem name and number/.code={\let\tcb@theo@form=\tcb@theo@form@namenumber},
  theorem number and name/.code={\let\tcb@theo@form=\tcb@theo@form@numbername},
  theorem name/.code={\let\tcb@theo@form=\tcb@theo@form@name},
  theorem style/.is choice,
  theorem style/standard/.style={separator sign colon,description delimiters none,
    terminator sign none,theorem name and number,attach title},
  theorem style/change standard/.style={theorem style=standard,theorem number and name},
  theorem style/plain/.style={separator sign none,description delimiters parenthesis,
    terminator sign colon,theorem name and number,attach title to upper={\ }},
  theorem style/plain apart/.style={separator sign none,description delimiters parenthesis,
    terminator sign none,theorem name and number,attach title},
  theorem style/break/.style={theorem style=plain,attach title to upper={\par}},
  theorem style/change/.style={theorem style=plain,theorem number and name},
  theorem style/change apart/.style={theorem style=plain apart,theorem number and name},
  theorem style/change break/.style={theorem style=break,theorem number and name},
  theorem style/margin/.style={theorem style=plain,theorem name,before title=\makebox[0pt][r]{\thetcbcounter\ }},
  theorem style/margin apart/.style={theorem style=margin,attach title,terminator sign none},
  theorem style/margin break/.style={theorem style=margin,attach title to upper={\par}},
}

\newcommand{\new@tcbtheorem}[5][]{%
  \@@newtcolorbox[auto counter,#1]{#2}[3][]{#4,%
    title={\tcb@theo@title{#3}{\thetcbcounter}{##2}},%
    list entry={\protect\numberline{\thetcbcounter}##2},%
    code={\tcb@theo@label{#5}{##3}},%
    ##1}%
  \@@newtcolorbox[#1,no counter,list inside=]{#2*}[2][]{#4,%
    title={\tcb@theo@title{#3}{\@empty}{##2}},%
    ##1}%
}

\def\newtcbtheorem{\let\@@newtcolorbox\newtcolorbox%
  \new@tcbtheorem}

\def\renewtcbtheorem{\let\@@newtcolorbox\renewtcolorbox%
  \new@tcbtheorem}

\newcommand{\tcbmaketheorem}[5]{%
  \newtcolorbox{#1}[3][]{#3,theorem={#2}{#4}{##2}{#5:##3},##1}%
}

\newtcbox{\tcboxmath}[1][]{nobeforeafter,math upper,tcbox raise base,#1}
\newtcbox{\tcbhighmath}[1][]{highlight math,nobeforeafter,math upper,tcbox raise base,#1}

\tcbset{%
  reset@theorems/.style={%
    description formatter,description color,description font,
    highlight math style={colframe=red,colback=yellow!25!white},%
    theorem style=standard,%
  },
  initialize@reset=reset@theorems,
}



==> tcbxparse.code.tex <==
%% The LaTeX package tcolorbox - version 3.80 (2015/11/27)
%% tcbxparse.code.tex: Code for xparse features
%%
%% -------------------------------------------------------------------------------------------
%% Copyright (c) 2006-2015 by Prof. Dr. Dr. Thomas F. Sturm <thomas dot sturm  at unibw dot de>
%% -------------------------------------------------------------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2005/12/01 or later.
%%
%% This work has the LPPL maintenance status `author-maintained'.
%%
%% This work consists of all files listed in README
%%
%\makeatletter
\tcb@set@library@version{3.80}

\RequirePackage{xparse}[2013/12/31]

\tcbset{%
  IfNoValueTF/.code args={#1#2#3}{\IfNoValueTF{#1}{\pgfkeysalso{#2}}{\pgfkeysalso{#3}}},
  IfValueTF/.code args={#1#2#3}{\IfValueTF{#1}{\pgfkeysalso{#2}}{\pgfkeysalso{#3}}},
  IfBooleanTF/.code args={#1#2#3}{\IfBooleanTF{#1}{\pgfkeysalso{#2}}{\pgfkeysalso{#3}}},
  verbatim/.style={fontupper=\ttfamily,nobeforeafter,tcbox raise base,top=0pt,bottom=0pt,left=1mm,right=1mm,boxrule=0.3mm}
}

%-- tcolorbox --
\long\def\tcb@New@TColorBox#1#2#3{%
  \tcb@newenvironment{#1}{#2}{\tcolorbox[#3,options@for=#1]}{\endtcolorbox}}

\def\DeclareTColorBox{%
  \let\tcb@newenvironment\DeclareDocumentEnvironment%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TColorBox%
  \tcb@process@newenvironment}

\def\NewTColorBox{%
  \let\tcb@newenvironment\NewDocumentEnvironment%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TColorBox%
  \tcb@process@newenvironment}

\def\RenewTColorBox{%
  \let\tcb@newenvironment\RenewDocumentEnvironment%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TColorBox%
  \tcb@process@newenvironment}

\def\ProvideTColorBox{%
  \let\tcb@newenvironment\ProvideDocumentEnvironment%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TColorBox%
  \tcb@process@newenvironment}

%-- tcolorbox (total) --
\long\def\tcb@New@TotalTColorBox#1#2#3#4{%
  \expandafter\tcb@newcommand\csname#1\endcsname{#2}{\begin{tcolorbox}[#3,options@for=#1]#4\end{tcolorbox}}}

\def\DeclareTotalTColorBox{%
  \let\tcb@newcommand\DeclareDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TotalTColorBox%
  \tcb@process@newcommand}

\def\NewTotalTColorBox{%
  \let\tcb@newcommand\NewDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TotalTColorBox%
  \tcb@process@newcommand}

\def\RenewTotalTColorBox{%
  \let\tcb@newcommand\RenewDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TotalTColorBox%
  \tcb@process@newcommand}

\def\ProvideTotalTColorBox{%
  \let\tcb@newcommand\ProvideDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TotalTColorBox%
  \tcb@process@newcommand}

%-- tcbox --
\long\def\tcb@New@TCBox#1#2#3{%
  \expandafter\tcb@newcommand\csname#1\endcsname{#2}{\tcbox[#3,options@for=#1]}}

\def\DeclareTCBox{%
  \let\tcb@newcommand\DeclareDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TCBox%
  \tcb@process@newcommand}

\def\NewTCBox{%
  \let\tcb@newcommand\NewDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TCBox%
  \tcb@process@newcommand}

\def\RenewTCBox{%
  \let\tcb@newcommand\RenewDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TCBox%
  \tcb@process@newcommand}

\def\ProvideTCBox{%
  \let\tcb@newcommand\ProvideDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TCBox%
  \tcb@process@newcommand}

%-- tcbox (total) --
\long\def\tcb@New@TotalTCBox#1#2#3#4{%
  \expandafter\tcb@newcommand\csname#1\endcsname{#2}{\tcbox[#3,options@for=#1]{#4}}}

\def\DeclareTotalTCBox{%
  \let\tcb@newcommand\DeclareDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TotalTCBox%
  \tcb@process@newcommand}

\def\NewTotalTCBox{%
  \let\tcb@newcommand\NewDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TotalTCBox%
  \tcb@process@newcommand}

\def\RenewTotalTCBox{%
  \let\tcb@newcommand\RenewDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TotalTCBox%
  \tcb@process@newcommand}

\def\ProvideTotalTCBox{%
  \let\tcb@newcommand\ProvideDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TotalTCBox%
  \tcb@process@newcommand}

\DeclareTotalTCBox{\tcboxverb}{ O{} v }{verbatim,#1}{#2}

%-- tcboxfit --
\long\def\tcb@New@TCBoxFit#1#2#3{%
  \expandafter\tcb@newcommand\csname#1\endcsname{#2}{\tcboxfit[#3,options@for=#1]}}

\def\DeclareTCBoxFit{%
  \let\tcb@newcommand\DeclareDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TCBoxFit%
  \tcb@process@newcommand}

\def\NewTCBoxFit{%
  \let\tcb@newcommand\NewDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TCBoxFit%
  \tcb@process@newcommand}

\def\RenewTCBoxFit{%
  \let\tcb@newcommand\RenewDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TCBoxFit%
  \tcb@process@newcommand}

\def\ProvideTCBoxFit{%
  \let\tcb@newcommand\ProvideDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TCBoxFit%
  \tcb@process@newcommand}

\long\def\tcb@New@TotalTCBoxFit#1#2#3#4{%
  \expandafter\tcb@newcommand\csname#1\endcsname{#2}{\tcboxfit[#3,options@for=#1]{#4}}}

\def\DeclareTotalTCBoxFit{%
  \let\tcb@newcommand\DeclareDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TotalTCBoxFit%
  \tcb@process@newcommand}

\def\NewTotalTCBoxFit{%
  \let\tcb@newcommand\NewDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TotalTCBoxFit%
  \tcb@process@newcommand}

\def\RenewTotalTCBoxFit{%
  \let\tcb@newcommand\RenewDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TotalTCBoxFit%
  \tcb@process@newcommand}

\def\ProvideTotalTCBoxFit{%
  \let\tcb@newcommand\ProvideDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TotalTCBoxFit%
  \tcb@process@newcommand}


%-- tcblisting --
\long\def\tcb@New@TCBListing#1#2#3{%
  \tcb@newenvironment{#1}{#2}{\tcblisting{#3,options@for=#1}}{\endtcblisting}}

\def\DeclareTCBListing{%
  \let\tcb@newenvironment\DeclareDocumentEnvironment%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TCBListing%
  \tcb@process@newenvironment}

\def\NewTCBListing{%
  \let\tcb@newenvironment\NewDocumentEnvironment%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TCBListing%
  \tcb@process@newenvironment}

\def\RenewTCBListing{%
  \let\tcb@newenvironment\RenewDocumentEnvironment%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TCBListing%
  \tcb@process@newenvironment}

\def\ProvideTCBListing{%
  \let\tcb@newenvironment\ProvideDocumentEnvironment%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TCBListing%
  \tcb@process@newenvironment}

%-- tcbinputlisting --
\long\def\tcb@New@TCBInputListing#1#2#3{%
  \expandafter\tcb@newcommand\csname#1\endcsname{#2}{\tcbinputlisting{#3,options@for=#1}}%
}

\def\DeclareTCBInputListing{%
  \let\tcb@newcommand\DeclareDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TCBInputListing%
  \tcb@process@newcommand}

\def\NewTCBInputListing{%
  \let\tcb@newcommand\NewDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TCBInputListing%
  \tcb@process@newcommand}

\def\RenewTCBInputListing{%
  \let\tcb@newcommand\RenewDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TCBInputListing%
  \tcb@process@newcommand}

\def\ProvideTCBInputListing{%
  \let\tcb@newcommand\ProvideDocumentCommand%
  \let\tcb@process@newtcolorbox@continue\tcb@New@TCBInputListing%
  \tcb@process@newcommand}


%-- sidebyside --

\def\tcb@sbs@content@none{\tcb@sbs@text@left\tcblower\tcb@sbs@text@right}
\def\tcb@sbs@content@left{\box\tcb@upperbox\tcblower\tcb@sbs@text@right}
\def\tcb@sbs@content@right{\tcb@sbs@text@left\tcblower\box\tcb@lowerbox}
\def\tcb@sbs@content@both{\box\tcb@upperbox\tcblower\box\tcb@lowerbox}

\tcbset{%
  sidebyside adapt/.is choice,
  sidebyside adapt/none/.style={%
    sidebyside@adapt@process/.style={%
      code={\let\tcb@sbs@content\tcb@sbs@content@none},
    }%
  },
  sidebyside adapt/left/.style={%
    sidebyside@adapt@process/.style={%
      code={\sbox{\tcb@upperbox}{\tcb@sbs@text@left}\let\tcb@sbs@content\tcb@sbs@content@left},
      lefthand width=\wd\tcb@upperbox,
    }%
  },
  sidebyside adapt/right/.style={%
    sidebyside@adapt@process/.style={%
      code={\sbox{\tcb@lowerbox}{\tcb@sbs@text@right}\let\tcb@sbs@content\tcb@sbs@content@right},
      righthand width=\wd\tcb@lowerbox,
    }%
  },
  sidebyside adapt/both/.style={%
    sidebyside@adapt@process/.style={%
      code={\sbox{\tcb@upperbox}{\tcb@sbs@text@left}\sbox{\tcb@lowerbox}{\tcb@sbs@text@right}\let\tcb@sbs@content\tcb@sbs@content@both},
      text width=\wd\tcb@upperbox+\kvtcb@sbs@gap+\wd\tcb@lowerbox,
      lefthand width=\wd\tcb@upperbox,
    }%
  },
  %
  sidebyside switch/.is choice,
  sidebyside switch/true/.style={%
    sidebyside@switch/.code={%
      \tcb@swap{\tcb@sbs@text@left}{\tcb@sbs@text@right}
    }%
  },
  sidebyside switch/false/.style={%
    sidebyside@switch/.style=%
  },
  sidebyside switch/.default=true
}


\DeclareTotalTColorBox{\tcbsidebyside}{ +O{} +m +m }{%
  code={\long\def\tcb@sbs@text@left{#2}\long\def\tcb@sbs@text@right{#3}},%
  #1,%
  sidebyside,%
  sidebyside@switch,sidebyside@adapt@process%
}{\tcb@sbs@content}


\tcbset{%
  reset@xparse/.style={%
    sidebyside adapt=none,sidebyside switch=false,%
  },
  initialize@reset=reset@xparse,
}

